Declarative Probabilistic Logic Programming in Discrete-Continuous Domains

Over the past three decades, the logic programming paradigm has been successfully expanded to support probabilistic modeling, inference and learning. The resulting paradigm of probabilistic logic programming (PLP) and its programming languages owes much of its success to a declarative semantics, the so-called distribution semantics. However, the distribution semantics is limited to discrete random variables only. While PLP has been extended in various ways for supporting hybrid, that is, mixed discrete and continuous random variables, we are still lacking a declarative semantics for hybrid PLP that not only generalizes the distribution semantics and the modeling language but also the standard inference algorithm that is based on knowledge compilation. We contribute the measure semantics together with the hybrid PLP language DC-ProbLog (where DC stands for distributional clauses) and its inference engine infinitesimal algebraic likelihood weighting (IALW). These have the original distribution semantics, standard PLP languages such as ProbLog, and standard inference engines for PLP based on knowledge compilation as special cases. Thus, we generalize the state of the art of PLP towards hybrid PLP in three different aspects: semantics, language and inference. Furthermore, IALW is the first inference algorithm for hybrid probabilistic programming based on knowledge compilation

==> experiment_dc/Dockerfile <==
FROM ubuntu:14.04


RUN apt-get update \
    && \
    echo "------------------------------------------------------ essentials" \
    && \
    apt-get install -y --no-install-recommends -y \
    build-essential \
    apt-utils \
    && \
    echo "------------------------------------------------------ editors" \
    && \
    apt-get install -y --no-install-recommends -y \
    emacs \
    vim \
    nano \
    && \
    echo "------------------------------------------------------ software" \
    && \
    apt-get install -y --no-install-recommends -y \
    python3-pip \
    tmux \ 
    wget \
    git \
    unzip





RUN echo "------------------------------------------------------ YAP install" \
    && \
    apt-get install -y --no-install-recommends libreadline6 libreadline6-dev libncurses5-dev \
    && \
    wget https://bitbucket.org/problog/dc_problog/downloads/yap-6.2.2.zip \
    && \
    unzip yap-6.2.2.zip \
    && \
    cd yap-6.2.2 \
    && \
    mkdir arch \
    && \
    cd arch \
    && \
    ../configure --enable-tabling=yes --enable-dynamic-loading --disable-myddas \
    && \
    make \
    && \
    make install \
    && \
    make install_library


RUN echo "------------------------------------------------------ DC install" \
    && \
    apt-get install -y --no-install-recommends  libgsl0-dev libgsl0ldbl \
    && \
    apt-get install -y --no-install-recommends libboost-all-dev  \
    && \
    cd / \
    && \
    git clone https://github.com/davidenitti/DC.git \
    && \
    cd DC \
    && \
    sh make.sh


RUN echo "------------------------------------------------------ cleanup" \
    apt-get clean && rm -rf /var/lib/apt/lists/*

==> files_excluded/implementation.tex <==

\section{Implementing \dcproblogsty}
\label{sec:implementation}

Having developed a probabilistic inference approach for \dcproblogsty based on knowledge compilation and similar to the one of \problogsty has the advantage of allowing us to leverage existing implementations of \problogsty (and its inference algorithms) in order to implement \dcproblogsty.
This entails that our implementation of \dcproblogsty, which we dub \dcproblogsys, inherits its general architecture from \problogsys and performs inference via a number of deterministic program transformations~\citep{dries2015problog2}. These program transformations reflect the inference steps described in Section~\ref{sec:dc2smt} and Section~\ref{sec:alw}.
We graphically summarize the program transformations in Figure~\ref{figure:dcproblog_sys} and describe further details in Appendix~\ref{sec:system_blocks}.
In Appendix~\ref{sec:system_query_predicates} we introduce built-in system predicates that allow a user to query and condition on atoms of interest, whose use we then briefly exhibit in Appendix~\ref{sec:usage}, where we present the usage of our implementation.


\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{../figures/dcproblog_sys.pdf}
	\caption[Overview of the program transformation steps in the \dcproblogsys system]{Overview of the program transformation steps in the \dcproblogsys system. The nodes represent the intermediate representations and the annotations of the arrows show which transformations is performed on them. Each transformation is implemented in a seperate system block. (Figure inspired by~\protect\citep[Figure 2]{zuidbergdosmartires2019transforming} and \citep[Figure 1]{dries2015problog2}.}
	\label{figure:dcproblog_sys}
\end{figure}





\subsection{System Blocks}
\label{sec:system_blocks}

The system blocks that constitute \dcproblogsys are alterations of the existing system blocks already present in the \problogsys implementation, which is mainly written in Python\footnote{\url{https://github.com/ML-KULeuven/problog}}. Consequently, \dcproblogsys is written in Python as well and effectively extends \problogsys with continuous random variables but also discrete random variables with infinite support (cf. Poisson distribution). We would like to point out that in the absence distributional facts, \dcproblogsty programs in \dcproblogsys are equivalent to \problogsty programs in \problogsys.

\paragraph{\bf Grounding}
Inference in \dcproblogsys starts with a non-ground probabilistic program, a query set and an evidence set. In a first instance, the program is grounded with respect to the query set, which results in the (relevant) ground program. Grounding is performed using the resolution rules described in Appendix~\ref{app:resolution}.
\dcproblogsys reuses the grounder of \problogsys by adding additional resolution rules to the ones that are already implemented. More specifically, \dcproblogsys additionally has resolution rules for the cases {\bf C3} to {\bf C6} (cf. Definition~\ref{def:resolution_rules}), while the resolution rules for the cases {\bf C1} and {\bf C2} are already present in \problogsys's grounder. Note that \problogsys has special resolution rules for probabilistic facts and annotated disjunctions, which means that the \dcproblogsys implementation can also handle these. In the absence of distributional facts grounding in \dcproblogsys is identical to grounding in \problogsys as none of the rules for {\bf C3} to {\bf C6} are used. 




\paragraph{\bf Breaking Cycles}
Once we have the relevant ground program we would like to obtain a cycle-free representation of the program, as such a cycle-free program is trivially mapped onto a Boolean formula (cf. Section~\ref{sec:relprog2boolfrom}). Concerning the cycle breaking step, \dcproblogsys reuses the cycle breaking algorithm deployed in \problogsys with minor bookkeeping extensions in order to ensure consistency between the names of random variables (stemming from distributional facts) before and after performing cycle breaking.  




\paragraph{\bf Knowledge Compiling}
Next, \dcproblogsys takes, a labeled propositional formula, \ie the acyclic representation of the program, and knowledge compiles it into a so-called sentential decision diagram (SDD)~\citep{darwiche2011sdd}.
Identically to \problogsys, the compilation of SDDs, which are a strict subset of d-DNNF formulas, is performed using bottom-up compilation\footnote{\url{http://reasoning.cs.ucla.edu/sdd/}}~\citep{choi2013dynamic}.

Currently, the compilation of labeled propositional formulas is agnostic towards information present in the labels of the atoms. This can lead to situations where infeasible labeled formula are not discarded. Take for instance the formula $a \land b$, where the labels are $\alpha(a)=\ive{x<0}$ and $\alpha(b)=\ive{x>1}$. Clearly there is no instantiation of $x$ that would satisfy the conditions in the labels. However, as the compiler is label-agnostic, it does not take this information into account and does not disregard such a formula by setting it equivalent to $\bot$. This might results in needless computations. To prevent this from happening one could take into account the information in the labels and effectively perform knowledge compilation with SMT formulas, which has been studied in the WMI literature~\citep{sanner2011symbolic,kolb2018efficient,kolb2019exploit,derkinderen2020ordering}.
We leave it for future research to adapt and further develop these techniques in the context of probabilistic programming.\footnote{We establish the link between computing expected labels of propositional logic formulas and weighted model integration in  Appendix~\ref{app:labeled_prop_to_SMT}.}




\paragraph{\bf Evaluating} Finally, we obtain the probability of a query to a (hybrid) probabilistic logic program by evaluating the compiled logic formula using algebraic likelihood weighting.
Note that the arithmetic circuit that corresponds to the compiled formula does not contain any program branches, in other words there are no if-else statements presents. Effectively, knowledge compilation transforms a query to a probabilistic query into a branchless program that can trivially be run on a graphics processing unit. Furthermore, we observe that each iteration in the loop of Algorithm~\ref{alg:unormalize_alw} uses the same (branchless) circuit. This means that the loop in Algorithm~\ref{alg:unormalize_alw} is  embarrassingly parallelizable, as already pointed out by~\citet{zuidbergdosmartires2019exact}.
\dcproblogsys implements the circuit evaluations for the different samples by using a vectorized version of Algorithm~\ref{alg:unormalize_alw} implemented in PyTorch~\citep{paszke2019pytorch} and Pyro~\citep{bingham2019pyro}.









\subsection{System Predicates to Query \dcproblogsty Programs}
\label{sec:system_query_predicates}

Implementations of probabilistic programming languages usually define a set of system predicates that allow users to declare queries and conditioning sets within a probabilistic program.
% A key issue of these system predicates is that they should encode unambiguous inference tasks, \eg encode conditional probabilities that exist and do not succumb to the Borel-Kolmogorov paradox. \ak{didn't you say in an earlier comment that syntax cannot ensure this? I agree about the unambiguous part, but not the rest.}
We are going to introduce such system predicates for \dcproblogsty based on \problogsty's system predicates.  

% Many probabilistic programming languages are often quite permissive with the use of system predicates for querying programs. This can then result in possibly ill-defined queries, such as in Distributional Clauses~\citep[Section 3.2]{nitti2016probabilistic}.
% Other languages, such as BLOG, leave it up to the user and simply assume the well-definedness of conditional probability queries~\citep{wu2018discrete}.
% A more sophisticated method to tackle the non-uniqueness of the conditional probability is {\em disintegration}~\citep{shan2017exact}, where, instead of returning a conditional probability, a family of conditional probabilities is returned (representing an uncountable number of limits).
% However, this does not resolve the issue of the observation/measuring process being inherently underspecified.








\begin{definition}[Query Predicates]
	\label{def:query_predicates}
	Let $\herbrandbase$ be the Herbrand base of a given \dcproblogsty program \dcpprogram.
	Let us assume that we are given the evidence $\evidenceset=e$ (with $\evidenceset \subset \herbrandbase$).
	and a set $\queryset \subset \herbrandbase$ of atoms of interest, called
	query atoms.
	We encode these sets directly as facts in \dcpprogram using the following system predicates:
	\begin{itemize}
		\item The unary predicate \probloginline{query/1} declares a set of Boolean atoms of interest $\queryset = \{ \text{\probloginline{q}} \mid \text{\probloginline{query(q)}} \in \dcpprogram     \}$.
		% 
		\item The binary predicate \probloginline{evidence/2}, where the second argument is either the \probloginline{true} symbol or the \probloginline{false} symbol, encodes a set of Boolean atoms that we condition on. It produces an ordered set of evidence atoms:
		$$
		\evidenceset =
		\{ E_\text{\probloginline{e@$_i$@}}  \mid \text{\probloginline{evidence(e@$_i$@,false)} } \in \dcpprogram \}
		\cup
		\{   E_\text{\probloginline{e@$_i$@}} = \mid \text{\probloginline{evidence(e@$_i$@,true)}} \in \dcpprogram \} $$
		and the corresponding ordered multiset of truth values for the elements of $\evidenceset$:
		$$
		e =
		\{  0   \mid \text{\probloginline{evidence(e@$_i$@,false)} } \in \dcpprogram \}
		\cup
		\{ 1 \mid \text{\probloginline{evidence(e@$_i$@,true)}} \in \dcpprogram \}
		$$
		The probability $P_\dcpprogram(\evidenceset=e)$ now corresponds to the denominator in Equation~\ref{eq:conditional_prob}.
		The unary version \probloginline{evidence/1} is shorthand for the \probloginline{true} case and omits the second argument.
		
		\item The binary predicate \probloginline{observation/2} is used to condition random variables on observed values they take. The first argument denotes a random term and the second one the observed value. We define the semantics of the \probloginline{observation/2} predicate in terms of  \probloginline{evidence/1} and a novel Boolean comparison predicate \probloginline{delta_interval/2}. The atom \probloginline{observation(x,v)} is syntactic sugar for two clauses of the form:
		\begin{problog}
obs:- delta_interval(x,v).
evidence(obs).
		\end{problog}
		where \probloginline{obs} is a fresh ground atom. \probloginline{delta_interval/2} is the built-in comparison predicate describing infinitesimally small intervals and which we introduce in Definition~\ref{def:delta_interval}.
	\end{itemize}
\end{definition}




The \probloginline{query} and \probloginline{evidence} predicates are inherited from \problogsty, contrary to \probloginline{observation}, which we introduce in order to handle point observations of both discrete and continuous random variables via the \probloginline{delta_interval/2} predicate.
%Note that the definition of the \probloginline{observation} predicate can equally be used with discrete and continuous random variables. This will allow us to condition queries to \dcproblogsty programs on mixed discrete-continuous random variables, cf. Example~\ref{ex:indian_gpa}.








\subsection{System Usage}
\label{sec:usage}

We provide two modes of use for \dcproblogsys. Firstly, through the command line  and secondly, as \dcproblogsys is implemented in Python, through Python scripts. To illustrate the command line interface, consider a file named \mintinline{bash}{coin_flip.pl} containing the program described in Example~\ref{example:bayesian_learning}.

\begin{example}\label{example:bayesian_learning}
	We model a coin flip scenario where the probability of the coin turning up heads is defined through two distributional clauses. We then flip the coin three times and get as evidence that the first and third flip turn up heads, and the second coin turns up tails. We then query for the probability of \probloginline{b>0.5.}
	\begin{problog*}{linenos}
0.2::a.
b~beta(1,1):- a.
b~beta(1,2):- not a.
b::coin_flip(N).

evidence(coin_flip(1), true).
evidence(coin_flip(2), false).
evidence(coin_flip(3), true).

q: b>0.5.
query(q).
	\end{problog*}
\end{example}
Having \dcproblogsys installed on a machine, which we provide as an extension of \problogsys, we can execute the query with the following command line instruction:
\begin{minted}{bash}
problog dc simple_coin.pl -n_samples=20000
\end{minted}
The instruction simply expresses our desire to run the \mintinline{bash}{simple_coin.pl} file using \problogsys with the \dcproblogsys extension and to furthermore use $20000$ samples (per random variable) to answer the query.

Alternatively, \dcproblogsys can also be used within Python scripts directly, which enhances its flexible as Python code can be mixed with ProbLog programs. For instance, take again the program from Example~\ref{example:bayesian_learning}. We can now extend \dcproblogsys with a new builtin \probloginline{samples} predicate that returns sampled values of random variables instead of querying for probabilities, cf. Example~\ref{example:bayesian_learning_python}.

\begin{example}[Using ProbLog from Python]
\label{example:bayesian_learning_python}
We write the program in Example~\ref{example:bayesian_learning} within a Python script and also use the \probloginline{samples} predicates to obtain samples. 

\begin{minted}[linenos]{python}
#import necessary classes from core ProbLog
from problog.program import PrologString

# import classes from DC-ProbLog
from problog.tasks.dcproblog.solver import InferenceSolver
from problog.tasks.dcproblog.parser import DCParser

# set up the configuration for inference
configuration = {
    "n_samples":20000, # set the number of samples to be used
    "device":"gpu", # use the GPU (alterntively CPU)
}

# put the ProbLog program in a string
str_program = """
    0.2::a.
    b~beta(1,1):- a.
    b~beta(1,2):- \+a.
    B::coin_flip(N):- B is b.
    
    evidence(coin_flip(1), true).
    evidence(coin_flip(2), false).
    evidence(coin_flip(3), true).
    
    samples(b).  % we are interested in samples
"""

# initiliaze the solver for DC-ProbLog inference
solver = InferenceSolver(**configuration)

# obtain a ProbLog program from a string 
# using the DCParser instead of the ProbLog parser
program = PrologString(str_program, parser=DCParser())

# query the program
probabilities = solver.probability(program, **configuration)
\end{minted}

The \mintinline{python}{probabilities} variable now contains the samples for the two beta distributions in the \dcproblogsty program. Retrieving the samples allows us to plot them as a histogram. We do this in Figure~\ref{fig:coins}.
\end{example}











\begin{figure}[h]
	\begin{center}
	\includegraphics[width=0.49\linewidth]{../figures/prior.pdf}
	\includegraphics[width=0.49\linewidth]{../figures/posterior.pdf}
	\end{center}
	\caption[Bayesian learning of coins]{On the left we have the histogram for the unconditioned samples (prior) from the program in Example~\ref{example:bayesian_learning} and the histogram on the right demonstrates the effect of conditioning on the outcome of the coin flips (posterior). The green part of the histogram corresponds to the first distributional clause (\probloginline{b~beta(1,1)}) and the red part to the second (\probloginline{b~beta(1,2)}).}
	\label{fig:coins}
\end{figure}



% Figure~\ref{fig:coins} shows the prior and posterior after learning with the dataset {\probloginline{coin_flip(1)=true}, \probloginline{coin_flip(2)=false}, \probloginline{coin_flip(3)=true}}.



% \subsection{old section intro}
% We make two observations:
% \begin{enumerate}
%     \item Every implementation of \prologsty  (or any other logic programming language)  reserves a set of {\em  system predicates} executing code not written in pure \prologsty~\citep[Chapter 8]{sterling1994art}.
%     System predicates complement pure \prologsty implementations and give users access to efficient algorithms that are cumbersome to implement in pure logic programming -- for instance algorithms for numeric computations.
%     \item In Section~\ref{sec:semantics} we have seen that we can separate a probabilistic logic program into a set of independent random choices and a logic program. The independent choices and the logic program communicate to each other via comparison predicates. Comparison predicates are an instance of system predicates.
% \end{enumerate}

% These observations hint at the possibility of implementing \dcproblogsty as a deterministic logic programming language with access to an external engine with support for random variables.
% On an implementation level, the key difference between a probabilistic logic programming language and a (deterministic) logic programming language is the availability of probability distributions in the external engine of the former.

% Decoupling independent choices (random variables) and the deterministic system (logic program) does also mean that we should be able to take a probabilistic logic programming language that only supports finite discrete probability distributions and extend it with continuous probability distributions.
% We will demonstrate how to achieve this by adding continuous random variables to the ProbLog2 system~\citep{dries2015problog2} (the most recent implementation of \problogsty). We dub our implementation \dcproblogsys.


==> files_excluded/procedural_semantics.tex <==
\section{Procedural Semantics of \dcproblogsty}\label{sec:swp}
We now provide a procedural view on the semantics that extends \citet{van1991well}'s $W_\dcpprogram$-operator for well-founded models to deal with comparison literals following the approach of the stochastic $T_\dcpprogram$-operator for negation-free distributional clauses \citep{gutmann2011magic}. As in the latter, we exclude comparison atoms from interpretations, and instead introduce a function \textsc{ReadTable}$(\cdot)$ that keeps track of the sampled values of random variables to evaluate comparison literals. Given a comparison literal \probloginline{q}, \textsc{ReadTable(\probloginline{q})}  returns the truth value of \probloginline{q} based on the values of the random terms \probloginline{x} in \probloginline{q}, which are either retrieved from the table or sampled according to their definition \probloginline{x~D} as included in the interpretation and stored in the table in case they are not yet available. 

\subsection{Unfounded Sets}

We first extend the notion of \emph{unfounded set}, which is used to draw negative conclusions, to the stochastic case.
\begin{definition}[Stochastic unfounded set]
	Let $\dcpprogram$ be a DC-ProbLog program with Herbrand base $H$. Let $I$ be a partial interpretation of  $H\setminus F$, \ie, not including comparison atoms. 
	We say that  $A\subseteq H\setminus F$ is a stochastic unfounded set (of $\dcpprogram$) with respect to $I$ if each atom $a\in A$ satisfies the following condition: For each instantiated rule $R$ of $\dcpprogram$ whose head is $a$, (at least) one of the following holds:
	\begin{enumerate}
		\item Some (positive or negative) non-comparison subgoal $q$ of the body is false in $I$.
		\item For some comparison literal $q$ in the body, the following both hold
		\begin{itemize}
			\item $I$ contains  a true atom \probloginline{x~D} for every random term \probloginline{x} in \probloginline{q}.
			\item $\textsc{ReadTable(\probloginline{q})}=true$
		\end{itemize}
		\item Some positive subgoal of the body occurs in $A$.
	\end{enumerate}
	The greatest stochastic unfounded set (of $\dcpprogram$) with respect to $I$, denoted $SU_\dcpprogram(I)$, is the union of all sets that are unfounded with respect to $I$.
\end{definition}
We note that comparison literals can invalidate external support for an unfounded set only if all involved random variables have associated distributions in the partial interpretation. \todo{example}

\begin{definition}[Stochastic $W_\dcpprogram$-operator]\label{def:swp}
	We define the transformations $ST_\dcpprogram$, $SU_\dcpprogram$, and $SW_\dcpprogram$ as follows:
	\begin{itemize}
		\item $p\in T_\dcpprogram(I)$ if and only if there is some instantiated rule $R$ of $\dcpprogram$ such that $R$ has head $p$, and
		\begin{itemize}
			\item each non-comparison  literal in the body of $R$ is true in $I$,
			\item $I$ contains a true atom \probloginline{x~D} for every random term \probloginline{x} that appears inside a comparison literal in the body, and 
			\item for each comparison literal \probloginline{q} in the body, $\textsc{ReadTable(\probloginline{q})}=true$
		\end{itemize}
		\item $SU_\dcpprogram(I)$ is the greatest unfounded set of $\dcpprogram$ with respect to $I$.
		\item $SW_\dcpprogram(I) = ST_\dcpprogram(I) \cup \neg SU_\dcpprogram(I)$
	\end{itemize}
	where negation applied to a set negates each element of the set.
\end{definition}
That is, comparison literals in rule bodies are evaluated based on the table, but can only decide on whether a rule is fired (in $ST_\dcpprogram$) or blocked (in $SU_\dcpprogram$) if all their random variables have a distributional atom in the (partial) interpretation.
However, for valid core \dcproblogsty programs, the first iteration of fixpoint computation adds all distributional facts to the interpretation. Thus, from the second iteration onwards, all rules with comparison atoms will have their necessary \probloginline{x~D} atoms available, and may access the table to evaluate comparisons. The procedural view thus exactly mirrors the three layers of the declarative view: it first introduces all random variables and their distributions, which then makes it possible to evaluate comparison atoms based on the sampled joint assignment maintained by the table, and thus enables derivation of logical consequences through the computation of the well-founded model. 

\todo{too much context assumed -- expand / illustrate}




\subsection{Procedural view}
As stated above, the semantics of a full \dcproblogsty program is given by the corresponding core program, which explicitly encodes in the program how each random term should be interpreted based on logical context. 
In Section~\ref{sec:swp}, we provided a procedural view on the semantics through the stochastic $W_\dcpprogram$ operator, which, as the procedural semantics of the distributional clause language, incorporates these context checks into the execution mechanism rather than the program itself. While the explicit encoding makes the program and its semantics independent of the execution mechanism, this generality comes at the price of a potentially significant blowup in program size, as illustrated in the following example.



\begin{example}
	Consider the following program fragment modeling a robot moving along a one-dimensional corridor under different conditions.
	\begin{problog*}{linenos}
0.2::cond(1); 0.5::cond(2); 0.3::cond(3).
pos(0) ~ normal(20,3).
pos(1) ~ normal(pos(0)+0.5, 0.1) :- cond(1). @\label{line:cond1pos1}@
pos(1) ~ normal(pos(0), 0.5) :- cond(2).
pos(1) ~ normal(pos(0), 2) :- cond(3).
pos(2) ~ normal(pos(1)+0.5, 0.1) :- cond(1). @\label{line:cond1pos2}@
pos(2) ~ normal(pos(1), 0.5) :- cond(2).
pos(2) ~ normal(pos(1), 2) :- cond(3).
...
	\end{problog*}
	Given any interpretation of the AD, only one of the three conditions applies, and determines the distribution to associate with every position. For instance, if \probloginline{cond(1)} holds, \probloginline{pos(1)} is determined by line~\ref{line:cond1pos1} only, and \probloginline{pos(2)} by line~\ref{line:cond1pos2}.  The transformed program, however, has to summarize \emph{all} situations, and thus needs a correspondingly larger set of random variables. We omit the transform of the annotated disjunction for brevity:
	\begin{problog*}{linenos}
v1 ~ normal(20,3).
refers2rv(pos(0),v1).

v2 ~ normal(v1+0.5, 0.1).
refers2rv(pos(1),v2) :- refers2rv(pos(0),v1),cond(1).
v3 ~ normal(v1, 0.5).
refers2rv(pos(1),v3) :- refers2rv(pos(0),v1),cond(2).
v4 ~ normal(v1, 2).
refers2rv(pos(1),v4) :- refers2rv(pos(0),v1),cond(3).

v5 ~ normal(v2+0.5, 0.1).
refers2rv(pos(2),v5) :- refers2rv(pos(1),v2), cond(1).
v6 ~ normal(v3+0.5, 0.1).
refers2rv(pos(2),v6) :- refers2rv(pos(1),v3), cond(1).
v7 ~ normal(v4+0.5, 0.1).
refers2rv(pos(2),v7) :- refers2rv(pos(1),v4), cond(1).
v8 ~ normal(v2, 0.5).
refers2rv(pos(2),v8) :- refers2rv(pos(1),v2), cond(2).
v9 ~ normal(v3, 0.5).
refers2rv(pos(2),v9) :- refers2rv(pos(1),v3), cond(2).
v10 ~ normal(v4, 0.5).
refers2rv(pos(2),v10) :- refers2rv(pos(1),v4), cond(2).
v11 ~ normal(v2, 2).
refers2rv(pos(2),v11) :- refers2rv(pos(1),v2), cond(3).
v12 ~ normal(v3, 2).
refers2rv(pos(2),v12) :- refers2rv(pos(1),v3), cond(3).
v13 ~ normal(v4, 2).
refers2rv(pos(2),v13) :- refers2rv(pos(1),v4), cond(3).
...
	\end{problog*}
	As the transform is purely syntactical, in this specific example, where conditions do not change from one timestep to the next, many of the random variables it introduces are irrelevant, as they correspond to impossible combinations of contexts. For instance, \probloginline{v6} is relevant only if \probloginline{v3} is relevant and \probloginline{cond(1)} holds (line 14), but \probloginline{v3} is relevant only if \probloginline{cond(2)} holds (line 7), which is inconsistent with \probloginline{cond(1)}. 
\end{example}

It is worth noting that, for a valid AD-free program $\dcpprogram$, the fixpoint of  the $SW_\dcpprogram$-operator (Definition~\ref{def:swp}) applied on $\dcpprogram$ itself realizes the same distribution over the non-comparison atoms' truth values as that of applying the operator to the transform of $\dcpprogram$, despite the fact that the transform uses different names for random variables. The $SW_\dcpprogram$-operator controls the application of rules with comparison literals in the body through the presence of suitable distributional atoms in the partial interpretation, which for distributional clauses can only appear in the interpretation if the body of the clause is satisfied. In the transformed program, the same control mechanism is explicitly implemented in the program itself through \dcplpinline{refers2rv}-atoms, whose defining rules mirror the original DC bodies.



==> files_excluded/smart_grounding.tex <==
\section{Grounding via Resolution}
\label{app:resolution}

In Section~\ref{sec:ALWviaKC} we describe the conversion of a queried \dcproblogsty program to a labeled propositional formula through a sequence of deterministic steps. The first of which is obtaining the relevant ground program with respect to a set of query atoms and evidence atoms.

The goal of this first step of the conversion algorithm is to identify a ground core \dcproblogsty program $\dcpprogram_g$ that defines the same joint distribution over the query and evidence atoms as the original program, and contains only logical rules and distributional facts that are relevant for the query and evidence atoms. 

To achieve this goal, we define a procedure that constructs a ground core program for each potential logical derivation of an atom. We use this procedure to construct the full ground program by iterating over all such derivations for the query and evidence atoms. The procedure itself consists of two steps. First, it constructs a derivation using a set of dedicated resolution rules, where each application of a resolution rule produces a tag consisting of a set of logical rules and a set of rule manipulation instructions. If the first step succeeds, the sequence of tags is then translated to a ground program in the second step by applying the rule manipulation instructions of the tags.

The overall approach 
%as well as the two rules for  atoms defined by logical rules are 
is borrowed from the corresponding procedure introduced by \citet{fierens2015inference} for \problogsty. To generalize this approach to \dcproblogsty, we introduce rules to deal with comparison atoms, distributional clauses, and the context-dependent random variables they introduce, in addition to the original rules intriduced by~\citet{fierens2015inference}.\footnote{\citet{nitti2016probabilistic} also introduced modified resolution rules for hybrid probabilistic logic programs but for an inference algorithm that interleaves grounding and sampling, which does not require keeping track of rule groundings.}

%To obtain the relevant ground program for a \problogsty program, \citet{fierens2015inference} introduce a backward chaining procedure that applies SLD resolution~\citep{kowalski1974predicate,sterling1994art}, but ignores negation symbols, as the goal is to \emph{identify}   ground rules that are (potentially) relevant for proving query or evidence atoms rather than to actually  \emph{prove} those atoms. 

%We extend this procedure to \dcproblogsty, where we additionally need to 
%identify the \emph{relevant distributional facts}, \ie, the random variables that are interpreted in the relevant ground program and their distributions. As we have seen in Sections~\ref{sec:semantics} and~\ref{sec:dcproblog}, random variables can be interpreted both within comparison literals and within distributions of other random variables, and can be context-dependent, \ie, the same random variable term may be used to refer to several random variables introduced by a set of distributional clauses. We therefore  introduce additional  resolution rules to handle these cases.\footnote{\citet{nitti2016probabilistic} also introduced modified resolution rules for hybrid probabilistic logic programs but for an inference algorithm that interleaves grounding and sampling.}

%In order to obtain the relevant ground program we deploy, similarly to \problogsty, {\em selective linear definite clause} resolution~\citep{kowalski1974predicate,sterling1994art} with {\em negation as failure}~\citep{Clark1977NegationAF} (SLDNF). SLDNF resolution allows for computing the relevant ground program for a specific query to the logic program, while avoiding the grounding of unnecessary predicates~\citep{kersting2000bayesian,fierens2015inference}. In the case of range-restricted programs SLDNF resolution is guaranteed to terminate. We refer the reader to \citet{fierens2015inference} for a more detailed account of grounding procedure. However, in order to handle comparison predicates and distributional clauses, we will need to modify the SLDNF-resolution rules\footnote{\citet{nitti2016probabilistic} also introduced modified resolution rules for hybrid probabilistic logic programs but for an inference algorithm that interleaves grounding and sampling.}.

%Before we describe the the adapted SLDNF  resolution rules, which we dub {\em SLDNF-DC resolution}, we need specify two helper functions and a builtin predicate that are used during SLDNF-DC resolution:
In contrast to the declarative transformation used to define the semantics of full \dcproblogsty, cf.~Definition~\ref{def:adfree-to-core}, which introduces additional atoms and rules to describe the logical contexts in which specific instances of a random variable term are used, the grounding procedure directly incorporates the original context definitions into the bodies of ground rules, without introducing further atoms.  
Our resolution rules further rely on two global helper functions and an auxiliary predicate:
\begin{itemize}
	\item The injective helper function `$\mathrm{createRVname}$' maps a pair consisting of a ground random variable term and a logical context\footnote{We syntactically represent the context as a tuple of terms, which is interpreted as their logical conjunction (and thus independently of order) by the function.} to a unique constant. This constant serves as the name for the random variable term in the specific context, thus providing an external implementation of the \probloginline{refers2rv/2} predicate.
	\item The function `$\mathrm{symbols}$' maps a term~$t$  to the set of random variable terms in~$t$.  For instance, $\mathrm{symbols}(\text{\probloginline{a(N)+b(1)*2}})$ returns the set $\{ \text{\probloginline{a(N)}}, \text{\probloginline{b(1)}} \}$. This function is crucial to identify relevant random variable terms. 
	\item The auxiliary predicate \probloginline{rv/3}  takes as first argument a random variable term, as second argument a distribution term, and as third argument a context for the random variable term, which is given as a tuple of terms. \probloginline{rv/3} atoms are inserted into the current conjunctive goal when new random variables are identified, and trigger the creation of the corresponding random variable once its full ground context, which combines the body of the defining distributional clause with the contexts of the parent random variables, is determined.
\end{itemize}

We describe each resolution rule using three elements: the condition under which the rule applies (\cposlit to \crvone), the actual resolution step performed by the rule (\rposlit to \rrvonea and \rrvoneb), and the tag that labels this step (\tposlit to \trvone). We overload substitution notation to also allow for substitution of a random variable term by a newly introduced context dependent random variable name. The context-dependent rewrite operator $\twoheadleftarrow$ introduced in the last tag (\trvone) will be defined in Definition~\ref{def:context-substitution}.

\begin{definition}[Resolution Rules]
	\label{def:resolution_rules}
	
	%Let $T_{RV}$ be a hash table of $(key, value)$ pairs that keeps track of random variables (key) and their distributions (value), with insertion function $\mathrm{INSERT}(T_{RV},key,value)$. 
	Let $T_{RV}$ be a hash table that keeps track of random variables, with insertion function $\mathrm{INSERT}(T_{RV},var)$. 
	The six resolution rules for grounding \dcproblogsty programs with respect to a given goal are defined as follows. 
	
	\begin{enumerate}
		\item[\cposlit] If the goal is $(l_1, l_2, \dots, l_n)$ and  $\exists \theta$ such that  $h \lpif b_1, \dots, b_m \in \dcpprogram$, $\theta  = mgu(l_1, h)$ then:
		\begin{align*}
			&{\text{\bf \rposlit:}} \quad (l_1, l_2, \dots, l_n) \vdash (b_1, \dots, b_m, l_2, \dots, l_n) \theta
			\\
			&{\text{\bf \tposlit:}} \quad \tau = (\{ h \lpif b_1, \dots, b_m \}, \theta)
		\end{align*}
		
		\item[\bf \cneglit]  If the goal is $(not(l_1), l_2, \dots, l_n)$ and  $\exists \theta$ such that  $h \lpif b_1, \dots, b_m \in \dcpprogram$, $\theta  {=} mgu(l_1, h)$ then:
		\begin{align*}
			&{\text{\bf \rneglit:}} \quad (not(l_1), l_2, \dots, l_n) \vdash (b_1, \dots, b_m, l_2, \dots, l_n) \theta
			\\
			&{\text{\bf \tneglit:}} \quad \tau = (\{ h \lpif b_1, \dots, b_m \}, \theta)
		\end{align*}
		
		\item[\ccompone]  If the goal is $( l_{comp}, l_1, \dots, l_n )$ where  $l_{comp}$ is a comparison literal, and  there exists a substitution $\theta$ such that for some $s \in symbols(l_{comp})\setminus T_{RV}$ it holds that $h\sim d\lpif b_1, \dots, b_m\in \dcpprogram$, with $\theta = mgu(s,h)$, then:
		\begin{align*}
			&{\text{\bf \rcompone:}} \quad ( l_{comp}, l_1, \dots, l_n ) \vdash (b_1, \dots, b_m, rv(h, d, (b_1, \dots, b_m)),  l_{comp}, l_1,\dots ,l_n)\theta
			\\
			&{\text{\bf \tcompone:}} \quad \tau = (\emptyset, \theta)
		\end{align*}
		
		\item[\bf \ccomptwo]  If the goal is $( l_{comp}, l_1, \dots, l_n )$  where $l_{comp}$ is a comparison literal, and   $symbols(l_{comp})\subseteq T_{RV}$ then:
		\begin{align*}
			&{\text{\bf \rcomptwo:}} \quad  ( l_{comp}, l_1, \dots, l_n ) \vdash  (l_1, \dots, l_n )
			\\
			&{\text{\bf \tcomptwo:}} \quad \tau = (\emptyset, \emptyset)
		\end{align*}
		
		\item[\bf \crvtwo]  If the goal is $(rv(x, d, (b_1, \dots, b_{m})), l_1,\dots, l_n)$ and  there exists a substitution $\theta$ such that for some $s \in symbols(d)\setminus T_{RV}$ it holds that $h\sim d' \lpif b'_1, \dots, b'_{k}\in \dcpprogram$, $\theta = mgu(s,h)$, then:
		\begin{align*}
			{\text{\bf \rrvtwo:}} \quad 
			&(rv(x, d, (b_1, \dots, b_{m})), l_1, \dots, l_n) \\
			&~~~\vdash (b'_1, \dots, b'_{k}, rv(h, d', (b'_1, \dots, b'_{k})), rv(x, d, (b_1, \dots, b_{m})), l_1, \dots, l_n)\theta
			\\
			{\text{\bf \trvtwo:}} \quad &\tau =  (\emptyset, \theta)
		\end{align*}
		
		\item[\bf \crvone]  If the goal is $(rv(x, d, (b_1, \dots, b_{m})), l_1,\dots, l_n)$ and   $symbols(d)\subseteq T_{RV}$ then we further  distinguish two cases.
		$\text{\bf R6a}$ applies if $l_1 = rv(y, d_y, (b'_1, \dots, b'_k))$ and $x\in symbols(d_y)$. $\text{\bf R6b}$ applies in all other cases.  The tag is identical for both.
		\begin{align*}
			{\text{\bf \rrvonea:}} \quad
			&x_{new} = \mathrm{createRVname}(x,(b_1,\dots, b_m)) \\
			& \mathrm{INSERT}(T_{RV}, x_{new}) \\
			&\phi = \{ x/ x_{new} \} \\
			&(rv(x, d, (b_1, \dots, b_{m})), rv(y, d_y, (b'_1, \dots, b'_k)) , l_2, \dots, l_n) \\
			&~~~    \vdash (rv(y, d_y, (b_1, \dots, b_{m}, b'_1, \dots, b'_k) , l_2, \dots, l_n)\phi
			\\
			{\text{\bf \rrvoneb:}} \quad
			&x_{new} = \mathrm{createRVname}(x,(b_1,\dots, b_m)) \\
			& \mathrm{INSERT}(T_{RV}, x_{new}) \\
			&\phi = \{ x/ x_{new} \} \\
			&(rv(x, d, (b_1, \dots, b_{m})), l_1, \dots, l_n) \vdash (l_1, \dots, l_n)\phi
			\\
			{\text{\bf \trvone:}} \quad &\tau =  (\{x\sim d \}, \{x\twoheadleftarrow (x_{new},(b_1,\dots, b_m))\})
		\end{align*}
	\end{enumerate}
	% AK: for R6a, note that: R5 always inserts the parent rv/3-atom to the left of the child rv/3-atom, so if we need to propagate context a generation down, it is always to the goal that directly follows. However, not all pairs of neighboring rv/3-atoms are parent and child (we could also get an unrelated rv/3 from the last subgoal of the parent's context directly before the parent's rv/3), and we thus also need to check the child's distribution mentions the parent. 
\end{definition}
Intuitively, the first two rules (\rposlit and \rneglit) apply SLD resolution just as for \problogsty, and record both the rule and substitution used in the tag, while the remaining four rules are responsible for collecting information related to random variables and their distributions. These latter rules use the `$\mathrm{symbols}$' function to extract the interpreted random variable terms from the current subgoal, and compare that set against the hash table storing known random variables to distinguish between cases where all interpretations are already available and cases where the interpretation of some symbol still needs to be determined. Rules \rcompone and \rcomptwo are concerned with comparison literals, which can simply be dropped from the goal once all their random variables are resolved (\rcomptwo), and otherwise are re-considered after resolving the body of a relevant distributional clause and inserting the corresponding random variable via the auxiliary predicate (\rcompone). The last two rules ensure that the parents of a relevant random variable are included recursively using the same principle (\rrvtwo), and that all random variables are recorded in the hash table once their ancestors and context have been fully evaluated (\rrvonea and \rrvoneb). Rules \rcompone--\rrvtwo only record their substitutions in the tag, whereas \rrvonea and \rrvoneb record a new distributional fact as well as contextual rewrite information for its random variable term.  Additionally, \rrvonea propagates the parent random variable's context into the context of the child. 

%Given a query or literal to be proven, the resolution rules in Definition~\ref{def:resolution_rules} allow us to construct a resolution tree from a specific non-ground program with respect to the query. 
%The conversion algorithm uses these rules to construct a resolution tree for each query or evidence atom, using a shared hash map for the random variables.



\begin{example}[Derivations and tag sequences]
	\label{ex:resolution_tree}
	%Consider the AD-free program obtained in Example~\ref{ex:eliminating_pf}. 
	%We can construct an SLDNF-DC tree using the resolution rules from Definition~\ref{def:resolution_rules}. We depict the resolution tree in
	Figures~\ref{fig:sld_tree_left} and~\ref{fig:sld_tree_right} graphically depict the derivations obtained by applying the resolution rules from Definition~\ref{def:resolution_rules} to the AD-free program in Example~\ref{ex:eliminating_pf} as a resolution tree, where nodes represent goals and edges are labeled with the context number of the applied rule. We represent empty context conjunctions resulting from distributional facts using the term \probloginline{true} in \probloginline{rv/3}-atoms and labels. 
	
	The tag sequence for the leftmost derivation is\\
	$(\{$\probloginline{works(N):-cool(N)}$\}, \emptyset)$, \\
	$(\{$\probloginline{cool(1):-rv_cool(1)=:=1}$\}, \{N/1\})$,\\
	$(\emptyset, \emptyset)$,\\
	$(\{$\probloginline{rv_cool(1)~flip(0.99)}$\}, \{$\probloginline{rv_cool(1)}$\twoheadleftarrow ($\probloginline{rv_cool_1_1}, \probloginline{true}$)\})$,\\
	$(\emptyset, \emptyset)$.
	
	The tag sequence for the derivation in the middle is\\
	$(\{$\probloginline{works(N):-temp(N)<25.0}$\}, \emptyset)$, \\
	$(\emptyset, \{N/1\})$,\\
	$(\{$\probloginline{hot :- rv_hot =:=1}$\}, \emptyset)$, \\
	$(\emptyset, \emptyset)$,\\
	$(\{$\probloginline{rv_hot~flip(0.2)}$\}, \{$\probloginline{rv_hot}$\twoheadleftarrow ($\probloginline{rv_hot_1}, \probloginline{true}$)\})$,\\
	$(\emptyset, \emptyset)$,\\
	$(\{$\probloginline{temp(1)~normal(27,5)}$\}, \{$\probloginline{temp(1)}$\twoheadleftarrow ($\probloginline{temp_1_1}, \probloginline{hot}$)\})$,\\
	$(\emptyset, \emptyset)$.
	
	The tag sequence for the rightmost derivation is\\
	$(\{$\probloginline{works(N):-temp(N)<25.0}$\}, \emptyset)$, \\
	$(\emptyset, \{N/1\})$,\\
	$(\{$\probloginline{hot :- rv_hot =:=1}$\}, \emptyset)$, \\
	$(\emptyset, \emptyset)$,\\
	$(\{$\probloginline{rv_hot~flip(0.2)}$\}, \{$\probloginline{rv_hot}$\twoheadleftarrow ($\probloginline{rv_hot_1}, \probloginline{true}$)\})$,\\
	$(\emptyset, \emptyset)$,\\
	$(\{$\probloginline{temp(1)~normal(20,5)}$\}, \{$\probloginline{temp(1)}$\twoheadleftarrow ($\probloginline{temp_1_2}, \probloginline{not hot}$)\})$,\\
	$(\emptyset, \emptyset)$.
	
	
	
	\begin{figure}[h]
		\begin{center}
			\begin{tikzpicture}
				{\small
					\node {(\probloginline{works(N)})} [sibling distance = 0.5\linewidth]{
						child [] { node {(\probloginline{cool(N)}) }
							child [] { node {(\probloginline{rv_cool(1)=:=1})}
								child [] { node {(\probloginline{rv(rv_cool(1),flip(0.99),true)}, \probloginline{rv_cool(1)=:=1})}
									child [] { node  {( \probloginline{rv_cool_1_1=:=1})}
										child [] {node {()} edge from parent [] node [left] { \scriptsize \ccomptwo } }
										edge from parent [] node [left] { \scriptsize \crvone }
									}
									edge from parent [] node [left] { \scriptsize \ccompone }
								}
								edge from parent [] node [left] { \scriptsize \cposlit }
							}
							edge from parent [] node [left,above] { \scriptsize \cposlit }
						}
						child [] { node {(\probloginline{temp(N)<25.0})} [sibling distance = 0.4\linewidth]
							child [] { node {} edge from parent [dashed] edge from parent [] node [left, above] { \scriptsize \ccompone   } }
							child [align=center] { node {} edge from parent [dashed] edge from parent [] node [right, above] { \scriptsize \ccompone  } }
							edge from parent [] node [right, above] {  \scriptsize \cposlit  }
						}
					};
				}
			\end{tikzpicture}
		\end{center}
		\caption{Left subtree of the resolution tree for the program in Example~\ref{ex:eliminating_pf} with respect to \probloginline{query(works(N))}; dashed lines continue in Figure~\ref{fig:sld_tree_right}.}
		\label{fig:sld_tree_left}
	\end{figure}
	
	
	
	\begin{figure}
		\begin{center}
			\begin{tikzpicture}
				{\small
					
					\node {} [sibling distance = 0.55\linewidth]
					child [] {node {(\probloginline{temp(N)<25.0})} edge from parent [dashed,level distance = 2.5cm] 
						child [align=center] {node { \probloginline{(hot},\\\probloginline{rv(temp(1),normal(27,5),hot)},\\ \probloginline{temp(1)<25.0}) } edge from parent [solid] 
							child [align=center] { node {(\probloginline{rv_hot=:=1},\\ \probloginline{rv(temp(1),normal(27,5),hot)},\\ \probloginline{temp(1)<25.0})}
								child [align=center] { node {(\probloginline{rv(rv_hot, flip(0.2), true) },\\  \probloginline{rv_hot=:=1}, \\ \probloginline{rv(temp(1),normal(27,5),hot)}, \\ \probloginline{temp(1)<25.0}) }
									child [align=center] { node {( \probloginline{rv_hot_1=:=1}, \\ \probloginline{rv(temp(1),normal(27,5),hot)}, \\ \probloginline{temp(1)<25.0}) }
										child [align=center, ] { node {( \probloginline{rv(temp(1),normal(27,5),hot)}, \\\probloginline{temp(1)<25.0} ) }
											child [ level distance = 1.5cm] { node {(\probloginline{temp_1_1<25.0})}
												child { node {()}  edge from parent [] node [left,] {  \scriptsize \ccomptwo  } }
												edge from parent [] node [left,] {\scriptsize \crvone } 
											}
											edge from parent [] node [left,] { \scriptsize \ccomptwo }
										}
										edge from parent [] node [left,] { \scriptsize \crvone }
									}
									edge from parent [] node [left,] { \scriptsize \ccompone }
								}
								edge from parent [] node [left,] { \scriptsize \cposlit }
							}
							edge from parent [] node [left,above] { \scriptsize \ccompone }
						}
						child [align=center] {node { (\probloginline{not hot},\\\probloginline{rv(temp(1),normal(20,5),not hot)},\\ \probloginline{temp(1)<25.0} } edge from parent [solid] 
							child [align=center] { node {(\probloginline{rv_hot=:=1},\\ \probloginline{rv(temp(1),normal(20,5),not hot)},\\ \probloginline{temp(1)<25.0})}
								child [align=center] { node {(\probloginline{rv(rv_hot, flip(0.2), true) }, \\ \probloginline{rv_hot=:=1}, \\ \probloginline{rv(temp(1),normal(20,5),not hot)}, \\ \probloginline{temp(1)<25.0}) } 
									child [align=center] { node {( \probloginline{rv_hot_1=:=1}, \\ \probloginline{rv(temp(1),normal(20,5),not hot)},\\\probloginline{temp(1)<25.0}) }
										child [align=center] { node {( \probloginline{rv(temp(1),normal(20,5),not hot)}, \\\probloginline{temp(1)<25.0}) }
											child [ level distance = 1.5cm] { node {(\probloginline{temp_1_2<25.0})}
												child { node {()}  edge from parent [] node [right,] { \scriptsize \ccomptwo } }
												edge from parent [] node [right,]  { \scriptsize \crvone  }
											}
											edge from parent [] node [right]  { \scriptsize \ccomptwo  }
										}
										edge from parent [] node [right]  { \scriptsize \crvone  }
									}
									edge from parent [] node [right] { \scriptsize \ccompone  }
								}
								edge from parent [] node [right] { \scriptsize \cneglit }
							}
							edge from parent [] node [right,above] { \scriptsize \ccompone}
						}
						edge from parent [] node [right] {\scriptsize \cposlit }
					}
					;
				}
			\end{tikzpicture}
		\end{center}
		\caption{Right subtree of the resolution tree for the program in Example~\ref{ex:eliminating_pf} with respect to \probloginline{query(works(N))}; dashed line continued from Figure~\ref{fig:sld_tree_left}}\label{fig:sld_tree_right}
	\end{figure}
\end{example}


\newpage
\clearpage

%The resolution tree functions as an intermediate representation for obtaining the relevant ground program. Defining a tagging function for each edge in the resolution tree will allow us to specify an algorithms that maps a path in a tree (also called derivation) to its corresponding relevant ground program.

%\begin{definition}[Edge Tagging in  Resolution Tree]
%\label{def:sld_edge_tagging_rules}
%Let $\mathcal{T}$ be a resolution tree. We tag each edge in the tree with a tuple $\tau=(\tau_r,\tau_s)$, where $\tau_r$ represents a set of logic rules and $\tau_s$ a substitution. The tag of an edge of the tree $\mathcal{T}$ depends on the condition ({\bf C1-C6}) that held when the edge was created.
%We now define the six tagging rules for edges in a resolution tree in function of the conditions that apply.



%\begin{enumerate}
%    \item[\cposlit] If the goal is $(l_1, l_2, \dots, l_n)$ and if  $\exists \theta$ such that  $h \lpif b_1, \dots, b_n \in \dcpprogram$, $\theta  = mgu(l_1, h)$ then:
%   \begin{align*}
	%      {\text{\bf \tposlit:}} \quad \tau = (\{ h \lpif b_1, \dots, b_n \}, \theta)
	% \end{align*}

% \item[\bf \cneglit]  If th goal is $(not(l_1), l_2, \dots, l_n)$ and if $\exists \theta$ such that  $h \lpif b_1, \dots, b_n \in \dcpprogram$, $\theta  {=} mgu(l_1, h)$ then:
%\begin{align*}
%   {\text{\bf \tneglit:}} \quad \tau = (\{ h \lpif b_1, \dots, b_n \}, \theta)
%\end{align*}

%\item[\ccompone]  If the goal is $( l_{comp}, l_1, \dots, l_n )$ and if $l_{comp}$ is a comparison atom (or its negation) and if there exists a substitution $\theta$ such that for an arbitrary symbol $s \in symbols(l_{comp})\setminus keys(T_{RV})$ it holds that $h\sim d\lpif b_1, \dots, b_n\in \dcpprogram$, with $\theta = mgu(s,h)$, then:
%\begin{align*}
%   {\text{\bf \tcompone:}} \quad \tau = (\emptyset, \theta)\\
%\end{align*}

%\item[\bf \ccomptwo]  If the goal is $( l_{comp}, l_1, \dots, l_n )$  and if $l_{comp}$ is a comparison atom (or its negation) and if $symbols(l_{comp})\subseteq keys(T_{RV})$ then:
%\begin{align*}
%   {\text{\bf \tcomptwo:}} \quad \tau = (\emptyset, \emptyset)
%\end{align*}

%  \item[\bf \crvtwo]  If the goal is $(rv(x, d, (b_1, \dots, b_{n})), l_1,\dots, l_m)$ and if there exists a substitution $\theta$ such that for an arbitrary symbol $s \in symbols(d)\setminus keys(T_{RV})$ it holds that $h\sim d^h \lpif b^h_1, \dots, b^h_{n^h}\in \dcpprogram$, $\theta = mgu(s,h)$, then:
%  \begin{align*}
	%      {\text{\bf \trvtwo:}} \quad \tau =  (\emptyset, \theta)\\
	%  \end{align*}

%  \item[\bf \crvone]  If the goal is $(rv(x, d, (b_1, \dots, b_{n})), l_1,\dots, l_m)$ and if  $symbols(d)\subseteq keys(T_{RV})$ then:
%  \begin{align*}
	%          {\text{\bf \trvone:}} \quad \tau =  (\{x\sim d \}, \{ x/ x_{b_1,\dots,b_n} \})
	%   \end{align*}
%\end{enumerate}
%\end{definition}

%\begin{definition}[Derivation]
%Let $\dcpprogram$ be a \dcproblogsty program, and $Q$ a query atom. We call a path in the   resolution tree of $Q$ for \dcpprogram a derivation of $Q$. A derivation consists of a set of edges $\{e^0,\dots, e^N  \}$.
%Edges in a derivation are ordered, starting at the root.
%We call a derivation tagged if the rules in Definition~\ref{def:sld_edge_tagging_rules} have been applied.
%\end{definition} 

In order to define the ground program corresponding to a tag sequence, we first need to define the rewrite operation introduced by \trvone.
\begin{definition}[RV substitution]\label{def:context-substitution}
	Let $\theta=\{x\twoheadleftarrow (v, (b_1, \dots ,b_m))\}$ be a random variable substitution. Then,
	\begin{align*}
		(h \lpif l_1\dots, l_n)\theta &= (h\lpif b_1, \dots, b_m,l_1, \dots, l_n)\{x/v\}, &\text{~if~x~is~interpreted~in~some~}l_i\\
		s\theta &= s\{x/v\}, &\text{~otherwise}
	\end{align*}
	where we overload regular substitution notation for random variable terms, \ie, $c\{x/v\}$ is $c$ with every occurrence of $x$ replaced by $v$.
\end{definition}
That is, we add the  context to the bodies of all rules that interpret $x$, \ie, whose body contains a comparison literal involving $x$, and replace all occurrences of $x$ by the new variable $v$.
%replace the old random variable term $x$ by the context-dependent random variable $v$ in all statements,  and  
% we do not need to substitute parents in distribution terms, as (1) R5 ensures that R6 is applied to all parents before it is applied to the child, (2) the moment R6 is applied to a parent, there is a rv/3 atom for the child in the rest of the goal, and R6 substitutes the new parent name there, thus (3) by the time the T6 tag of the child is created, the distribution contains the parent's new name
Algorithm~\ref{alg:tags2gp} uses this rewrite operation, together with regular substitutions included in other types of tags, to extract a relevant ground program from a tag sequence. 


\begin{algorithm}[h!]
	\SetKwInput{KwOutput}{Output}              
	\DontPrintSemicolon
	\KwInput{Derivation tag sequence $S=((P_1,\theta_1),\ldots,(P_N,\theta_N))$}
	\KwOutput{Corresponding Relevant Ground Program}
	
	
	$\dcpprogram_S \leftarrow \emptyset$\;
	\For{$i \in \{0,\dots, N\}$  }{
		$\dcpprogram_S \leftarrow \dcpprogram_S \cup P_i$\;
		$\dcpprogram_S \leftarrow  \dcpprogram_S\theta_i$
	}
	
	\Return $\dcpprogram_S$
	\caption{Relevant Ground Program for a Derivation Tag Sequence}
	\label{alg:tags2gp}
\end{algorithm}
%Note that applying a tag's substitutions directly after adding its rules is crucial, as several tags may substitute the same random variable terms

%\begin{algorithm}[h!]
% \SetKwFor{For}{for (}{}
%
%\newlength\mylen
%\newcommand\myinput[1]{%
	%  \settowidth\mylen{\KwIn{}}%
	%  \setlength\hangindent{\mylen}%
	%  \hspace*{\mylen}#1\\}
%
%
%\SetKwInput{KwOutput}{output}              
%\DontPrintSemicolon
%\KwInput{Tagged derivation $\mathcal{R}$ (of depth $N$)}
%\myinput{Table $tags$ storing the tags of the edges in $\mathcal{R}$}
%\KwOutput{Relevant Ground Program corresponding to $\mathcal{R}$}
%
%
%$RelGroundProgram \leftarrow \emptyset$\;
%\For{$i \in \{0,\dots, N\}$  }{
	%    $\tau_r^i, \tau_s^i \leftarrow tags[i] $\;
	%    $RelGroundProgram \leftarrow RelGroundProgram \cup \tau_r^i$\;
	%    $RelGroundProgram \leftarrow  RelGroundProgram/\tau_s^i$
	%}
%
%\Return $RelGroundProg$
%\caption{Relevant Ground Program with Respect to a Derivation}
%\label{alg:tags2gp}
%\end{algorithm}

%\begin{definition}[Relevant Ground Program]
%Let \dcpprogram be an AD-free program, $Q$ a query atom, and  $\mathcal{T}$ the resolution tree obtained from applying the resolution rules in Definition~\ref{def:resolution_rules} to  \dcpprogram and $Q$, where all derivations have been tagged. We denote these derivations by  $\{\mathcal{R}_0, \dots,  \mathcal{R}_M \}$  and their ground programs as obtained from Algorithm~\ref{alg:tags2gp} by $\dcpprogram
%_g^{\mathcal{R}} =\{\dcpprogram_g^{\mathcal{R}_0}, \dots, \dcpprogram_g^{\mathcal{R}_M}  \}$. The relevant ground program of \dcpprogram with respect to the atom of interest $Q$, denoted by $\dcpprogram_g^Q$, is then given by: $ \dcpprogram_g^Q = \bigcup_{i\in \{0,\dots,M  \}} \dcpprogram_g^{\mathcal{R}_i}  $.
%\end{definition}

\begin{example}
	Algorithm~\ref{alg:tags2gp} constructs the following program for the rightmost tagging sequence in the example:
	\begin{problog*}{linenos}
works(1) :- not hot, temp_1_2<25.0.
hot :- true, rv_hot_1 =:= 1.
rv_hot_1~flip(0.2).
temp_1_2~normal(27,5).
	\end{problog*}
	Note that all random variable terms have been replaced by the new random variables, and appropriate contexts added to the rules interpreting them. 
\end{example}

\begin{definition}[Relevant ground program for an atom]
	Let \dcpprogram be an AD-free program, $A$ an atom and $\mathcal{S}$ be the set of all derivation tag sequences for $A$ in \dcpprogram. The \emph{relevant ground program with respect to $A$}, denoted by $\dcpprogram_g^A$, is given by $\dcpprogram_g^A = \bigcup_{S\in\mathcal{S}}\dcpprogram_S$.
\end{definition}

\begin{definition}[Relevant ground program]
	Let \dcpprogram be an AD-free program, $\queryset$ a set of queries of interest, and  $\evidenceset=e$ the evidence. The \emph{relevant ground program}  is $\dcpprogram_g = \bigcup_{A\in (\queryset\cup\evidenceset)}\dcpprogram_g^A$.
\end{definition}


\begin{example}[Relevant Ground Program] 
	%Applying the edge tagging and the definition of a relevant ground program  to the resolution tree in Example~\ref{ex:resolution_tree} results in the following ground program.
	The full ground program obtained from the derivations in Example~\ref{ex:resolution_tree} is
	\begin{problog*}{linenos}
rv_hot_1 ~ flip(0.2).
hot :- true, rv_hot_1=:=1.
rv_cool_1_1 ~ flip(0.99).
cool(1) :- true, rv_cool_1_1=:=1.

temp_1_1 ~ normal(27,5).
temp_1_2 ~ normal(20,5).

works(1):- cool(1).
works(1):- hot, temp_1_1<25.0.
works(1):- not hot, temp_1_2<25.0.
	\end{problog*}
	Note that lines 1 and 2 are generated by both the middle and the rightmost derivation, while all other statements stem from a single derivation in this example.	
	%Note how the `$\mathrm{createRVname}$' function created unique names for the random variables in the program, which are then also inserted into the arguments of the comparison terms. For instance \probloginline{temp_1_2} in the the comparison \probloginline{temp_1_2<25.0}. 
\end{example}


In order to implement an efficient resolving algorithm, one ought to avoid processing the same atom twice. This is usually done through tabling, which also avoids going into an infinite loop when cyclical rules are present in the (logic part of the) program. 
%Note also that if we had had multiple query atoms, instead of a single one, our approach would not change dramatically. The main difference would lie in having a multi-rooted resolution tree instead of a single root tree.
Note also that while the relevant ground program computed by this approach does not contain any rules that are disconnected from the reasoning process related to queries and evidence, it is not necessarily the smallest such program. It may for instance include rules whose bodies are logically inconsistent because of added conjunctions of contexts, or invalidated by the actual values of the evidence. 

==> files_excluded/types.tex <==
\section{Typing \dcproblogsty}
\label{app:types}


\subsection{Type System}\label{sec:type_system}

A distinctive property of system predicates, which are implemented using an external engine, is their mandatory type signature.
An instance of such system predicates are comparison predicates.
Consider for example the comparison (\probloginline{x>20}).
The right-hand side is an integer and if the \probloginline{x} denotes a numeric random variable we have a well-typed comparison predicate inducing a measurable set.
Consider for the sake of contrast also the comparison predicate (\probloginline{a>2}), where \probloginline{a} is an atomic formula. This comparison predicate is ill-typed as atomic formulas cannot be compared to (integer) numbers. In other words, the external engine, which implements the system predicates does not know how to commensurate an atomic formula and a number.
A type system lets us specify which combinations of types are allowed as arguments of comparison predicates, \ie which comparisons encode measurable sets and are supported by the external engine.



\begin{samepage}
\begin{definition}\label{def:type_system}
	The \dcproblogsty type system is a hierarchical type system with each type being a disjoint union of its subtypes.
	The base type for \dcproblogsty is the \type{Term} type. We subtype terms with a \type{Distribution} type and a \type{Symbol} type. 
    A diagrammatic overview of the \dcproblogsty type system is given in Figure~\ref{fig:type_system}.
	\begin{enumerate}
		\item[] \type{Term} 
		\begin{enumerate}
			\item[1.] \type{Distribution}
			\begin{itemize}
				\item \type{NumericD}
				\item \type{CategorialD}
			\end{itemize}
			\item[2.] \type{Symbol}
			\begin{itemize}		
				\item \type{RandomSymbol}
				\begin{itemize}
				    \item \type{NumericRV}
				    \item \type{CategoricalRV}
				\end{itemize}
				\item \type{DeterministicSymbol}
				\begin{itemize}
				    \item \type{Number}
				    \item \type{Atom}
				\end{itemize}	
			\end{itemize}
		\end{enumerate}
	\end{enumerate}
\end{definition}
\end{samepage}



\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\linewidth]{../figures/type_hierarchy_reduced.pdf}
	\end{center}
	\caption[Diagrammatic representation of the hierarchical \dcproblogsty type system.]{Diagrammatic representation of the hierarchical \dcproblogsty type system.}
	\label{fig:type_system}
\end{figure}




\begin{definition}[\type{Distribution}]
	Terms of type \type{Distribution} are constructed by using a reserved random function symbol and applying it to a (possible empty) tuple of input arguments, which maps the input tuple to a distribution term.
	Distribution terms are only allowed to be invoked as a second argument to the reserved distribution predicate \probloginline{~}\lstinline[columns=fixed]|/2|.
	This also means that random function symbols are only used there as well. 
% 	\dcproblogsty subtypes the \type{Distribution} type into \type{NumericD} and \type{CategoricalD}.
% 	\type{DiscreteD}, \type{ContinuousD}, and \type{MixtureD} types.
\end{definition}

\type{Distribution} terms determine the probability distribution according to which a random variable is distributed.
\probloginline{poisson(6)} and \probloginline{normal(20,5)} are for instance of type \type{NumericD}.

% Note that distributions of type \type{ContinuousD} denote {\em absolutely continuous} probability distributions\footnote{\dcproblogsty does not support {\em singular continuous} probability distributions such as the Cantor distribution.}. \ak{would be nice to have a hint on why this restriction is there} We give an example of a distribution of type \type{MixtureD} in Example~\ref{ex:indian_gpa_function}.
%\begin{example} \probloginline{mixed} is a random variables that is a mixture of a continuous part (the truncated normal between $0$ and $4$ with mean $3$ and standard deviation $1$) and a discrete part. 
%\begin{problog}
%mixted~Mix((0.998,TruncNormal(3,1,0,4)),(0.001,4),(0.001,4))
%\end{problog}
%\end{example}

%For and example, see Example~\ref{example:dcproblog_poisson_population}: we have the random function symbol \probloginline{poisson}\lstinline[columns=fixed]{/1}, apply it to the input tuple \probloginline{(6)}, and obtain a term of type \type{Distribution}.

\begin{definition}[\type{Symbol}]
  \type{Symbol} terms are the building blocks of the discrete structure that makes up a logic program and as such determine also the deterministic system of a probabilistic logic program. Beyond the reserved syntax, which is used to define the distribution terms, the user is free to use any identifier (following \prologsty conventions) to declare \type{Symbol} terms (this includes standard \prologsty terms such as lists).  
\end{definition}


%The subtyping of the \type{Symbol} type (shown in Figure~\ref{fig:type_system}) follows the convention given in~\citep[Chapter 9]{sterling1994art}.

% \begin{definition}[\type{Arithmetic}]
% 	Terms of type \type{Symbol} for which arithmetic operations are defined are of type \type{Arithmetic}. \type{Arithmetic} terms can be used as second argument to the builtin \probloginline{is}\lstinline[columns=fixed]|/2| functor. \type{Arithmetic} terms are subtyped with \type{RandomVariable} terms and \type{Number} terms.
%	\ak{Def 6.3 Arithmetic terms: if (as stated in def 6.1) each type is the disjoint union of its subtypes, that means that "arithmetic" is made up exclusively of numbers and RVs, \ie, terms like 3-2 or min(x,5) for a RV x are not allowed, whereas the first two sentences of def 6.3 suggests they might be allowed (only having numbers and RVs directly on the rhs of is/2 seems quite boring...). Which is it?
%		Related to this, defs 6.8 and 6.10 talk about RVs and Numbers, why not simply "arithmetic"?}
% \end{definition}


\begin{definition}[\type{RandomSymbol}] \label{def:random_variable}
	\type{RandomSymbol} terms are named by the programmer using distributional facts with the binary infix predicate \probloginline{~}\lstinline[columns=fixed]|/2| and inherit their subtype from the distribution term. All random variables present in a \dcproblogsty program  explicitly named.
\end{definition}

Examples of terms of type \type{RandomSymbol} would be \probloginline{temperature} and \probloginline{n_people} in Examples~\ref{example:dcproblog_machine} and~\ref{example:dcproblog_poisson_population}, where we declared the random variables through distributional facts: 
\begin{problog}
temperature ~ normal(20,5).
n_people ~ poisson(6).
\end{problog}
As mentioned in Defintion~\ref{def:random_variable}, \type{RandomSymbol} terms inherit their type from the associated \type{Distribution} term, \eg a \type{NumericD} term induces a random variable term of type \type{NumericRV}.

Note that not all probabilistic programming languages enforce the naming of random variables. In the functional probabilistic programming language \anglicansty~\citep{wood2014approach}, for instance, the user can declare anonymous random variables, much like anonymous functions, \ie \textlambda-functions. 
\ak{Discussion of named/unnamed between Defs 6.4 and 6.5: would be nice to have a brief hint on why you made that choice} \pedro{usually in logic programming everything is global. an unamed random variable would mean that it is only available locally. we could allow that, I guess but would have to introduce new syntax. moreover, internally we would give the unnamed random variable a name anyway.}

\begin{definition}[\type{Atom}]
	An atom is of the form \probloginline{p(t@$_1$@,@\dots @, t@$_n$@ )} where \dcplpinline{p} is a predicate with arity $n$ and the \probloginline{t@$_i$@} are \type{Symbol} terms. Functors used to construct \type{Atom} terms must not clash with the builtin predicates and reserved functors used to declare \type{Distribution} terms.
% 	Terms of type \type{Atom} constitute the building blocks of the discrete structure of a probabilistic logic program.
\end{definition}

Examples of \type{Atom} terms would be \probloginline{foo} or \probloginline{bar(foo,42)}. The latter is constructed using the predicate \lstinline{bar/2} and the tuple of \type{Symbol} terms \probloginline{(foo,42)}. \probloginline{foo} is of type \type{Atom} and \probloginline{42} is a \type{Number} term.

\begin{definition}[\type{Number}] Terms of type \type{Number} are used to express numerical data types such as integers and real numbers.	
\end{definition}

\paragraph{Strongly Typed \prologsty}

While \prologsty is traditionally not strongly/statically typed, there have been efforts to extend \prologsty with such a type system. Arguably, the most interesting effort is presented in~\citep{Schrijvers2008TowardsTP}, where the authors develop the idea of partially typing a \prologsty program, \ie typing is optional and untyped code is interpreted instead of compiled. Introducing predicates with strongly typed signatures can be regarded as adding predicates with a specific meaning to the \prologsty implementation but the {\em `evaluation'} of these predicates still takes place within \prologsty.
Our efforts of introducing a type system for system predicates within a probabilistic programming context are orthogonal and complimentary to the efforts of~\citet{Schrijvers2008TowardsTP}.


% \dcproblogsty's type system refines the one of DC-PLP to instantiate a conrete version of the abstract language.  Specifically, we have the following refinements:
% \begin{enumerate}
%     \item distribution functors are further partitioned into \emph{discrete distribution functors}. \emph{continuous distribution functors} and \emph{mixture distribution functors}
%     \item arithmetic functors are further partitioned into \emph{operation functors} and \emph{number functors}, with the latter in turn partitioned into \emph{integers} and \emph{floats} \todo{do we have / want a complete list of operations? should we at least give some examples?}
%     \item we use Boolean query functors 	$\bowtie=\{ \text{\probloginline{=:=}}, \text{\probloginline{=\=}}, \text{\probloginline{<}}, \text{\probloginline{>}},  \text{\probloginline{=<}}, \text{\probloginline{>=}} \}$
% 	in infix notation (and lift them to predicate level as discussed before)
% \end{enumerate}

% \ak{I don't think we need to sub-type random variable functors here, as rv terms inherit the \emph{output} type of the distribution only, which should be integer, float etc, not "discrete distribution"}
























\subsection{External Engine}\label{sec:external_engine}

In the previous subsection we have introduced an abstract type system.
Abstract types describe the structure/hierarchy of a type system and cannot be instantiated. Concrete types, which are subtypes of abstract types are used for instantiations. This means that abstract types relate collections of concrete types, \ie implementations, to each other. For example, the \type{Integer} \probloginline{3} could be instantiated as an \type{Int32} or also an \type{Int64}, which are both concrete types. The choice taken depends on the external engine used to evaluate arithmetic expressions. 

The only condition that we necessitate for an implementation of \dcproblogsty is that the external engine provides concrete types for the abstract types. Additionally, a practical external engine should also implement operations on these types. For example, an engine should be able to multiply a floating point value and an integer value: (\probloginline{3.12*2}). The type for floating points could be dubbed \type{Float32} and would be a concrete type subtyped from the abstract type \type{Real}. The type of the integer value could be \type{Int32} subtyped from \type{Integer}. The return type could then again be \type{Float32}.



\begin{example}\label{example:julia_addition}
We show two functions that perform addition of numbers but with different types. These different number could be invoked on either side of a comparison predicate, \eg (\probloginline{1<3+5} ) or (\probloginline{1<3+5.0} ). We write these functions using Julia like syntax~\citep{bezanson2017julia}. 
\begin{samepage}

\begin{minted}[
    breaklines,
    escapeinside=||,
    mathescape=true, 
    linenos,
    xleftmargin=20pt, 
    % numbersep=3pt, 
    % gobble=2, 
    % framesep=2mm
]{julia}
function +(a::Int32, b::Int32)::Int32
    return int32_addition(a,b)
end;
\end{minted}

\end{samepage}


\begin{samepage}
\begin{minted}[
    breaklines,
    escapeinside=||,
    mathescape=true, 
    linenos,
    xleftmargin=20pt, 
    % numbersep=3pt, 
    % gobble=2, 
    % framesep=2mm
]{julia}
function +(a::Int32, b::Float32)::Float32
    float_a = convert(Float32, a)
    return float32_addition(float_a,b)
end;
\end{minted}

\end{samepage}
\end{example}

The programming paradigm followed in Example~\ref{example:julia_addition} is called {\em multiple dispatch} \citep{keene1989object,castagna1995calculus,bezanson2017julia}.
Multiple dispatching is the process of dynamically selecting at run time a specific implementation of a function based on the types of the arguments.
Functions with the same functor but a different type signature are called multimethods.

We implement probability distributions using the external engine. As such, the corresponding random funtions symbols are necessarily typed. We recede again to multiple dispatch to implement probability distributions.
Consider, for instance, the declaration of the normal distribution in Example~\ref{example:dcproblog_machine}.
The definition of the function is the following:
$$ \text{\probloginline{normal}}: \type{Number} \times \type{Number} \rightarrow \type{ContinuousD}$$
However, the arguments of a normal distribution (its mean and standard deviation) might as well be random variables themselves.
Multiple dispatching then allows us to {\em overload} the \probloginline{normal} function symbol by using arguments of a different type\footnote{For simplicity we omit that the standard deviation has to be a strictly positive (real) number, which can be enforced by extending the type system.}:
\begin{align*}
	\text{\probloginline{normal}}&: \type{NumericRV} \times \type{Number} \rightarrow \type{ContinuousD} \\
	\text{\probloginline{normal}}&: \type{Number} \times \type{NumericRV} \rightarrow \type{ContinuousD} \\
	\text{\probloginline{normal}}&: \type{NumericRV} \times \type{NumericRV} \rightarrow \type{ContinuousD}
\end{align*}

Reusing the idea of multimethods in the context of probabilistic logic programming with random function symbols results in a simple and neat syntax.
The exact implementation of these random function symbols is left to to the actual implementation of the language by providing an external engine capable of performing adequate arithmetic evaluations.

Currently, \dcproblogsys, our implementation of \dcproblogsty, does only emulate multimethods. This is due to the fact that the \dcproblogsys is written in Python, which does not follow the multiple dispatch programming paradigm. The emulation of multimethods is performed by using the \verb|isinstance| function in Python, which checks whether an object is of a certain type or not. This allows us to branch on the type of the arguments passed to a function and call different implementation given differently typed arguments.

An advantage of decoupling the deterministic system from the independent choices and implementing probability distribution using an external engine is that we can a single language with two different external engines, which might perform probabilstic inference differently.
\dcproblogsys, for instance, provides an interface to two different external engines. The first one uses \pyrosty~\citep{bingham2019pyro}, a probabilistic programming language built on top of the PyTorch~\citep{paszke2019pytorch} deep learning framework.
The second option uses the probabilistic programming language PSI~\citep{gehr2016psi}. PSI is a computer probabilistic computer algebra system. The main difference between the two different external engines becomes apparent when performing inference. The first one performs approximate inference while the second one exact inference. We will discuss this in more detail in Section~\ref{sec:inference}.


==> files_excluded/wmi.tex <==

\section{Weighted Model Integration}
\label{app:wmi}

Standard weighted model counting only supports discrete probability distributions. To repair this omission, WMC has recently been extended towards weighted model integration (WMI)~\citep{belle2015probabilistic}, supporting additionally continuous variables. Contrary to WMC, which is formulated using weighted propositional logic formulas, WMI uses so-called {\em weighted  satisfiability modulo theory} (SMT) formulas. We refer the reader to~\citep{barrett2009handbook} for a treatise on (unweighted) SMT formulas.

\begin{example}\label{example:wmi_intro}
    Consider the theory $\mathtt{broken}$
	\begin{align}
	\textstyle{\texttt{broken} \leftrightarrow ( \texttt{no\_cool} \land (\texttt{t}> 20) )  \lor (\texttt{t}> 30)} \label{eqn:broken}
	\end{align}
	where \texttt{no\_cool} is a Boolean variable and \texttt{t} a real-valued variable.
    Let us assume that \texttt{t} is distributed  according to $\texttt{t} \sim \mathcal{N}_\texttt{t}(20,5)$ and that the probability for $\texttt{no\_cool}$ being true is $0.01$. Determining the probability of the formula being true/satisfied is the weighted model integration problem.
\end{example}


We see in Example~\ref{example:wmi_intro} that SMT formulas generalize traditional propositional logic formulas by additionally allowing the use of expressions formulated in a background theory. More formally, following \cite{zuidbergdosmartires2019exact}:

\begin{definition}[SMT($\mathcal{RA}$) (real arithmetics)] \label{def:smtra}
	Let $\bvars$ be a set of $M$ Boolean and $\xvars$ a set of $N$ real variables.
	An {\bf atomic formula} is an expression of the form $g(X) \bowtie c$, where $c \in \mathbb{Q}$, $\bowtie \in \{ =,\neq, \geq,\leq,>,< \}$, and  $g:\mathbb{R}^{N} \rightarrow \mathbb{R}$. The symbols $\mathbb{Q}$  and $\mathbb{R}$ denote the rational number and real numbers, respectively. 
	We then define SMT($\mathcal{RA}$) formulas as Boolean combinations (by means of the standard Boolean operators $\{\neg, \land, \lor, \rightarrow, \leftrightarrow \}$) of {\bf Boolean variables} $b_i \in \bvars$ and of {\bf atomic formulas} over $\xvars$.

	We distinguish two special cases:
	\begin{itemize}
		\item SMT($\mathcal{NRA}$) (non-linear real arithmetics): atomic formulas take the form $\sum_i c_i \cdot x_i^{p_i}\bowtie c$, where the $x_i \in \xvars$ and $c_i,c, p_i \in \mathbb{Q}$.  
		\item SMT($\mathcal{LRA}$) (linear real arithmetics): atomic formulas take the form $\sum_i c_i \cdot x_i \bowtie c$, where the $x_i \in \xvars$ and $c_i,c \in \mathbb{Q}$.
	\end{itemize}
\end{definition}

We define weighted model integration in terms of an indicator function over an SMT formula, cf.~\citep{kolb2019exploit}.
\begin{definition}[{\bf WMI}]\label{def:wmi}
Given a set $\bvars$ of $M$ Boolean variables,  $\xvars$ of $N$ real variables, a weight function $\pweight:
\mathbb{B}^M {\times} \mathbb{R}^N {\rightarrow} \mathbb{R}_{\geq 0}$, and a support $\support$, in the form of an SMT formula, over $\bvars$ and  $\xvars$, the weighted model integral is given by:
\begin{align}
  \wmi(\support, \pweight {\mid} \xvars, \bvars) = \sum_{\bvars} \int \ive{\support(\xvars, \bvars)} \pweight({\xvars},{\bvars}) d{\xvars} \label{eqn:def_wmi}
\end{align}
where we use the Iverson bracket notation in $\ive{\support(\xvars, \bvars)}$ to denote the indicator function of $\support(\xvars, \bvars)$. If the set of real variables $\xvars$ is empty the WMI task reduces to WMC (cf.~\ref{app:amc}).
\end{definition}

\citet{kolb2019exploit} further manipulate the expression in Equation~\ref{eqn:def_wmi} in order to
% get rid of the Boolean dependencies in the weights function $\pweight$ and to 
transform the $\lor$-$\land$ structure present in $\ive{\support(\xvars, \bvars)}$ into a simple conjunction of SMT atoms.
\begin{align}
\wmi(\support, \pweight {\mid} \xvars, \bvars)&=\sum_{\wsupport_i \in \wtuples} \sum_{\bvars} \int \llbracket  \wsupport_i  (\xvars, \bvars) \rrbracket \pwweight(\xvars, \bvars) d\xvars \label{eqn:wmi_sum_ive_weight} \\
&=\sum_{\wsupport_i \in \wtuples} \sum_{\bvars} \int \Bigg\llbracket  \bigwedge_{j} \wsupport_{ij} (\xvars, \bvars) \Bigg\rrbracket \pwweight(\xvars, \bvars) d\xvars 
\end{align}
The weighted model integral in Equation~\ref{eqn:def_wmi} over a support with disjunctions and conjunctions, has become now a sum of multiple weighted model integrals whose supports are simple conjunctions of SMT atoms. $\wtuples$ denotes the set of mutually exclusive SMT formulas whose disjunction is equivalent to the original SMT formula $\support$, \ie $\support\leftrightarrow \lor_i \support_i \leftrightarrow \lor_i \land_j  \support_{ij}$.

% For the purely Boolean case, they correspond to the possible worlds of $\support$. 





==> files_old/arithmetics_old_20210120.tex <==
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%








\section{Arithmetic Expressions}\label{sec:arithmetic}
\ak{I think this should be a part of implementation section, and should be about comparison predicates rather than about arithmetic expressions}

Implementations of (probabilistic) logic programming languages, such as \prologsty and \problogsty, reserve a set of predicate names for system-related procedures. These system predicates (or built-in predicates) are usually deployed when the goal is to perform efficient arithmetic operations on numbers. Either by using specialized algorithms or specialized hardware. In \dcproblogsty we are going to use an external arithmetic engine to evaluate expressions within comparison predicates.

\begin{example}\label{ex:eval_comp} A \dcproblogsty code snippet demonstrating arithmetic evaluations within a comparison predicate.\ak{how is this example relevant here?}
	\begin{problog*}{linenos}
0.5::a.
x ~ normal(0,3):- a.
x ~ normal(1,2):- \+a.

q:- x+3>3.
query(q).
	\end{problog*}
Using the \probloginline{map}\lstinline[columns=fixed]|/2| predicate this program gets transformed into the program below.
	\begin{problog*}{linenos}
0.5::a.
x1 ~ normal(0,3).
map(x1,x):- a.

x2 ~ normal(1,2).
map(x2,x):- \+a.

q:- map(X,x), X+3>3.
query(q).
	\end{problog*}

\end{example}





\luc{technical problem with DC; do we need this?}

\subsection{Type System} \label{sec:type_system}

While we have stated that arithmetic expressions can appear on both sides of comparison predicates, we have not yet mentioned what they evaluate to.
To this end we will regard expressions to be evaluated as unnamed functions, instead of arithmetic predicates\ak{we do not have arithmetic predicates, only arithmetic functors}. Let us consider, for instance, the expression \probloginline{3+5}. This can can be viewed as a term whose predicate is \probloginline{+}\lstinline[columns=fixed]|/2| in infix notation. However, we can also regard the expression as a function with two inputs and an output. Furthermore, we can equip the function with a type signature. The input values are of type \type{Integer} and the output value is of \type{Integer} as well. We will now introduce a type system for the evaluation of arithmetic expressions in \dcproblogsty.

The base type for (arithmetic evaluations in) \dcproblogsty is the \type{Term} type. We subtype terms with a \type{Distribution} type and a \type{Symbol} type. 
Dividing \dcproblogsty terms into \justify\type{Distribution} terms and \type{Symbol} terms reflects the characterization of~\citet{poole2010probabilistic} of probabilistic programs as being constituted of independent choices (\type{Distribution}) and a deterministic system (\type{Symbol}).

\begin{definition}\label{def:type_system}
	The \dcproblogsty type system is a hierarchical type system with each type being a disjoint union of its subtypes. A diagrammatic overview of the \dcproblogsty type system is given in Figure~\ref{fig:type_system}.
	\begin{enumerate}
		\item[] \type{Term} 
		\begin{enumerate}
			\item[1.] \type{Distribution}
			\begin{itemize}
				\item \type{NumericD}
				\item \type{CategorialD}
			\end{itemize}
			\item[2.] \type{Symbol}
			\begin{itemize}		
				\item \type{RandomSymbol}
				\begin{itemize}
				    \item \type{NumericRV}
				    \item \type{CategoricalRV}
				\end{itemize}
				\item \type{DeterministicSymbol}
				\begin{itemize}
				    \item \type{Number}
				    \item \type{Atom}
				\end{itemize}	
			\end{itemize}
		\end{enumerate}
	\end{enumerate}
\end{definition}



\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\linewidth]{../figures/type_hierarchy.pdf}
	\end{center}
	\caption[Diagrammatic representation of the hierarchical \dcproblogsty type system.]{Diagrammatic representation of the hierarchical \dcproblogsty type system. Compared to Definition~\ref{def:type_system},  the \type{Number} type is further subtyped into \type{Integer} and \type{Real} types and the \type{RandomVariable} type is subtyped into \type{DiscreteRV}, \type{ContinuousRV}, and \type{MixtureRV}. These subtypes of \type{RandomVariable} mimic the subtypes of the \type{Distribution} type.\luc{do we want mixtureRV?}}
	\label{fig:type_system}
\end{figure}




\begin{definition}[\type{Distribution}]
	Terms of type \type{Distribution} are constructed by using a reserved random function symbol and applying it to a (possible empty) tuple of input arguments, which maps the input tuple to a distribution term.
	Distribution terms are only allowed to be invoked as a second argument to the reserved distribution predicate \probloginline{~}\lstinline[columns=fixed]|/2|.
	This also means that random function symbols are only used there as well. \dcproblogsty subtypes the \type{Distribution} type into \type{NumericD} and \type{CategoricalD}.
% 	\type{DiscreteD}, \type{ContinuousD}, and \type{MixtureD} types.
\end{definition}

\type{Distribution} terms determine the probability distribution according to which a random variable is distributed.
\probloginline{poisson(6)} and \probloginline{normal(20,5)} are for instance of types \type{DiscreteD} and  \type{ContinuousD}, respectively.
Note that distributions of type \type{ContinuousD} denote {\em absolutely continuous} probability distributions\footnote{\dcproblogsty does not support {\em singular continuous} probability distributions such as the Cantor distribution.}. \ak{would be nice to have a hint on why this restriction is there} We give an example of a distribution of type \type{MixtureD} in Example~\ref{ex:indian_gpa_function}.
%\begin{example} \probloginline{mixed} is a random variables that is a mixture of a continuous part (the truncated normal between $0$ and $4$ with mean $3$ and standard deviation $1$) and a discrete part. 
%\begin{problog}
%mixted~Mix((0.998,TruncNormal(3,1,0,4)),(0.001,4),(0.001,4))
%\end{problog}
%\end{example}

%For and example, see Example~\ref{example:dcproblog_poisson_population}: we have the random function symbol \probloginline{poisson}\lstinline[columns=fixed]{/1}, apply it to the input tuple \probloginline{(6)}, and obtain a term of type \type{Distribution}.


\type{Symbol} terms are the building blocks of the discrete structure that makes up a logic program and as such determine also the deterministic system of a probabilistic logic program. Beyond the reserved syntax, which is used to define the distribution terms, the user is free to use any identifier (following \prologsty conventions) to declare \type{Symbol} terms -- this includes standard \prologsty terms such as lists.
%The subtyping of the \type{Symbol} type (shown in Figure~\ref{fig:type_system}) follows the convention given in~\citep[Chapter 9]{sterling1994art}.

% \begin{definition}[\type{Arithmetic}]
% 	Terms of type \type{Symbol} for which arithmetic operations are defined are of type \type{Arithmetic}. \type{Arithmetic} terms can be used as second argument to the builtin \probloginline{is}\lstinline[columns=fixed]|/2| functor. \type{Arithmetic} terms are subtyped with \type{RandomVariable} terms and \type{Number} terms.
%	\ak{Def 6.3 Arithmetic terms: if (as stated in def 6.1) each type is the disjoint union of its subtypes, that means that "arithmetic" is made up exclusively of numbers and RVs, \ie, terms like 3-2 or min(x,5) for a RV x are not allowed, whereas the first two sentences of def 6.3 suggests they might be allowed (only having numbers and RVs directly on the rhs of is/2 seems quite boring...). Which is it?
%		Related to this, defs 6.8 and 6.10 talk about RVs and Numbers, why not simply "arithmetic"?}
% \end{definition}


\begin{definition}[\type{RandomSymbol}] \label{def:random_variable}
	\type{RandomSymbol} terms are named by the programmer using distributional facts with the binary infix predicate \probloginline{~}\lstinline[columns=fixed]|/2| and inherit their subtype from the distribution term. All random variables present in a \dcproblogsty program are named.
\end{definition}

Examples of terms of type \type{RandomSymbol} would be \probloginline{temperature} and \probloginline{n_people} in Examples~\ref{example:dcproblog_machine} and~\ref{example:dcproblog_poisson_population}, where we declared the random variables through distributional facts: 
\begin{problog}
temperature ~ normal(20,5).
n_people ~ poisson(6).
\end{problog}
As mentioned in Defintion~\ref{def:random_variable}, \type{RandomSymbol} terms inherit their type from the associated \type{Distribution} term, \eg a \type{ContinuousD} term induces a random variable term of type \type{ContinuousRV}.

Note that not all probabilistic programming languages enforce the naming of random variables. In the functional probabilistic programming language \anglicansty~\citep{wood2014approach}, for instance, the user can declare anonymous random variables, much like anonymous functions, \ie \textlambda-functions.
\ak{Discussion of named/unnamed between Defs 6.4 and 6.5: would be nice to have a brief hint on why you made that choice}

\begin{definition}[\type{Number}] Terms of type \type{Number} are used to express numerical data types such as integers and real numbers.	
\end{definition}


\ak{terminology mix-up; predicates never form terms} \pedro{not sure what this comment refers to.}

\begin{definition}[\type{Atom}]
	An atom is of the form \probloginline{p(t@$_1$@,@\dots @, t@$_n$@ )} where \probloginline{p} is a predicate of arity $n$ and the \probloginline{t@$_i$@} are \type{Symbol} terms~\citep{fierens2015inference}. Predicates used to construct \type{Atom} terms must not clash with the builtin predicates and reserved random function symbols used to declare \type{Distribution} terms.
% 	Terms of type \type{Atom} constitute the building blocks of the discrete structure of a probabilistic logic program.
\end{definition}

Examples of atoms terms would be \probloginline{foo} or \probloginline{bar(foo,42)}. The latter is constructed using the predicate \lstinline{bar/2} and the tuple of \type{Symbol} terms \probloginline{(foo,42)}. \probloginline{foo} is of type \type{Atom} and \probloginline{42} is a \type{Number} term.






% \dcproblogsty's type system refines the one of DC-PLP to instantiate a conrete version of the abstract language.  Specifically, we have the following refinements:
% \begin{enumerate}
%     \item distribution functors are further partitioned into \emph{discrete distribution functors}. \emph{continuous distribution functors} and \emph{mixture distribution functors}
%     \item arithmetic functors are further partitioned into \emph{operation functors} and \emph{number functors}, with the latter in turn partitioned into \emph{integers} and \emph{floats} \todo{do we have / want a complete list of operations? should we at least give some examples?}
%     \item we use Boolean query functors 	$\bowtie=\{ \text{\probloginline{=:=}}, \text{\probloginline{=\=}}, \text{\probloginline{<}}, \text{\probloginline{>}},  \text{\probloginline{=<}}, \text{\probloginline{>=}} \}$
% 	in infix notation (and lift them to predicate level as discussed before)
% \end{enumerate}

% \ak{I don't think we need to sub-type random variable functors here, as rv terms inherit the \emph{output} type of the distribution only, which should be integer, float etc, not "discrete distribution"}




\subsection{Multiple Dispatch} \label{ref:multiple_dispatch}
\ak{I think there's a lot in here that misses context to be understandable; and I'm not sure all of it is really needed for the paper}
The attentive reader might have noticed that, for example in Example~\ref{ex:dc-vs-dcproblog}, we used the same comparison predicates, for \type{RandomSymbol} terms as well as \type{Number} terms. In \dcproblogsty we resolve this clash through {\em multiple dispatching}~\citep{castagna1995calculus}.
Multiple dispatching is the process of dynamically selecting at run time\footnote{In the context of logic programming we understand as run time the grounding of the logic program part of a \dcproblogsty program.} a specific implementation of a function based on the types of the arguments that are fed as input to the corresponding function symbol.
Such functions are referred to as {\em multimethods}. 
An early example of multiple dispatch is the {\em Common Lisp Object System}~\citep{keene1989object}. Multiple dispatch is also the programming paradigm on which the \juliasty programming language is built~\citep{bezanson2017julia}.

We also find multimethods in logic programming languages such as \prologsty. While, for groundings of relations \prologsty simply checks whether the grounding is present in the database (agnostic towards the types of the arguments), this is not the case for built-in predicates such as comparison predicates, which make a call to an external arithmetic engine in order to evaluate an expression. For instance, (\probloginline{1<3+5}) calls an integer addition procedure, whereas (\probloginline{1<3.0+5}) might call a floating point procedure. Calling the external arithmetic engine with an ill-typed expression might even cause a run time error. Something that is not possible in {\em pure} \prologsty without an external arithmetic engine.

\luc{implementatin details}
Compared to \problogsty and \problogsty, \dcproblogsty does not only have type signatures for the built-in comparison predicates but also for random function symbols, \eg \probloginline{normal/2}.
Consider, for instance, the declaration of the normal distribution in Example~\ref{example:dcproblog_machine}.
The definition of the function is the following:
$$ \text{\probloginline{normal}}: \type{Number} \times \type{Number} \rightarrow \type{ContinuousD}$$
However, the arguments of a normal distribution (its mean and standard deviation) might as well be random variables themselves.
Multiple dispatching then allows us to {\em overload} the \probloginline{normal} function symbol by using arguments of a different type\footnote{For simplicity we omit that the standard deviation has to be a strictly positive (real) number, which can be enforced by extending the type system.}:
\begin{align*}
	\text{\probloginline{normal}}&: \type{NumericRV} \times \type{Number} \rightarrow \type{ContinuousD} \\
	\text{\probloginline{normal}}&: \type{Number} \times \type{NumericRV} \rightarrow \type{ContinuousD} \\
	\text{\probloginline{normal}}&: \type{NumericRV} \times \type{NumericRV} \rightarrow \type{ContinuousD}
\end{align*}

Reusing the idea of multimethods in the context of probabilistic logic programming with random function symbols results in a simple and neat syntax.
The exact implementation of these random function symbols is left to the designer of an implementation of the language by providing an external engine that performs arithmetic evaluations.

%In the next Subsection~\ref{sec:arithmetic} we will encounter further usages of multiple dispatching in \dcproblogsty.


% We can say that interpreted predicates and functors, that is predicates and functors that have a system internal meaning, possess a type signature. This results in a type dependent calculus.

\paragraph{Strongly Typed \prologsty}

While \prologsty is traditionally not strongly/statically typed, there have been efforts to extend \prologsty with such a type system. Arguably, the most interesting effort is presented in~\citep{Schrijvers2008TowardsTP}, where the authors develop the idea of partially typing a \prologsty program, \ie typing is optional and untyped code is interpreted instead of compiled. Introducing predicates with strongly typed signatures can be regarded as adding interpreted predicates to the \prologsty implementation but the {\em `evaluation'} of these predicates still takes place within \prologsty.
Our efforts to utilize multiple dispatch for arithmetic expressions with an external engine are orthogonal and complimentary to the efforts of~\citet{Schrijvers2008TowardsTP}.

\ak{move to related work?}







\subsection{External Engine}

The key difference between the external arithmetic engine of \prologsty (or \problogsty) and the external arithmetic engine of \dcproblogsty is that the external engine of the latter is capable of performing arithmetic operations (perform evaluations) with random variables. Combining this innovation with multiple dispatch allows us to retain the same syntax (same functor) to perform arithmetic operations on \type{SymbolicRV} terms and/or \type{Number} terms.

In Subsection~\ref{sec:type_system} we introduced an abstract type system.
Abstract types describe the structure/hierarchy of a type system and cannot be instantiated. Concrete types, which are subtypes of abstract types are used for instantiations. This means that abstract types relate collections of concrete types, \ie implementations, to each other. For example, the \type{Integer} \probloginline{3} could be instantiated as an \type{Int32} or also an \type{Int64}, which are both concrete types. The choice taken depends on the external engine used to evaluate arithmetic expressions. 

The only condition that we necessitate for an implementation of \dcproblogsty is that the external arithmetic back-end provides concrete types for the abstract types that should be used in arithmetic expression. Additionally, a practical arithmetic engine should implement arithmetic operations on these types. For example, an engine should be able to multiply a floating point value and an integer value: (\probloginline{3.12*2}). The type for floating points could be dubbed \type{Float32} and would be a concrete type subtyped from the abstract type \type{Real}. The type of the integer value could be \type{Int32} subtyped from \type{Integer}. The return type could then again be \type{Float32}.



\begin{example}
We show two functions that perform addition of numbers but with different types. These different number could be invoked on either side of a comparison predicate, \eg (\probloginline{1<3+5} ) or (\probloginline{1<3+5.0} ). We write these functions using Julia like syntax, as Julia follows the multiple dispatch paradigm.
\luc{too much}
\begin{samepage}

\begin{minted}[
    breaklines,
    escapeinside=||,
    mathescape=true, 
    linenos,
    xleftmargin=20pt, 
    % numbersep=3pt, 
    % gobble=2, 
    % framesep=2mm
]{julia}
function +(a::Int32, b::Int32)::Int32
    return int32_addition(a,b)
end;
\end{minted}

\end{samepage}


\begin{samepage}
\begin{minted}[
    breaklines,
    escapeinside=||,
    mathescape=true, 
    linenos,
    xleftmargin=20pt, 
    % numbersep=3pt, 
    % gobble=2, 
    % framesep=2mm
]{julia}
function +(a::Int32, b::Float32)::Float32
    float_a = convert(Float32, a)
    return float32_addition(float_a,b)
end;
\end{minted}

\end{samepage}


\end{example}












\subsubsection*{Eager Evaluation}

Let us revisit the comparison predicates, \eg (\probloginline{1<2}), (\probloginline{x>20}). According to Definition~\ref{def:semantics_dcproblog} these get wrapped into a \dcplpinline{holds/3} predicate when \dcproblogsty is transformed into \dcplpsty. For the deterministic case we can eagerly evaluate these \dcplpinline{holds/3} predicates. That is, we can replace the atom with its corresponding Boolean value. For the comparison (\probloginline{1<2}) we would get \probloginline{true}. 

Eager evaluation of arithmetic expressions makes most sense when this leads to program simplifications. More concretely, when a comparison predicate is not satisfied this results in a \probloginline{false} atom and proving a goal during grounding can be stopped pre-maturely.\ak{we haven't talked about grounding before...}
Eager evaluation of the \dcplpinline{holds/3} predicate allows \dcproblogsty to retain the usual behavior of proving in \problogsty where a proof fails if a (deterministic) comparison is not satisfied.









% \subsubsection{Arithemtics of Random Variables}

% Evaluating arithmetic expressions that contain random variables should not to be confused with performing arithmetic operations on random variables. Writing \probloginline{x+y} in a comparison predicate, where \probloginline{x} and \probloginline{y} are random variables has the semantics of evaluating both random variables (for instance by drawing a sample) and adding up both evaluations.

% In order to perform arithmetic operations on random variables directly, we would need to introduce syntax and an arithmetic engine for random variables. This could, for example, be achieved in the following fashion:
% \begin{problog*}{linenos}
%  x ~ normal(20,5).
%  y ~ normal(25,6).
%  z ~ x+y.
% \end{problog*}
% In this case z would be a normal distribution with mean ($20{+}25$) and standard deviation ($5{+}6$). We leave arithmetic operations on random variables for future research.\pedro{maybe add citation of somebody who has done something like this already?}






%%%%%%%%%%%%%%%%%%%%

==> files_old/dcplp.tex <==
\section{\dcproblogsty: Core syntax and semantics}\label{sec:semantics}

\todo{better guide the reader through this part; potentially reconsider subsection headings}

In this section, we define the semantics of  \dcproblogsty programs that combine normal logic programs with ground \emph{distributional facts} only, which we also call \emph{core} \dcproblogsty. 
This restriction is for clarity only, 
as we will see in Section~\ref{sec:dcproblog}, where 
we will introduce additional modeling constructs inherited from the ProbLog and DC languages as syntactic sugar defined in terms of this core language. 

\dcproblogsty's semantics is an instance of  Sato's distribution semantics~\citep{sato1995statistical}, which starts from a probability measure over a countable set of facts $F$, the so called \emph{basic distribution},  and then extend this to a probability measure over the Herbrand interpretations of the full program. It is worth noting that the basic distribution is independent of the logical rules. 
In our case, the set $F$ consists of ground Boolean comparison atoms over the random variables defined by the distributional facts. These comparison atoms form an interface between the random variables (represented as terms) and the logical layer that reasons about truth values of atoms. 
While \cite{gutmann2011magic} used the same principle to define the declarative semantics for Distributional Clauses without negation, their focus was on the procedural semantics, and only the latter has been extended to include negation \citep{nitti2016probabilistic}; cf.~also Section~\ref{sec:dcproblog-dc}.
\ak{it seems appropriate to clearly attribute the idea to DC here already, but not sure how to best do this "in passing", without raising too many questions}




\subsection{Syntax}
In the following, we assume the following reserved vocabulary:
\begin{itemize}
    \item A finite set $F_D$ of \emph{distribution functors}, such as \verb|normal/2|, \verb|poisson/1| etc, used to specify the distributions of random variables.
    \item A finite set $F_A$ of \emph{arithmetic functors}, such as \verb|max/2|, (infix) \verb|+/2| etc, as in Prolog arithmetic.
    \item The countable set $F_N=\{0,1,2,\ldots\}$ of constants denoting natural numbers.
    \item $F_M = F_A\cup F_N$
    \item A finite set $C$ of \emph{comparison predicates}, which we further fix to the binary 
    operators \verb|<,>,=<,>=,=:=,=\=| (in Prolog syntax and infix notation) for the sake of concreteness.
\end{itemize}
The precise definitions of $F_D$ and $F_A$, as well as the syntax for defining queries and observations for inference, are left to system designers. \ak{decide names of sets later, when we know all of them...}
As logic programming generally operates on a countable universe, we restrict arithmetic to the rational numbers (constructed from the natural numbers and appropriate functors) here. As for Prolog arithmetic, an implementation can of course support floating point numbers as syntactic sugar in programs, and we also use those in our examples for ease of readability. 

\begin{definition}[Distributional Fact]
A \emph{distributional fact} is of the form \probloginline{x ~ d}, with \probloginline{x} a ground term whose functor is not part of the reserved vocabulary, and \probloginline{d} a ground term with a functor in $F_D$. Such a fact declares \probloginline{x} to be a random variable following the distribution denoted by \probloginline{d}. 
\end{definition}

\begin{definition}[(Core) DC-ProbLog program]
A \dcproblogsty program $P=(D,R)$ consists of
a countable set $D$=\{\probloginline{x1 ~ d1}, \probloginline{x2 ~ d2}, \ldots\} of distributional facts, where the \probloginline{xi} are all different, and a normal logic program $R$ where clause heads do not use reserved predicates. $P$ defines the set of random variables $V=\{\text{\probloginline{x}}~|~\exists \text{\probloginline{d}}. \text{\probloginline{x~d}}\in D\}$. 
\end{definition}


\begin{example}\label{ex:random_choice_dependency}
Consider the  following \dcproblogsty program $P=(D,R)$.
\begin{problog*}{linenos}
% distributional facts D
x ~ normal(5,2).
y ~ normal(x,7).
z ~ normal(y,1).
% logic program R
a :- abs(x-y) =< 1. 
b :- not a, z>10.
\end{problog*}
The distributional facts encode a Bayesian network with  normally distributed random variables, two of which serve as parameters in the distribution of another one. We thus have $V=\{$\dcplpinline{x}, \dcplpinline{y}, \dcplpinline{z}$\}$.
The logic program defines two logical consequences of Boolean comparisons over the BN, where \probloginline{a} is true if the absolute difference between random variables \probloginline{x} and \probloginline{y} is at most one, and \probloginline{b} is true if \probloginline{a} is false and random variable \probloginline{z} is greater than ten. 
Here, $F$ contains the comparison atoms \probloginline{abs(x-y) =< 1} and \probloginline{z>10} explicitly mentioned in the logic program, but also all other meaningful comparison atoms that can be built from the numbers in the program and the vocabulary for arithmetic and comparisons, \eg, \probloginline{x<y} or \probloginline{7*x=:=y+5}. 
\end{example}
\ak{What about eg x/y<5 which divides by zero in some worlds?}
In Section~\ref{sec:dcproblog}, we will extend the syntax to also include probabilistic facts, annotated disjunctions and distributional clauses.

\subsection{Validity}\label{sec:dcplpvalidity}
We now discuss validity criteria under which a 
DC-ProbLog program defines a unique probability distribution over its Herbrand interpretations. 

The semantics of a \dcproblogsty program involves two kinds of assignments. First, each random variable takes a value according to the associated distribution. Second, once fixed, the values of the random variables jointly determine a truth value assignment to the comparison atoms, which we call a \emph{consistent fact database} to distinguish it from arbitrary interpretations of these atoms that may not respect their intended meaning, and which is extended to a Herbrand interpretation of the program via the logical rules. The following definition  introduces corresponding terminology and notation.
\begin{definition}[Consistent fact database]
Let $P=(D,R)$ be a \dcproblogsty program. For a distributional fact \probloginline{x~d} $\in D$, we denote by  $\omega$(\probloginline{x}) any value that \probloginline{x} can take according to \probloginline{d}.\todo{proper terminology for "can take"?} We write $\omega = (\omega(v_1),\omega(v_2),\ldots)$ for a combination of value assignments to all random variables $V=v_1,v_2,...$. 
We denote by $F=\{q_1,q_2,\ldots\}$ the set of all well-typed ground Boolean comparison atoms  that can be built from the reserved vocabulary $F_A\cup C$ together with $V$. \todo{what exactly is "well-typed"?} We define $I_{\omega}(q_i)=1$ if $q_i$ is true after setting all random variables to their values under $\omega$, and $I_{\omega}(q_i)=0$ otherwise. $I_{\omega}$ induces the  \emph{consistent fact database} $F_{\omega}=\{q_i~|~I_{\omega}(q_i)=1\}$. 
\end{definition}

Informally, in order to obtain a probability distribution over Herbrand interpretations, we  need to ensure that
\begin{itemize}
    \item The distributional facts $D$ define a unique joint distribution over the random variables they introduce, which will be our starting point.
    \item The comparison atoms are measurable under that distribution, such that we can use it to define the basic distribution.
    \item For any consistent fact database, adding the rules $R$ results in a program whose canonical model is two-valued, \ie, assigns a truth value to every atom in the Herbrand base. This is needed to extend the basic distribution to all atoms.
\end{itemize}

We further elaborate on the first point in the following. The key idea is to view the set of random variables as the nodes in a Bayesian network, where each node's distribution is parameterized by the parents of that node, as already illustrated in Example~\ref{ex:random_choice_dependency}.  
\begin{definition}[parent, ancestor]
Given a program $P$ with facts \probloginline{vp~dp} and \probloginline{vc~dc}  in $D$, the random variable \probloginline{vd}  is a \emph{parent} of the child random variable \probloginline{vc} if and only if  \probloginline{vd} appears in \probloginline{dc}. We define \emph{ancestor} to be the transitive closure of \emph{parent}.
\end{definition}


\begin{example}\label{ex:random_choice_dependency_parents}
In Example~\ref{ex:random_choice_dependency}, \probloginline{x} is the parent of \probloginline{y}, and \probloginline{y} is the parent of \probloginline{z}. Thus, \probloginline{x} does not have ancestors, \probloginline{y}'s only ancestor is \probloginline{x}, and both \probloginline{x} and \probloginline{y} are ancestors of \probloginline{z}.
\end{example}


The next definition formalizes the BN idea.
\begin{definition}\label{def:well-defd-facts}
The set $D$ of distributional facts in a program $P=(D,R)$ is called \emph{well-defined} if and only if it satisfies the following criteria:
\begin{labeling}{W3}
\item[W1] Each $v_i\in V$ has a finite set of ancestors.
\item[W2] The ancestor relation on the variables~$V$ is acyclic.
\item[W3] For each atom $v_i \sim d_i$ in $D$, and for each combination of possible values the parents of $v_i$ can take given the distributions associated to them in $D$, 
$d_i$ is a well-defined distribution term. 
\end{labeling}  
\end{definition}

%\pedro{do we need finite support condition?}\ak{finite support is something else, and not needed here (not part of DS, only needed for inference)}



\begin{definition}\label{def:core-valid}
A \dcproblogsty program $P=(D,R)$ is called \emph{valid} if and only if it satisfies the following criteria:
\begin{labeling}{V3}
\item[V1] The set $D$ is well-defined. 
\item[V2] All Boolean queries in $F$ are Lebesgue-measurable.
\item[V3] For each consistent fact database $F_{\omega}$, the logic program $F_{\omega}\cup R$ has a two-valued well-founded model~\citep{van1991well}.  
\end{labeling}
\end{definition}





\subsection{Semantics}
We follow the common practice of defining the semantics with respect to ground programs; the semantics of a program with non-ground $R$ is defined as the semantics of its grounding with respect to the  Herbrand universe.

Let $P$ be a valid \dcproblogsty program as defined above.
If $D$ is empty, \ie, $P$ does not define any random variables,  the semantics of $P$ is the well-founded model of $R$. Thus, normal logic programs are a special case of \dcproblogsty.\footnote{Note that in the absence of random variables, all well-typed Boolean queries, and thus all facts in $F$, have deterministic truth values.} In the following, we assume that $D$ is not empty. 

Our definition of the semantics closely follows Sato's distribution semantics \citep{sato1995statistical}, \ie, we first establish a probability measure over interpretations of the countable set of facts $F$, and then  extend this to one over Herbrand interpretations. The key differences are that (1) to support continuous distributions, our measure over facts is in itself induced by a measure over value assignments to the random  variables and (2) to support negation, we use normal logic programs with the well-founded model as canonical model instead of definite clause programs with least Herbrand models.


\subsubsection{Probability measure over random variables}
We first show that a valid DC-ProbLog program $P=(D,F)$ defines a probability measure $P_V$ on truth value assignments $\omega$ to its random variables $V$. To do so, we borrow ideas from Bayesian Logic Programs (BLPs)~\citep{kersting2000bayesian}\footnote{Note that while BLPs also use LP syntax to define the random variables and structure of a Bayesian network, the way they use that syntax is fundamentally different from ours.}, exploiting the analogy between the ancestor structure on $V$ and the structure of a Bayesian network. 
Validity condition V1 states that $D$ is well-defined, \ie, each random variable has a finite set of ancestors, and the ancestor relation is acyclic. There thus exists an enumeration $v_1,v_2,...$ of the random variables such that $i<j$ for all pairs $(v_i,v_j)$ where $v_i$ is an ancestor of $v_j$.
V1 further ensures that each variable's distribution is well-defined for every combination of parent values. For each finite subset of random variables closed under the ancestor relation, the joint distribution on that set  thus has the form of a Bayesian network, and factorizes into the product of the individual variables' distributions. It can be shown that under these conditions, there is a unique probability measure $P_V$ over the space of possible assignments to $V$; we refer to \cite[Theorem 4.9]{kersting2000bayesian} for the technical details. 

\luc{not formal enough?}
\ak{should be a bit more formal than before; I don't know how to make it more formal without reproducing Kristian's work...}

\subsubsection{Probability measure over (consistent) fact databases}
We now show that the probability measure $P_V$ over assignments to the random variables uniquely induces a probability measure $P_F$ over truth value assignments to the facts $F$; this is the \emph{basic distribution} in the distribution semantics.

We fix an arbitrary enumeration  $A_1,A_2,...$ of the atoms in $F$. 
Each $A_i$ \emph{depends} on a finite set $V_i$ of random variables, namely  those mentioned in $A_i$ as well as all their ancestors. We write $V_{\leq n}=\bigcup_{1\leq j\leq n}V_j $ for the union of random variables the first $n$ atoms in the enumeration depend on, and $P_{V_{\leq n}}$ for $P_V$ restricted to this set.  

By validity criterion {\bf V2}, all queries $q_i$ are  Lebesgue-measurable, and we thus get a family of distributions
\begin{align}
P_F^{(n)}(A_1=x_1,\ldots,A_n=x_n) = \int_{\Omega(V_{\leq n})} \mathbf{1}_{[q_1=x_1\wedge\ldots\wedge q_n=x_n]}(\omega)dP_{V_{\leq n}}(\omega)
\end{align}
where the $x_i$ are $0$ or $1$, $P_{V_{\leq n}}$ factorizes over the random variables in $V_{\leq n}$ as discussed above, $\Omega(V_{\leq n})$ denotes the space of possible assignments for variables in $V_{\leq n}$, and $\mathbf{1}_{[\varphi]}$ is the indicator function, \ie, equals $1$ if $\varphi$ is true and $0$ otherwise. The definition in terms of an indicator function and the measurability of the underlying Boolean queries ensures that this family of distributions is of the form required for the distribution semantics, \ie, they are well-defined probability distributions satisfying the compatibility condition\footnote{I.e., $P_F^{(n)}$ can be obtained from $P_F^{(n+1)}$ by summing out $A_{n+1}$, for any $n$.}. There thus exists a completely additive probability measure $P_F$ over the space of truth value assignments to $F$ such that for any $n$, we have
\begin{align}
P_F(A_1=x_1,\ldots,A_n=x_n) =P_F^{(n)}(A_1=x_1,\ldots,A_n=x_n)
\end{align}
We note that by construction, this measure assigns mass to consistent fact databases only. 

\subsubsection{Probability measure over Herbrand interpretations}
In the last step, we follow Sato's construction to obtain a probability measure $P_P$ over Herbrand interpretations from $P_F$. To do so, we fix an enumeration $A_1,A_2,\ldots$ of all atoms in the Herbrand base, which includes those in $F$. 
Validity criterion {\bf V3} ensures that for every consistent fact database $F_{\omega}$, the logic program $F_{\omega}\cup R$ has a total well-founded model $M_{\omega}$, and we can thus define   
\begin{align}
P_P^{(n)}(A_1=x_1,\ldots,A_n=x_n) := P_F(\{F_{\omega}~|~ M_{\omega}\models A_1^{x_1}\wedge\ldots\wedge A_n^{x_n}\})
\end{align}

\pedro{is the $P_F$(of a set) equal to sum of $P_F$(not a set)}\ak{what do you mean? note that the elements of the set are mutually exclusive}

where $A_i^1=A_i$ and $A_i^0=\neg A_i$, and it again follows that there is a completely additive probability measure $P_P$ over Herbrand interpretations, which completes the definition of the semantics. 

\pedro{$P_p^{n}$ never introduced}\ak{(3) introduces it? we could explicitly write the analogue of (2) for $P_p$ as well if needed}



\subsection{Inference tasks}\label{sec:inference-tasks}
As in any probabilistic programming language, key inference tasks include computing the marginal probability of a query, \ie, a ground atom, being true in a given program, or the conditional probability of a query being true given observed truth values of one or more other logical atoms.
\ak{do we need formal details?}

\subsubsection{Conditional Queries}
\ak{this is mostly adapted from text moved from elsewhere; I am not fully sure whether all of it should stay here (some of it could be related work or details of inference algorithms)}

Queries conditioned  on standard logic atoms only  can be answered as usual by dividing the marginal probabilities of the conjunction of query and evidence by the marginal probability of just the evidence. 


As the probability of a random variable with uncountably many outcomes taking a specific value is zero, conditioning on a random variable taking a specific value is slightly more complicated, as the above approach would result in  a division by zero and consequently an undefined conditional probability. 
This problem is related to the Borel-Kolomogorov paradox~\citep{kolmogorov1950foundations,gyenis2017conditioning}, which is again caused by a zero-division.

We will, analogously to \citet{nitti2016probabilistic},   follow~\citet{kadane2011principles} to resolve the division by zero issue.
We make the explicit distinction between the probability $P$ and the probability density function $p:\frac{d}{dx}P(X \leq x)=p(x)$. The conditional probability is defined as:\todo{align syntax with rest of semantics section}
\begin{align}
	P(\support_q| \support_e)
	&=P(\support_q|rv=v) & (\support_e \leftrightarrow rv=v )\\
	&=\lim_{\Delta v\rightarrow 0} \frac{P(\support_q,rv \in [v-\nicefrac{\Delta v}{2},v+\nicefrac{\Delta v}{2}])}{ P(rv \in [v-\nicefrac{\Delta v}{2},v+\nicefrac{\Delta v}{2}])} \label{equ:borel_limit} \\
	&=\lim_{\Delta v\rightarrow 0} \frac{\int \ive{ \support_q(x,rv=v)} p(x,rv=v)dx \cancel{\Delta v}}{p(rv=v)\cancel{\Delta v}} \\
	&=\frac{\int \ive{ \support_q(x, rv=v)} p(x,rv=v)dx}{p(rv=v)}
\end{align}
This means that we do not divide anymore by zero but by the number obtained when evaluating the probability distribution at the observed point. For example, when evaluating \probloginline{beta(2,3)} (cf. Example~\ref{example:dcproblog:observation}, Line~\ref{example:dcproblog:observation:beta23}) at $4/10$  we get $1.7280$ instead of zero.
% Note that this is not a probability between zero and one.

In order to guarantee that the limit in Equation~\ref{equ:borel_limit} exists, we restrict this kind of conditioning to equality between a {\em named} random variable and a given constant, cf. Example~\ref{example:dcproblog:observation}.
Relaxing this restriction might lead to the non-existence of the limit. Exactly this situation gives rise to the Borel-Kolmogorov paradox emerges. 

Nevertheless, some languages lift this restriction, which results in possibly semantically ill-defined programs, such as in Distributional Clauses~\citep[Section 3.2]{nitti2016probabilistic}. A more sophisticated method to tackle the non-uniqueness of the conditional probability is {\em disintegration}~\citep{shan2017exact}, where, instead of returning a conditional probability, a family of conditional probabilities is returned (representing an uncountable number of limits). Other languages, such as BLOG, simply assume the existence of the limit~\citep{wu2018discrete}.

The limitation to direct equality statements might seem too restrictive for the purpose of probabilistic programming. Take for example the following conditional probability~\citep{nitti2016probabilistic}:
\begin{align}
	P(nationality| height {=} 160 \lor height {=} 180) \label{eqn:disj_conditioning}
\end{align}
We cannot express this query. However, if we think about what a conditioning set represents in the context of probabilistic programming and machine learning, the example above appears quite odd. The conditioning set tells us which observations we have made about the world, \ie data that we collected using a physical device (\eg tape measure for the height of a person). The example in Equation~\ref{eqn:disj_conditioning} now tells us that our measuring device returned two numbers for a single measurement, which means that the measuring protocol is underspecified.

We just stated that a measurement consists of retrieving a number from a measuring device. This is not entirely correct. In the natural sciences a measurement consists always of a number and an upper and lower error bound, which effectively eliminates the problem of zero probability events. However, given the ubiquity of single point measurement, we feel that a probabilistic programming language that is not able to handle single point measurements is greatly hurt in its expressivity.

To conclude,  \dcproblogsty allows a user to condition on zero probability events, while at the same time the imposed restrictions ensure that the encoded probability distribution is well defined.


\ak{conditional probabilities: just wondering: is it possible to condition on tests, \eg, observing that someone's height is at most 180? related to that, in (17), what if someone with bad handwriting measured the height and recorded it on a piece of paper, and I can't tell whether it is 160 or 180? :) }
\pedro{in this case the measurement is the pixels and you would have yes/no for each pixel}

We introduce syntax to specify inference tasks when discussing our implementation of \dcproblogsty in Section~\ref{sec:implementation}.

==> files_old/dcplp_old.tex <==

\section{DC-PLP}\label{sec:semantics}

In this section we will briefly sketch the main ideas for defining the semantics of \dcproblogsty.
The semantics of \dcproblogsty are defined through the semantics of DC-PLP, a probabilistic logic programming language with both discrete and continuous random variables following \citeauthor{sato1995statistical}'s distribution semantics~\citep{sato1995statistical}. DC-PLP is an assembly language with minimal syntax, whose main purpose is to define the declarative semantics of the language independently of existing syntax, inference algorithms or systems. 

\citet{poole2010probabilistic} has characterised probabilistic programming as independent choices plus deterministic systems, with (discrete) probabilistic logic programming being the case where the deterministic system is given by a logic program~\citep{poole2010probabilistic}. DC-PLP builds upon this idea, but relaxes the independence assumption by explicitly distinguishing two types of dependencies: 1) those expressed by the logic program (i.e.  deterministic system), and 2) those expressed by using random variables as parameters of distributions for other random variables. 

DC-PLP serves as a stepping stone towards \dcproblogsty: the semantics of \dcproblogsty are defined through the semantics of DC-PLP and an additional unique deterministic program transformation that takes \dcproblogsty programs and maps them to DC-PLP programs.

%which will combine the semantics defined here with a higher level modeling language and a system combining that modeling language with inference algorithms developed in the context of related languages from the \problogsty family.


The key idea behind DC-PLP is to build the semantics of a program in three steps:
\begin{enumerate}
	\item Define a {\bf countable set of random variables}
	%	(denoted by terms in the logic program)
	and associate a unique parametric distribution
	%	(denoted by a term from a language $P$ in the logic program)
	to each random variable through a logic program that defines terms of the form \probloginline{rv(name,dist)}. We do not use the \probloginline{is}\lstinline[columns=fixed]|/2| infix notation for distributional clauses to make explicit that this is restricted to fully deterministic bodies. We do not introduce syntax for probabilistic facts, as these can be modeled through Boolean random variables and rules.
	For valid programs, this will give us a 
	unique joint probability measure over these random variables that factors into the individual distributions.
	\item Define a {\bf countable set of measurable Boolean queries}
	%	(denoted by terms from a language $Q$)
	over the random variables. These correspond to the type of tests that are written with comparison predicates (\probloginline{<}, \probloginline{=<}, \probloginline{>}, \probloginline{>=}, \probloginline{=:=}, \probloginline{=\=}). However, we here define these on the term level and wrap them into a single predicate \probloginline{test}\lstinline[columns=fixed]|/1| for ease of uniform notation.
	\item Define a {\bf logic program} that computes consequences of the Boolean queries. To include a  Boolean query \probloginline{q} in the body of a clause, it gets wrapped into a term of the form \probloginline{test(q)}. 
\end{enumerate}

The first step defines all random choices, while the second and third step form the deterministic system. 
As the second and third step are deterministic functions of the random variables, the measure defined in the first step extends to the Boolean queries and from there to the terms in the logic program.

%Note that DC-PLP is parameterized by two sets: the  language $P$ of parameterized distribution terms  and the language $Q$ of basic Boolean queries.
%We sometimes use DC-PLP(P,Q) to highlight this. 

%Note further that while we implicitly assume  ``atomic'' random variables here, the principles also apply to ``compound'' random variables (such as multivariate Gaussians), provided usual laws of probability are respected and suitable syntax for such variables is introduced.

In contrast to the Distributional Clauses probabilistic programming language~\citep{gutmann2011magic}, where several conditional distributional clauses can jointly define the distribution of a single random variable through a complex logical factorization, DC-PLP uses a single fact to define a random variable unconditionally and associates a single parameterized distribution to it. As we still have the full power of normal logic programs to model the deterministic system, this does not restrict expressivity, but simplifies the formal definition of the semantics. When modeling conditional distributions, users have a range of choices, from encoding the entire conditional probability distribution into a single term within the defining \probloginline{rv}\lstinline[columns=fixed]|/2| fact, all the way to a set of individually named choice random variables with minimal use of random variables as parameters tied together by a deterministic system, or any intermediate factorisation.
As already discussed by~\citet{poole2010probabilistic}, not all choices work equally well with all inference algorithms.
DC-PLP provides these choices within the same semantical framework, leaving it to system developers to focus the syntax towards a subset of choices and/or to exploit the different choices when integrating different inference approaches into their system.

\ak{example 6.7: I'm surprised that the test/1 atoms explicitly appear as facts in the DC-PLP program, as I've always imagined them as a component defined implicitly (like the Herbrand universe in LP semantics). Is there a reason to make them explicit?}

\begin{example}[DC-PLP Program] \label{ex:dcproblog_program_without_dc_plpdc}
	This example program models the correct working of a machine.
	
\begin{problog*}{linenos}
rv(hot, flip(0.2)). 
rv(cooling(1), flip(0.99)). 
rv(temperature(hot), normal(27,5)).
rv(temperature(not_hot),normal(20,5)).


test(cooling(N)=:=1)
test(hot=:=1).
test(hot=:=0).
test(temperature(hot)<25.0).
test(temperature(not_hot)<25.0).


machine(1).
works(N):- machine(N), test(cooling(N)=:=1).
works(N):-
	machine(N),
	test(temperature(hot)<25.0),
	test(hot=:=1). 
works(N):-
	machine(N),
	test(temperature(not_hot)<25.0),
	test(hot=:=0). 

query(works(1)).
\end{problog*}
	We are now able to clearly identify the three components of a DC-PLP program. In the first part we see the random variables (representing independent choices). Here we also also included the probabilistic facts from the intial \dcproblogsty program. DC-PLP encodes probabilistic facts using the \probloginline{flip}\lstinline[columns=fixed]|/2| random function symbol, which returns either $1$ or $0$ with the probability given as the argument. In the second block of code we see the countable set of measurable Boolean queries, and the last part contains the logic program.
\end{example}

\subsubsection*{Multiple Dispatch and Comparison Predicates}

As mentioned earlier, multiple dispatching is of outstanding usefulness when applying comparison predicates to different type signatures that result in semantically different terms. We will illustrate this by example.

\begin{example} Consider the following \dcproblogsty code snippet with no random variables.
	\begin{problog*}{linenos}
people(N):- N is 8.
large_group:- people(N), N>6.
	\end{problog*}
	During grounding, the comparison operator in the second line will dispatch to a deterministic comparison, as both sides of the comparison are of type \type{Number}. The arithmetic engine replaces the grounded comparison term with atom \probloginline{true}.
\end{example}

\begin{example} Consider now  a \dcproblogsty code snippet where a comparison predicate is present that receives as one of its arguments a term of type \type{RandomVariable}.
	\begin{problog*}{linenos}
people ~ poisson(6).
large_group:- people>6.
	\end{problog*}
	During grounding the comparison predicate dispatches to a probabilistic comparison. Instead of replacing the comparison by either \probloginline{true} or \probloginline{false}, the arithmetic engine defers the evaluation and ultimately adds a \probloginline{test(people>6)} term to the set of measurable Boolean queries.
\end{example}

\subsection{Valid DC-PLP Programs}

\pedro{\url{https://youtu.be/rdsPMCYMcZA?t=1510} stuart russell makes an interesting point about restricting the language.}

\begin{definition}
	A DC-PLP program \dcpprogram consists of:
	\begin{enumerate}
		\item A countable set $P$ of random variables.
		\item A countable set $Q$ of measureable Boolean queries over the random variables.
		\item A logic program $L$, which has access to the set of Boolean queries.
	\end{enumerate}
\end{definition}

\ak{\begin{itemize}
		\item says two conditions for a list of 3 (also check use of "second" in the text afterwards; not sure total models link to finite support)
		\item point 1: doesn't seem fully defined, as it only assigns ranks to RVs, but not all $d_i$ are necessarily RVs
		\item point 2: "every model of L" -- what is a model of a program with access to Boolean queries? needs to be defined
		\item point 3: what does it mean for a model to be "derivable" from a set of queries?
	\end{itemize}
}

\begin{definition} \label{def:valid_dcplp}
	A DC-PLP \dcpprogram program is called valid  if the following two conditions hold.
	\begin{enumerate}
		\item The program \dcpprogram is distribution stratisfied, that is, there exists a function $rank(\cdot)$ that maps ground random variables, of the form \probloginline{rv(rand,dist(d@$_1$@,...,d@$_n$@))}, to $\mathbb{N}$ and that satisfies $rank(\text{\probloginline{rand}})>rank(\text{\probloginline{d@$_i$@}})$ for every $i$ ($1\leq i \leq n$). 
		\item The logic program $L$ is {\em sound}~\citep{riguzzi2013well}, \ie every model of $L$ is a two-valued well-founded model~\citep{van1991well,riguzzi2013well}.
		\item Each model of $L$ is derivable from a finite set of Boolean queries in $Q$.
	\end{enumerate}
\end{definition}
The first condition ensures that programs do not exhibit cyclic functional dependencies, disallowing programs of the form:
\begin{problog*}{linenos}
x ~ normal(y,1).
y ~ normal(x,1).
q:- y>3.
query(q).
\end{problog*}
The second condition is necessary to satisfy the finite support condition of the distribution semantics~\citep{sato1995statistical}. Definition~\ref{def:valid_dcplp} follows closely the semantics of \problogsty~\citep{fierens2015inference}, which guarantees that a \dcproblogsty program without distributional facts is in fact a \problogsty program.


\subsubsection{Negation}

In order to add negation to the hybrid probabilistic logic programming language Distributional Clauses, \citet{nitti2016probabilistic} resorted to {\em negation as failure} within a {\em Selective Linear Definite (SLD) resolution}~\citep{sterling1994art} inference scheme to patch the initial (negation-free) semantics given in~\citep{gutmann2011magic}. The semantics then follow~\citep{przymusinski1988perfect}'s perfect model semantics.

The well-founded semantics already account for negation in logic programs and we do not have to add any extra machinery to add negation. On a side note: in the absence of negation the well-founded model of a logic program is identical to the {\em least Herbrand model}. 




\subsubsection{Probability of a DC-PLP Program}

\begin{definition}
	Let $MOD(L)$ be the set of all two-valued well-founded models of $L$, which is the logic program of a valid DC-PLP program \dcpprogram, and $Q(l)$ the set of Boolean queries used to derive $l \in MOD(L)$. Furthermore, let $var(Q(l))$ be the set of random variables on which $Q(l)$ depends.
	The probability of the model $l$ is then given by:
	\begin{align}
		p(l) = \int \left( \prod_{q \in Q(l)} \ive{q} \right) \underbrace{\left( \prod_{x_l \in var(Q(l))} D_l(x_l)  \right)}_{\eqqcolon D_l(\xvars_l)} \underbrace{\left( \prod_{x_l \in var(Q(l))} d x_l  \right)}_{\eqqcolon d\xvars_l}
	\end{align}
	$D_l(x_l)$ is the probability distribution according to which the variable $x_l$ is distributed and which is given by the countable set $P$.
	
	The probability of the DC-PLP program \dcpprogram is given by:
	\begin{align}
		p(\dcpprogram) = \sum_{l \in MOD(L)} p(l) = \sum_{l \in MOD(L)} \int \prod_{q \in Q(l)} \ive{q} D_l(\xvars_l) d\xvars_l \label{eq:definition_probability_dcplp}
	\end{align}
\end{definition}





==> files_old/dcplp_old_16122020.tex <==
\section{DC-PLP}\label{sec:semantics}
We introduce DC-PLP, a probabilistic logic programming language with both discrete and continuous random variables following Sato's distribution semantics \citep{sato1995statistical}. DC-PLP is an assembler language with minimal syntax whose  purpose is to define the declarative semantics of the language independently of existing syntax, inference algorithms or systems. 

Poole has characterised probabilistic programming as independent choices plus deterministic systems, with (discrete) probabilistic logic programming being the case where the deterministic system is given by a logic program \cite{poole2010probabilistic}. DC-PLP builds upon this idea, but relaxes the independence assumption by explicitly distinguishing two types of dependencies, namely those expressed by the logic program /  deterministic system, and those expressed by using random variables as parameters of distributions for other random variables. It further allows for both discrete and continuous random variables.

In the context of of probabilistic logic programming, \cite{gutmann2011magic} have introduced Distributional Clauses (DC), which also combines continuous random variables with (definite) logic programs. We deviate from their proposal in the following ways:
\begin{itemize}
    \item we provide a simpler framework that clearly exposes all dependencies at no loss in expressivity
    \item we refine their validity criteria to address two known issues (logical cycles and parameter cycles)
    \item we support negation from the start
    \item we provide explicit connections to a range of existing PLP languages
\end{itemize}

DC-PLP serves as a stepping stone towards DC-ProbLog, which will combine the semantics defined here with a higher level modeling language, and a system combining that modeling language with inference algorithms that have been or will be developed in the context of related languages from the ProbLog family.  

The key idea behind DC-PLP is to build the semantics of a program in three steps:
\begin{enumerate}
\item Define a countable set of random variables (denoted by terms in the logic program) and associate a unique parametric distribution (denoted by a term from a language $P$ in the logic program) to each random variable through a set of ground atoms of the form \verb|rv(name,dist)|. For valid programs, this will give us a 
unique joint probability measure over these random variables that factors into the individual distributions.
\item Define a countable set of measurable Boolean queries (denoted by terms from a language $Q$) over the random variables.
\item Define a logic program that computes consequences of the Boolean queries. To include a  Boolean query in the body of a clause, it gets wrapped into an atom of the form \verb|holds(query)|, whose purpose is to explicitly transfer the externally determined truth value of the query into the truth value of an atom within the logic program.\footnote{This is for simplicity of exposition; higher level modeling languages such as DC-ProbLog would usually provide comparison predicates on terms directly.}
\end{enumerate}
The first step defines all random choices, the second and third step form the deterministic system. 
As the second and third step are deterministic functions of the random variables, the measure defined in the first step extends to the Boolean queries and from there to the atoms in the logic program.

We restrict the definition of \verb|rv/2| to be a database of facts here purely for simplicity; this can be relaxed to a logic program that does not refer to any \verb|holds| atoms or any predicates defined in the third component (which can be mapped back to a fact database corresponding to its well-founded model).


Note  that while we implicitly assume  ``atomic'' random variables here, the principles also apply to ``compound'' random variables (such as multivariate Gaussians), provided usual laws of probability are respected and suitable syntax for such variables is introduced.

In contrast to DC, where several conditional distributional clauses can jointly define the distribution of a single RV through a complex logical factorisation, DC-PLP uses a single fact to define a random variable unconditionally and to associate a single parameterised distribution to it. As we still have the full power of normal logic programs to model the deterministic system, this does not restrict expressivity (as we will see in Section~\ref{sec:dc}), but simplifies the formal definition of the semantics. When modeling conditional distributions, users have a range of choices depending on the syntax provided, from encoding the entire CPD into a single term within the defining \verb|rv/2| fact all the way to a set of individually named choice RVs with minimal use of RVs as parameters tied together by a deterministic system, or any intermediate factorisation. As already discussed by Poole \cite{poole2010probabilistic}, not all choices work equally well with all inference algorithms. We provide these choices within the same semantical framework, leaving it to system developers to focus the syntax towards a subset of choices and/or to exploit the different choices when integrating different inference approaches into their system.

\subsection{Syntax}
A key element of DC-PLP are reserved functors\footnote{We consider constants to be functors of arity 0.} with a specific external interpretation, which are used to define distributions and evaluable expressions over random variables. While the exact choice of these functors is up to the designers of a specific DC-PLP instance, they have to obey certain rules which we specify next.

The set of functors used in a DC-PLP program can be partitioned into the following types:
\begin{enumerate}
\item \emph{reserved functors} with typed arguments and an output type, further partitioned into 
\begin{enumerate}
    \item \emph{distribution functors}, \eg \verb|poisson/1| with input and output type \emph{natural number}
    \item \emph{arithmetic functors}, \eg, the (zero-arity) functor \verb|17| is of return type number, \verb|max/2| takes two numbers and returns a number
    \item \emph{Boolean query functors} with output type Boolean, \eg, \verb|</2| with two arguments of type number
\end{enumerate}
\item \emph{user-defined functors}, whose arguments do not need to be typed, further partitioned into
\begin{enumerate}
\item \emph{random variable functors} with type declared  in the program through association with a distribution term as detailed below
    \item \emph{regular functors} do not need to be typed
\end{enumerate}
\end{enumerate}
We refer to a term with top level functor of type X as a term of type X, \eg, \verb|poisson(6)| is a distribution term, and \verb|x<5| with random variable \verb|x| a Boolean query term. 
In the following, we assume a fixed set of reserved functors.

DC-PLP further uses two reserved, typed predicates:
\begin{enumerate}
    \item \verb|rv/2|, where the  first argument has to be a random variable term and the second argument has to be a distribution term, and a fact \verb|rv(x,d)| associates the random variable \verb|x| with the distribution term \verb|d|, thus also setting the type of \verb|x| to the output type of \verb|d|
    \item \verb|holds/1|, where the argument has to be a Boolean query term, and the truth value of a ground atom \verb|holds(q)| is the result of evaluating query \verb|q|
\end{enumerate}
As in the non-probabilistic case of logic programming versus Prolog, we leave the introduction of the external arithmetic evaluation predicate \verb|is/2| to DC-ProbLog, but note that the \verb|holds/1| predicate has a similar role as external evaluation interface (which includes evaluating any arithmetic functors that are part of its argument). 


A DC-PLP program $P=(D,R)$ consists of
\begin{itemize}
    \item a countable set $D=\{\mathtt{rv}(x_1,d_1),\mathtt{rv}(x_2,d_2),\ldots\}$ of ground well-typed \verb|rv/2| facts,  where the $x_i$ are all different 
    \item a normal logic program $R$ where the heads of clauses cannot use reserved predicates, and any occurrence of reserved predicates in clause bodies is well-typed
\end{itemize}

Consider the following example DC-PLP program:
\begin{example}[DC-PLP Program] \label{ex:dcproblog_program_without_dc_plpdc}
	This example program models the correct working of a machine.
	
\begin{problog*}{linenos}
rv(hot, flip(0.2)). 
rv(cooling(1), flip(0.99)). 
rv(temperature(hot), normal(27,5)).
rv(temperature(not_hot),normal(20,5)).

machine(1).
works(N):- machine(N), test(cooling(N)=:=1).
works(N):-
	machine(N),
	test(temperature(hot)<25.0),
	test(hot=:=1). 
works(N):-
	machine(N),
	test(temperature(not_hot)<25.0),
	test(hot=:=0). 

query(works(1)).
\end{problog*}
	We are now able to clearly identify the two components of a DC-PLP program. In the first part we see the random variables (representing independent choices). Here we also also included the probabilistic facts from the initial \dcproblogsty program. DC-PLP encodes probabilistic facts using the \probloginline{flip}\lstinline[columns=fixed]|/2| random function symbol, which returns either $1$ or $0$ with the probability given as the argument. The second block of code  contains the logic program.
\end{example}
\todo{be consistent on test vs holds}\ak{from a declarative / LP perspective, I prefer holds over test}

Here, \verb|flip/1| and \verb|normal/2| are distribution functors, \verb|=:=/2| and \verb|</2| are Boolean query functors written in infix notation, \verb|hot/0|, \verb|cooling/1|, and \verb|temperature/1| are random variable functors, and we do not have  arithmetic and regular functors. \todo{change / expand example?} 

\subsection{Validity}\label{sec:dcplpvalidity}
For a DC-PLP program $P=(D,R)$, let $V=\{v_1,v_2,\ldots\}$  be the set of  random variable terms appearing as first arguments in the facts in $D$, 
let $Q=\{q_1,q_2,\ldots\}$ be the set of all well-typed ground Boolean query terms  that can be built from the reserved vocabulary and $V$, and let $F=\{\mathtt{holds}(q_i)~|~q_i\in Q\}$ be the set of possible holds-atoms for these queries.

Given a program $P$ with facts \verb|rv|$(v_p,d_p)$ and \verb|rv|$(v_c,d_c)$ in $D$, the random variable $v_p$  is a \emph{parent} of the random variable $v_c$ if and only if  $v_p$ appears in $d_c$. We define \emph{ancestor} to be the transitive closure of \emph{parent}.\todo{example}

\begin{definition}\label{def:well-defd-facts}
The set $D$ is \emph{well-defined} if and only if it satisfies the following criteria:
\begin{enumerate}
\item For each atom \verb|rv|$(v_i,d_i)$ in $D$, $d_i$ is a well-defined distribution term for all possible values of the parents. \todo{is well-typed sufficient for this? if so, drop this point}
\item The ancestor relation is acyclic.
\item Each $v_i\in V$ has a finite set of ancestors.
\end{enumerate}  
\end{definition}

Let $\omega$ be an assignment that maps each random variable $v_i \in V$ to a possible value $\omega(v_i)$ from the associated distribution $d_i$. 
Such an $\omega$ induces a unique truth value assignment $b_{\omega}$ for the Boolean queries in $Q$, \ie, $b_{\omega}(q_i)=1$ if $q_i$ is true after setting all random variables to their values under $\omega$, and $b_{\omega}(q_i)=0$ otherwise. 
It further induces a unique truth value assignment $I_{\omega}$ to facts in $F$, \ie, $I_{\omega}(\mathtt{holds}(q_i))=b_{\omega}(q_i)$. We also write $F_{\omega}=\{\mathtt{holds}(q_i)~|~b_{\omega}(q_i)=1\}$, and refer to such a $F_{\omega}$ as a \emph{consistent fact database}. 



A program is \emph{valid} if and only if it satisfies the following criteria:
\begin{description}
\item[(C1)] $D$ is well-defined. 
\item[(C2)] All Boolean queries in $Q$ are Lebesgue-measurable.
\item[(C3)] For each consistent fact database $F_{\omega}$, the logic program $F_{\omega}\cup R$ has a two-valued well-founded model.  
\end{description}

\subsection{Semantics}
We follow the common practice of defining the semantics with respect to ground programs; the semantics of a program with non-ground $R$ is defined as the semantics of its grounding with respect to the  Herbrand universe.

Let $P$ be a valid DC-PLP program as defined above.

If $D$ is empty, \ie, $P$ does not define any random variables,  the semantics of $P$ is the well-founded model of $R$. Thus, normal logic programs are a special case of DC-PLP.\footnote{Note that in the absence of random variables, all well-typed Boolean queries, and thus all holds-atoms, have deterministic truth values.} In the following, we assume that $D$ is not empty. 

Our definition of the semantics closely follows Sato's distribution semantics, \ie, we also establish a probability measure over interpretations of a countable set of facts $F$ (the \verb|holds/1|-atoms), and extend this to one over Herbrand interpretations. The key differences are that (1) our measure over facts is in itself induced by a measure over value assignments to the random random variables and (2) we use normal logic programs with the well-founded model as canonical model instead of definite clause programs.


\subsubsection{Probability measure over random variables}
The (non-empty) set of facts $D$ introduces a  countable set of random variables $V=\{v_1,v_2,\ldots\}$, each associated with a distribution $d_i$.  Condition C1 ensures that these distributions are well-defined for every combination of parent values. It further ensures finite numbers of ancestors per random variable and an acyclic ancestor relation. As shown by  \citeauthor{kersting2000bayesian} \cite[Theorem 4.9]{kersting2000bayesian}, under these conditions, there exists a unique probability measure $P_V$ over the space of possible assignments to $V$ that for every finite set of random variables $V'\subseteq V$ closed under the ancestor relation factors into the distributions of the random variables in $V'$.

\subsubsection{Probability measure over (consistent) fact databases}
We now show that the probability measure $P_V$ over assignments to the random variables uniquely induces a probability measure $P_F$ over truth value assignments to the facts $F$; this is the \emph{basic distribution} in the distribution semantics.

We fix an arbitrary enumeration  $A_1=\mathtt{holds}(q_1),A_2=\mathtt{holds}(q_2),...$ of the atoms in $F$. 
Each $A_i$ \emph{depends} on a finite set $V_i$ of random variables, namely  those mentioned in $q_i$ as well as all their ancestors. We write $V_{\leq n}=\bigcup_{1\leq j\leq n}V_j $ for the union of random variables the first $n$ atoms in the enumeration depend on, and $P_{V_{\leq n}}$ for $P_V$ restricted to this set.  

By condition C2, all queries $q_i$ are  Lebesgue-measurable, and we thus get a family of distributions 
$$P_F^{(n)}(A_1=x_1,\ldots,A_n=x_n) = \int_{\Omega(V_{\leq n})} \mathbf{1}_{[q_1=x_1\wedge\ldots\wedge q_n=x_n]}(\omega)dP_{V_{\leq n}}(\omega) $$ where the $x_i$ are $0$ or $1$, $P_{V_{\leq n}}$ factorizes over the random variables in $V_{\leq n}$ as discussed above, $\Omega(V_{\leq n})$ denotes the space of possible assignments for variables in $V_{\leq n}$, and $\mathbf{1}_{[\varphi]}$ is the indicator function, \ie, equals $1$ if $\varphi$ is true and $0$ otherwise. The definition in terms of an indicator function and the measurability of the underlying Boolean queries ensures that this family of distributions is of the form required for the distribution semantics, \ie, they are well-defined probability distributions satisfying the compatibility condition. There thus exists a completely additive probability measure $P_F$ over the space of truth value assignments to $F$ such that for any $n$, we have
$$P_F(A_1=x_1,\ldots,A_n=x_n) =P_F^{(n)}(A_1=x_1,\ldots,A_n=x_n)$$
We note that by construction, this measure assigns mass to consistent fact databases only. 

\subsubsection{Probability measure over Herbrand interpretations}
In the last step, we follow Sato's construction to obtain a probability measure $P_P$ over Herbrand interpretations from $P_F$. To do so, we fix an enumeration $A_1,A_2,\ldots$ of all atoms in the Herbrand base, which includes those in $F$. 
Condition C3 ensures that for every consistent fact database $F_{\omega}$, the logic program $F_{\omega}\cup R$ has a total well-founded model $M_{\omega}$, and we can thus define   
$$P_P^{(n)}(A_1=x_1,\ldots,A_n=x_n) = P_F(\{F_{\omega}~|~ M_{\omega}\models A_1^{x_1}\wedge\ldots\wedge A_n^{x_n}\})$$ where $A^1=A$ and $A^0=\neg A$, and it again follows that there is a completely additive probability measure $P_P$ over Herbrand interpretations, which completes the definition of the semantics. 


==> files_old/dcproblog.tex <==
\section{\dcproblogsty Semantics}\label{sec:dcproblog}
While DC-PLP is an expressive probabilistic programming language for which we have defined fully declarative semantics, using DC-PLP in practice might turn out to be challenging. The syntax is simply too cumbersome. Therefore, we will now introduce semantics for the higher-level \dcproblogsty language whose syntax we already introduced in Section~\ref{sec:syntax}.




A \dcproblogsty program consists of a countable set of ground distributional facts, a countable set of ground probabilistic facts, and a logic program (i.e. a finite set of facts and normal clauses), where bodies of normal clauses can use comparison predicates.   


\begin{definition} A \dcproblogsty program \dcpprogram is {\bf valid} if and only if it encodes a unique probability distribution.
\end{definition} 

This raises the question: what are the conditions we have to impose on \dcproblogsty programs such that they are valid, or in other words such that they encode unique probability distributions? We will answer this question in Theorem~\ref{theo:valid_dcproblog}. But first we are going to define a program transformation that maps a \dcproblogsty program to a DC-PLP program.  





\begin{definition} \label{def:dcproblog2dcplp}


\todo{ make transformations formal with substitutions}

\pedro{@Angelika, I believe you mentioned you had this transformation ready already?}
\ak{see copy from old below for probabilistic facts; LP stays the same (modulo dropping the test-wrapping?); distributional facts should be just rv(v,d) to v\probloginline{~}d (the complicated part would be directly mapping full DC)}

\end{definition}

\ak{begin copy}
\subsubsection{ProbLog with probabilistic facts only}
ProbLog with probabilistic facts (no ADs) restricts $P$ to discrete distributions over Boolean truth values, and $Q$ to equality comparisons between a random variable and the constant \verb|true|. The translation is modular, mapping each normal logic clause to itself, and each ground probabilistic fact \verb|p::f| to a program fragment
\begin{verbatim}
rv(f,flip(p)).
f :- holds(f=true).
\end{verbatim}
where \verb|flip(p)| denotes the distribution that returns \verb|true| with probability \verb|p| and \verb|false| otherwise.\footnote{This assumes that all probabilistic facts are syntactically different and associated to a single probability; for the multi-set view of the current system, the name of the random variable has to be made unique through different means, which is straightforward.} The correspondence in semantics is straightforward. 

\subsubsection{ProbLog with ADs}
Adding ADs to ProbLog adds discrete distributions over finite sets $\{1,...,n\}$ to $P$, and equality comparisons between random variables and the elements of these sets to $Q$.
A ground AD \verb|p1::h1;...;pn::hn :- body| maps to a program fragment
\begin{verbatim}
rv(id,[p1:1,...pn:n]).
h1 :- body, holds(id=1).
...
hn :- body, holds(id=n).
\end{verbatim}
where \verb|id| is a fresh term not used anywhere else. The correspondence in semantics is again straightforward. 
\ak{end copy}




\begin{theorem} \label{theo:valid_dcproblog}
A \dcproblogsty program is valid if the following two validity conditions hold.
	\begin{itemize}
	    \item[V1] No two distributional facts can introduce the same random variable, \ie use the same term on the left hand side.
		\item[V2] The program \dcpprogram is distribution stratified, that is, there exists a function $rank(\cdot)$ that maps ground terms to $\mathbb{N}$ and that satisfies the following properties:
		\begin{enumerate}			
			\item for each ground instance of a distributional fact of the form \linebreak \probloginline{rand~dist(d@$_1$@,...,d@$_n$@)} it holds that   $rank(\text{\probloginline{rand}})>rank(\text{\probloginline{d@$_i$@}})$ for every $i$ ($1\leq i \leq n$).
			\item for each ground instance of another program clause \probloginline{h:- b@$_1$@,...,b@$_n$@} it holds that $rank(\text{\probloginline{h}})\geq rank(\text{\probloginline{b@$_i$@}})$, for all $i$.
			\item for each ground term \probloginline{b} that contains a random variable \probloginline{rand}, $rank(\text{\probloginline{b}})\geq rank(\text{\probloginline{rand~dist}})$ (with \probloginline{rand~dist} the head of the distributional clause defining \probloginline{rand}).
		\end{enumerate}
	    \item[V3] \todo{Lebesgue measurabiltiy of comparisons}
	\end{itemize}
\end{theorem}


\proof{\todo{}

\begin{itemize}
    \item use transformation from \dcproblogsty to DC-PLP and show uniqueness under conditions
    \item we need to show that the transformation is unique (order does not matter) and results in a valid DC-PLP program
\end{itemize}
}


\todo{Discuss complexity/decidability of determining whether program is valid, cf. \citep[Chapter 4.5]{milch2006probabilistic}. discuss sufficiency not necessity of validity conditions. maybe disucss in dc-plp section }








\section{\dcproblogsty with Distributional Clauses}



\begin{example}[\dcproblogsty Program] \label{ex:dcproblog_distributional_clause}
	This example program models the correct working of a machine. The probability distribution of the \probloginline{temperature} of the machine depends on whether it is a \probloginline{hot} day or not.
	\begin{problog*}{linenos}
machine(1).

0.2::hot.
0.99::cooling(1).

temperature ~ normal(27,5):- hot.
temperature ~ normal(20,5):- \+hot. 

works(N):- machine(N), cooling(N).
works(N):- machine(N), temperature<25.0. 

query(works(1)).
	\end{problog*}
	Note that we introduced {\em distributional clauses} in this example, which let us write down conditional probability distributions. 
\end{example}






\begin{definition}
	Distributional clauses are syntactic sugar to concisely write down conditional probability distributions of random variables. \todo{more elaborate}

	
\end{definition}




\begin{definition}




\todo{formal transformation: \dcproblogsty with distributional clauses to \dcproblogsty without}
	A \dcproblogsty program containing a random variable \probloginline{rand} involved in $N$ distributional clauses
    \begin{problog}
rand ~ dist@$_i$@ :- b@$_i$@
    \end{problog}
	with mutually logically inconsistent bodies $\text{\probloginline{b@$_i$@}}$ ($1{\leq} i {\leq} N$)
	is equivalent to a \dcproblogsty program with $N$ fresh random variables \probloginline{rand@$_i$@} ($1{\leq} i {\leq} N$) involved in $N$ distinct distributional facts
    \begin{problog}
rand@$_i$@ ~ dist@$_i$@.
    \end{problog}
    Each clause initially containing \probloginline{rand} is replaced in the equivalent program that does not contain distributional clauses for \probloginline{rand} by $N$ clauses, where \probloginline{rand} is substituted by $\text{\probloginline{rand@$_i$@}}$ and its body is conjoined with \probloginline{b@$_i$@} for every i with $1{\leq} i {\leq} N$.

\end{definition}



Mapping distributional clauses to distributional facts is akin to mapping intentional probabilistic facts (e.g \probloginline{0.2::a:- b.}) to probabilistic facts (and deterministic rules). Note that \dcproblogsty allows, just as \problogsty, the usage of intentional probabilistic facts, with the same semantics as in \problogsty. In absence of any distributional facts and clauses, a \dcproblogsty program reduces to a \problogsty program.


\begin{theorem}\label{theo:valid_dcproblog_w_clauses} A {\bf \dcproblogsty program} \dcpprogram{} {\bf with distributional clauses} is {\bf valid} if it can be mapped to an equivalent valid \dcproblogsty program. Such a mapping exists if the following three validity conditions hold.
	\begin{itemize}
		\item[V1] The bodies of ground distributional clauses with the same random variable in their heads are pairwise logically inconsistent.
		\item[V2] The program \dcpprogram is distribution stratified, that is, there exists a function $rank(\cdot)$ that maps ground terms to $\mathbb{N}$ and that satisfies the following properties:
		\begin{enumerate}			
			\item for each ground instance of a distributional clause of the form \linebreak \probloginline{rand~dist(d@$_1$@,...,d@$_n$@):-b} it holds that   $rank(\text{\probloginline{rand}})>rank(\text{\probloginline{d@$_i$@}})$ for every $i$ ($1\leq i \leq n$).
			\item for each ground instance of a distributional clause \probloginline{rand~dist:-b@$_1$@,...,b@$_n$@} it holds that $rank(\text{\probloginline{rand ~ dist}})>rank(\text{\probloginline{b@$_i$@}})$, for all $i$.
			\item for each ground instance of another program clause \probloginline{h:- b@$_1$@,...,b@$_n$@} it holds that $rank(\text{\probloginline{h}})\geq rank(\text{\probloginline{b@$_i$@}})$, for all $i$.
			\item for each ground term \probloginline{b} that contains a random variable \probloginline{rand}, $rank(\text{\probloginline{b}})\geq rank(\text{\probloginline{rand~dist}})$ (with \probloginline{rand~dist} the head of the distributional clause defining \probloginline{rand}).
		\end{enumerate}
	    \item[V3] \todo{Lebesgue measurabiltiy of comparisons}
	\end{itemize}

\proof{transform distributional clauses to distributional facts.

}
\end{theorem}

The criterion V1 in Theorem~\ref{theo:valid_dcproblog_w_clauses} is equivalent to the validity criterion V1 given in~\citep[Definition 3]{gutmann2011magic}, which requires that there is a unique ground distribution for each ground random variable \probloginline{rand}. V2 is a carbon copy of the second validity criterion of~\citep[Definition 3]{gutmann2011magic}, with the exception of the first point of V2. We added it, as distributional clauses with cyclic functional dependencies were not {\em explicitly} disallowed in ~\citep{gutmann2011magic}.

\subsection*{Difference to Distributional Clauses}

\ak{discussion on differences to DC: in how far is this semantics vs implementation? I believe we silently assumed (but never stated) that only defined RVs would be used, but I don't remember how Davide handled this when introducing negation to the semantics...}

This is also a good point to illustrate a major difference between the semantics of random variables in Distributional Clauses and \dcproblogsty. Take the code snippet below:
\begin{problog*}{linenos}
x ~ normal(20,2).

q(1):- x>20.
q(2):- y>20.

query(q(1)).
query(q(2)).
\end{problog*}
The first query succeeds and returns as an answer $p(\text{\probloginline{query(q(1)))}}) = 0.5$. The second query, however, throws an error as there is no term of type \type{RandomVariable} declared that is named \probloginline{y}. The second query would also fail if there were an \type{Atom} term named \probloginline{y}. In this case the lefthand side of \probloginline{y>20} would be ill-typed.

Let us now write the same program as a Distributional Clauses program:
\begin{adjustwidth}{1em}{0em}
	{
		\normalfont
		\begin{lstlisting}[breaklines,mathescape]
x ~ normal(20,3).

q(1)$\leftarrow$ $ {\simeq}(x)$<20.
q(2)$\leftarrow$  $ {\simeq}(y)$<20.

query(q(1)).
query(q(2)).
		\end{lstlisting}
	}
\end{adjustwidth}
The first query will again return $ p(\text{\lstinline|query(q(1))|}) =0.5$ (or an approximation thereof) but the second query will not throw an error but return a probability of zero. How does this work? The term \lstinline[mathescape]|$ {\simeq} (y)$| tries to unify with the value of the random variable \lstinline|y|. As there is no such random variable, this silently fails and the body of the clause whose head is \lstinline|q(2)| is simply not satisfied.

If we were to negate the comparison predicate in the body of the \lstinline|q(2)| clause, \ie write:
\begin{adjustwidth}{1em}{0em}
	{
		\normalfont
		\begin{lstlisting}[breaklines,mathescape]
q(2) $\leftarrow$  \+(${\simeq}(y)$<20).
		\end{lstlisting}
	}
\end{adjustwidth}
we would obtain for the second query: $ p(\text{\lstinline|query(q(1))|}) =1$. Negating the corresponding comparison predicate in \dcproblogsty would still result in an ill-typed term, \ie an error would be thrown.

The comparison we just performed does not only illustrate a semantic difference between \dcproblogsty and Distributional Clauses but also a conceptual one. In \dcproblogsty the values of of random variables never enter the realm of the logic program: values of random variables only live in the external arithmetic engine of \dcproblogsty. In contrast,  random variables in Distributional Clauses are part of the logic program: the values of random variables are stored in a logic data base and can be accessed through logical unification. Distributional Clauses currently does this via SLD resolution.


==> files_old/early_examples.tex <==
\section{Motivating examples}
\dcproblogsty is a probabilistic logic programming language derived from two related but separate probabilistic logic programming languages,  \problogsty and Distributional Clauses (DC).
It inherits its Prolog syntax and the concept of probabilistic facts from \problogsty, and combines this with the ideas to define and query continuous random variables in DC, using DC's infix 
\probloginline{~}\lstinline[columns=fixed]|/2| predicate to define  {\em distributional facts}. Distributional facts allow a user to express random variables that are distributed according to a certain probability distribution specified by a random function symbol.

In the following example, the distributional fact in line 3 introduces the random variable \verb|temperature| and associates it with the distribution term \verb|normal(20,5)|. This random variable is then queried in the clause in line 8 using comparison predicate \verb|</2|, again written in infix notation. 
\begin{example}\label{example:dcproblog_machine}
	In this example we model the temperature as a continuous random variable distributed according to a normal distribution with mean $20$ and standard deviation $5$ (Line \ref{program:dcproblog_machines_temp}).
	\begin{problog*}{linenos}
machine(1). machine(2).

temperature ~ normal(20,5). @\label{program:dcproblog_machines_temp}@
0.99::cooling(1).
0.95::cooling(2).

works(N):- machine(N), cooling(N).
works(N):- machine(N), temperature<25.0. @\label{program:dcproblog_machines_work_temp}@

evidence(works(2)).  @\label{program:dcproblog_machines_evidence}@
query(works(1)).
	\end{problog*}
\end{example}


Distributional facts are not limited to describe continuous random variables but can, for example, also model discrete probability distributions, of which an example would be the Poisson distribution.
\begin{example}\label{example:dcproblog_poisson_population}
	In this example we show how to model the size of a group of people as a Poisson distribution and answer queries about the size of the group using the comparison predicates  \probloginline{>}\lstinline[columns=fixed]{/2} and \probloginline{=:=}\lstinline[{columns=fixed}]{/2}.
	\begin{problog*}{linenos}
n_people ~ poisson(6).

more_than_five:- n_people>5@.@
exactly_five:- n_people=:=5@.@

query(more_than_five).
query(exactly_five).
	\end{problog*}
	
\end{example}

We will formally introduce \dcproblogsty in Section~\ref{}. To introduce the semantics, in the next Section, we start by introducing DC-PLP, an abstract version of the language that omits syntactic sugar. 





==> files_old/implementation.tex <==
\section{Implementation} \label{sec:implementation}
\ak{needs an introduction (and I'd suggest reorganization into algorithms first, then system)}
We make two observations:
\begin{enumerate}
    \item Every implementation of \prologsty  (or any other logic programming language)  reserves a set of {\em  system predicates} executing code not written in pure \prologsty~\citep[Chapter 8]{sterling1994art}.
    System predicates complement pure \prologsty implementations and give users access to efficient algorithms that are cumbersome to implement in pure logic programming -- for instance algorithms for numeric computations.
    \item In Section~\ref{sec:semantics} we have seen that we can separate a probabilistic logic program into a set of independent random choices and a logic program. The independent choices and the logic program communicate to each other via comparison predicates. Comparison predicates are an instance of system predicates.
\end{enumerate}

These observations hint at the possibility of implementing \dcproblogsty as a deterministic logic programming language with access to an external engine with support for random variables.
On an implementation level, the key difference between a probabilistic logic programming language and a (deterministic) logic programming language is the availability of probability distributions in the external engine of the former.

Decoupling independent choices (random variables) and the deterministic system (logic program) does also mean that we should be able to take a probabilistic logic programming language that only supports finite discrete probability distributions and extend it with continuous probability distributions.
We will demonstrate how to achieve this by adding continuous random variables to the ProbLog2 system~\citep{dries2015problog2} (the most recent implementation of \problogsty). We dub our implementation \dcproblogsys.

% First, we will introduce a type system 
% (Section~\ref{sec:type_system}), followed by a description of how a type system aids the extension of the ProbLog2 system with continuous random variables (Section~\ref{sec:external_engine}).
% Followed by a description of the system architecture of \dcproblogsty in Section~\ref{sec:architecture}, which is based on the \problogsys architecture~\citep{dries2015problog2} and which we dub \dcproblogsys.








% To this end we will first introduce a type system (Section~\ref{sec:type_system}), followed by a description of how a type system aids the extension of the ProbLog2 system with continuous random variables (Sections~\ref{sec:multiple_dispatch} and~\ref{sec:external_engine}).
% Lastly, we will also discuss the implementation of ALW (cf. Section~\ref{sec:inference}) and how it uses the existing inference mechanisms already present in the ProbLog2 system.













\subsection{\dcproblogsty System Architecture}
\label{sec:architecture}

\dcproblogsys, is built on top of the existing \problogsys system. This means we inherit the general architecture of performing inference via a number of deterministic program transformations performed on the source program (written in \dcproblogsty). Figure~\ref{figure:dcproblog_sys} summarizes the program transformation steps in \dcproblogsys. These are grounding, cycle breaking, compiling, and evaluating. Conceptually the transformations are identical to the ones performed in the \problogsys implementation.
% We will briefly describe the four transformations and give a more detailed account of the compilation and evaluation steps in Section~\ref{sec:inference} as these are the steps where \dcproblogsys and \problogsys differ most.

\begin{figure}[h]
	\centering
	\includegraphics[width=\linewidth]{figures/dcproblog_sys.pdf}
	\caption[Overview of the program transformation steps in the \dcproblogsys system]{Overview of the program transformation steps in the \dcproblogsys system. (Figure inspired by~\protect\citep[Figure 2]{zuidbergdosmartires2019transforming}.}
	\label{figure:dcproblog_sys}
\end{figure}

%%% moved from elsewhere
\subsection{Conditional \dcproblogsty Programs}
\ak{this is not the right place for the sec; just moved it from the language section as it is about system}

This lets us, for instance, compute the probability of the query in Example~\ref{example:dcproblog_machine}, where we saw that we can express a conditional probability by using the reserved \probloginline{evidence/1} predicate. \dcproblogsty also has a binary predicate \probloginline{evidence/2}, where the second argument is either the \probloginline{true} symbol or the \probloginline{false} symbol. The former is equivalent to using the unary version, while the latter allows one to express negative evidence. These predicates are also present in \problogsty.



While the \probloginline{evidence} predicate allows us to express conditional probabilities where we condition on Boolean random variables, its semantics does not extend directly to conditioning on continuous random variables: a continuous random variable can neither be true nor false. In order to allow a user to condition on continuous random variables in \dcproblogsty, we introduce the \probloginline{observation/2} predicate.

\begin{example}\label{example:dcproblog:observation}
	We model the size of a ball as a mixture of  different beta distributions, depending on whether the ball is made out of wood or metal (Line~\ref{program:dcproblog_machines_observation:ad})\footnote{Annotated disjunctions are used to concisely write down mutually exclusive Boolean random variables. Internally they are compiled down to probabilistic facts and deterministic rules.}.
	We would now like to know the probability of the ball being made out of wood given that we have a measurement of the size of the ball. In order to condition on a continuous random variable we introduce the \probloginline{observation/2} predicate, which has an analogous functionality as the evidence predicates for Boolean random variables.
	\begin{problog*}{linenos}
3/10::material(wood);7/10::material(metal).@\label{program:dcproblog_machines_observation:ad}@

size~beta(2,3):-material(metal)@\label{example:dcproblog:observation:beta23}@.
size~beta(4,2):-material(wood).

observation(size,4/10).
query(material(wood)).
	\end{problog*}
	This \dcproblogsty program encodes the conditional probability:
	\begin{align}
		p(\text{\probloginline{material(wood)}}| \text{\probloginline{size=4/10}})
	\end{align}
\end{example}



%%% end moved from elsewhere

\ak{if we keep this overview, include pointers to the sections that discuss details}
\paragraph{\bf Grounding}

\dcproblogsys is an extension of the \problogsys system: the logic programming components in both systems are identical. This means that we can simply bootstrap the logic grounding engine of the \problogsys system for \dcproblogsys. Grounding is performed using {\em selective linear definite clause} (SLD) resolution~\citep{kowalski1974predicate,sterling1994art}. SLD resolution allows for computing the relevant ground program for a specific query to the logic program, which avoids grounding of unnecessary predicates~\citep{kersting2000bayesian,fierens2015inference}.\ak{what about negation? SLDNF or something else?}

\paragraph{\bf Cycle Breaking} Logic programs may contain cycles. In order to perform inference these need to be removed from the ground program. As these cycles only occur in the logic program part of a \dcproblogsty program we can again bootstrap the cycle breaking available in \problogsys, which is currently a variation of the algorithm proposed in~\citep{janhunen2004representing} \citet{mantadelis2010dedicated} have also proposed an alternative cycle breaking algorithm.

\paragraph{\bf Compiling} The next step that \problogsys performs to compute probabilities is the compilation of acyclic ground programs. Acyclic ground programs have a one-to-one mapping to propositional logic formulas, which are then compiled into decision diagrams in a process dubbed knowledge compilation~\citep{darwiche2002knowledge}. \dcproblogsys differs in that acyclic ground \dcplpsty programs are not mapped to propositional logic formulas but to so-called {\em satisfiability modulo theory} (SMT) formulas (\eg $x>3$)~\citep{barrett2009handbook}, which are then compiled to decision diagrams that support algebraic constraints~\citep{sanner2011symbolic,zuidbergdosmartires2019exact}.


\paragraph{\bf Evaluating} The probability of a query to a (hybrid) logic program is obtained by evaluating the compiled logic formula (decision diagram). While in \problogsys this is performed using the weighted model counting (WMC)~\citep{chavira2008probabilistic} framework, \dcproblogsys uses weighted model integration~\citep{belle2015probabilistic} -- an extension of WMC that allows also for algebraic constraints on random variables.

\bigbreak

We provide the necessary background on knowledge compilation, weighted model counting, weighted model integration, and SMT formulas in~\ref{app:amc}, \ref{app:compilation}, and
\ref{app:wmi}.


\subsection{Grounding}
As already mentioned, grounding in \dcproblogsys is performed by bootstrapping the existing grounding engine of \problogsys. The sole minor difference concerns the grounding of comparison predicates, \eg (\probloginline{1<2}), (\probloginline{x>20}).
During the grounding of a \dcproblogsty program, the types of the comparison's arguments are checked and the comparison is considered to be proven if the types of the arguments match the type signature of the comparison predicate.
The possible types of a comparison's predicate arguments are dictated by the external arithmetic engine. For instance, \prologsty only allows for (deterministic) numbers, in contrast to \dcproblogsty where the external arithmetic engine also allows for comparing random variables.\ak{what if typecheck fails?}

More concretely, if a comparison predicate of the form (\probloginline{x>20}) is encountered during the grounding, the engine checks whether there are distributional facts of the form \probloginline{x ~ Dist} present in the program. If such a clause is present, the type of \probloginline{x} is inferred from the distribution \probloginline{Dist}. The comparison predicate is proven if the external engines allows for comparing the inferred types, \eg can the external arithmetic engine compare continuous random variables to real valued numbers. We give a more detailed account of typing and the external arithmetic engine in \ref{app:types}.


\subsection*{Evaluation of Comparison Predicates}

A distinctive property of comparison predicates in \dcproblogsty is that they have a potential infinite and uncountable number of groundings, \ie an infinite number of possible assignment to the variables in the arguments that would satisfy the comparison\ak{careful with grounding (replacing logical variable by ground terms) vs evaluating (replacing random variable by its value)}.
This cannot to be carried out using a logic grounding engine.
Therefore, we have to defer the grounding of comparison predicates to a later stage of the inference mechanism and at the same time retain a symbolic representation of the set containing all possible groundings. Probabilistic inference then constitutes of {\em measuring} the size of these sets using integration.
We call the grounding of a system predicate also an evaluation, as the external engines performs an arithmetic evaluation in the background.

In the special case of a `deterministic' comparison, \ie a comparison not containing any random variables in its arguments, we can interleave the grounding with the evaluation of the predicate.
That is, we can replace the atom with its corresponding Boolean value. For the comparison (\probloginline{1<2}) we would get \probloginline{true}. Such a type dependent eager evaluation during grounding can be regarded as an instance of multiple dispatch: differently typed predicates induce different run time behavior~\citep{castagna1995calculus}.

Eager evaluation of arithmetic expressions makes most sense when this leads to simplifications of the ground program. More concretely, when a comparison predicate is not satisfied this results in a \probloginline{false} atom and proving a goal during grounding can be stopped pre-maturely.
Eager evaluation of the comparison predicates allows \dcproblogsty to retain the usual behavior of proving and grounding in \problogsty where a proof fails if a (deterministic) comparison is not satisfied.

Depending on the arithmetic engine deployed, eager evaluation is also possible for evaluations of non-deterministic arithmetic expressions. If the evaluation of arithmetic expressions is purely sampling-based, the random variables in an arithmetic expression are replaced by sampled values. For each sample the arithmetic expressions can then be eagerly evaluated. This is the approach taken by~\citet{nitti2016probabilistic}.\ak{we need to be more explicit about this entire "external engine" stuff; right now, remarks about alternative engines are mingled into the description of a pipeline that seems to be fixed to one such engine (sampling here, Prolog earlier)}

% For symbolic arithmetic engines it does also make sense to perform eager evaluations to some degree. Consider the comparison (\probloginline{3+5>2+1}). A purely symbolic external engine would evaluate two symbolic expression trees and wrap the comparison into a \probloginline{holds}\lstinline[columns=fixed]|/1| predicate. Eagerly evaluation the expression tree however lets us replace the \probloginline{holds(3+5>2+1)} with \probloginline{false}.


\begin{example}[\dcproblogsty grounding] \label{example:grounding}
Consider the non-ground \dcproblogsty program below.

	\begin{problog*}{linenos}
0.2::hot.
0.99::cooling(1).

temperature(1) ~ normal(27,5):- hot.
temperature(1) ~ normal(20,5):- \+hot.

works(N):- cooling(N).
works(N):- temperature(N)<25.0.

query(works(1)).
	\end{problog*}
The grounding mechanism in \dcproblogsys is the same one as in \problogsys and only works on pure logic programs. However, the logic program and the random variables are still interleaved. In a first step we remove syntactic sugar and rewrite the distributional clauses and probabilistic facts  as distributional facts, cf. Section~\ref{sec:semantics}.
	
	\begin{dcplp*}{linenos}
rv_1_hot ~ flip(0.2). @\label{line:dist_hot}@
map(rv_hot,rv_1_hot).
hot:- map(rv_hot,R), R=:=1.

rv_1_cooling(1) ~ flip(0.99). @\label{line:dist_cooling}@
map(rv_cooling(1),rv1_cooling(1)).
cooling(1):- map(rv_cooling(1),R), R=:=1.

rv_1_temperature(1) ~ normal(27,5). @\label{line:dist_temp_1}@
map(rv_temperature(1), rv_1_temperature(1)):- hot.

rv_2_temperature(1) ~ normal(20,5). @\label{line:dist_temp2}@
map(rv_temperature(1), rv_2_temperature(1)):- \+hot.

works(N):- cooling(N).
works(N):- map(rv_temperature(N),R) , R<25.0.

query(works(1)).
	\end{dcplp*}
After removing the syntactic sugar we have a \dcplpsty program constituted of distributional facts in Lines~\ref{line:dist_hot}, \ref{line:dist_cooling}, \ref{line:dist_temp_1} and \ref{line:dist_temp2}, and a (non-probabilistic) logic program in the remaining lines. The logic  part of the \dcplpsty program can now be grounded using the \problogsys grounding engine:
	
	\begin{dcplp*}{linenos}
rv_1_hot ~ flip(0.2). 
rv_1_cooling(1) ~ flip(0.99). 
rv_1_temperature(1) ~ normal(27,5).
rv_2_temperature(1) ~ normal(20,5).

map(rv_hot,rv_1_hot).
map(rv_cooling(1),rv_1_cooling(1)).
map(rv_temperature(1), rv_1_temperature(1)):- hot.
map(rv_temperature(1), rv_2_temperature(1)):- \+hot.

hot:- map(rv_hot,), rv_1_hot=:=1.
cooling(1):-
    map(rv_cooling(1),rv_1_cooling(1)), 
    rv_1_cooling(1)=:=1.
works(1):- cooling(1).
works(1):-
    map(rv_temperature(1),rv_1_temperature(1)) ,
    rv_1_temperature(1)<25.0.
works(1):-
    map(rv_temperature(1),rv_2_temperature(1)) 
    rv_2_temperature(1)<25.0.

query(works(1)).
	\end{dcplp*}
As there are no cycles present in the \dcplpsty program above, we do not need to perform cycle breaking on the logic program part.
\end{example}

Note that for, the sake of clarity, we performed the rewriting of a \dcproblogsty program to a \dcplpsty program in Example~\ref{example:grounding} as a separate and preliminary step. In the \dcproblogsys implementation the elimination of syntactic sugar is interleaved with the grounding and performed on the fly. This avoids rewriting parts of the program that are irrelevant to computing the probability of a query.\ak{why/when is grounding on the fly possible?}










%%%%%%%%%%%%%%%%%%%%

















% In probabilistic programming a recent trend has emerged of mixing eager evaluation (usually in combination with sampling based probabilistic inference) and lazy evaluation (also called delayed evaluation). Examples for this are the probabilistic programming languages Birch~\citep{murray2018automated} or the symbolic probabilistic programming language PSI~\citep{gehr2016psi}. Lazy evaluation of arithmetic expressions do also allow to simplify probabilistic programs such that inference becomes tractable after these simplifications. An obvious example for this is then rewriting a conjugate prior-likelihood pair into a single expression. Lazy evaluation combined with symbolic simplifications goes into the direction of compiling probabilistic programs, \eg~\citep{wu2016swift}.


% The key difference between the external arithmetic engine of \prologsty (or \problogsty) and the external arithmetic engine of \dcproblogsty is that the external engine of the latter is capable of performing arithmetic operations (perform evaluations) with random variables. Combining this innovation with multiple dispatch allows us to retain the same syntax (same functor) to perform arithmetic operations on \type{SymbolicRV} terms and/or \type{Number} terms.








% \subsubsection{Arithemtics of Random Variables}

% Evaluating arithmetic expressions that contain random variables should not to be confused with performing arithmetic operations on random variables. Writing \probloginline{x+y} in a comparison predicate, where \probloginline{x} and \probloginline{y} are random variables has the semantics of evaluating both random variables (for instance by drawing a sample) and adding up both evaluations.

% In order to perform arithmetic operations on random variables directly, we would need to introduce syntax and an arithmetic engine for random variables. This could, for example, be achieved in the following fashion:
% \begin{problog*}{linenos}
%  x ~ normal(20,5).
%  y ~ normal(25,6).
%  z ~ x+y.
% \end{problog*}
% In this case z would be a normal distribution with mean ($20{+}25$) and standard deviation ($5{+}6$). We leave arithmetic operations on random variables for future research.\pedro{maybe add citation of somebody who has done something like this already?}















%%%%%%%%%%%%%%%%%%%%







\subsection{Mapping Acyclic Ground \dcproblogsty to Weighted SMT Formulas}

In \problogsys, a query to a probabilistic program is mapped to a weighted propositional formula~\citep{fierens2015inference}. The probability of the query being satisfied is then the weight of the propositional formula. This weight is also called the {\em weighted model count}~\citep{darwiche2009modeling}.
Inference in \dcproblogsys follows a similar principle, with the difference that a hybrid probabilistic program is mapped to a weighted SMT formula, instead of a weighted propositional formula.
The weight of a weighted SMT formula is called the {\em weighted model integral}.
% Weighted model integration (WMI)~\citep{belle2015probabilistic} generalizes weighted model counting in that it also allows for continuous variables.

The probability of a query \probloginline{query(q)} in a \dcproblogsty program is obtained by computing the probability of an equivalent weighted SMT formula using weighted model integration:
\begin{align}
	p(\text{\probloginline{query(q)}})= p(\support_q) = \wmi(\support_q, w_q)
\end{align}
where $\support_q$ denotes the SMT formula and $\weight_q$ the associated weight.

% We first encode a query to a \dcproblogsty program as a weighed logic formula and present then algebraic likelihood weighting (ALW), a probabilistic inference algorithm that computes the weight of a logic formula in the discrete-continuous domain in the context of probabilistic logic programming.

% We just mapped the probability encoded by a \dcplpsty program to a weighted model integral. Inference in \dcplpsty/\dcproblogsty can hence be performed by any algorithm capable of computing the weighted model integral in question.


\begin{example}[Mapping \dcplpsty to WMI] Consider again the \dcplpsty program in Example~\ref{ex:dcproblog_program_without_dc_plpdc}. If we ground the purely logic component of the program we obtain the ground program .
\begin{dcplp*}{linenos}
hot ~ flip(0.2). 
cooling(1) ~ flip(0.99). 
temperature(hot) ~ normal(27,5).
temperature(not_hot) ~ normal(20,5).

machine(1).
works(1):- machine(1), cooling(1)=:=1.
works(1):-
	machine(1),
	temperature(hot)<25.0,
	hot=:=1. 
works(1):-
	machine(1),
	temperature(not_hot)<25.0,
	hot=:=0. 

query(works(1)).
	\end{dcplp*}
	We map the acyclic ground logic program and the Boolean queries to an SMT formula $\support_q$:
	\begin{align}
		\support_q
		&\leftrightarrow \text{\dcplpinline{machine(1)}} \land (\text{\dcplpinline{cooling(1)}}=1) \lor \nonumber \\
		&\phantom{{}\leftrightarrow{}} \text{\dcplpinline{machine(1)}} \land (\text{\dcplpinline{temperature(hot)}}<25.0) \land (\text{\dcplpinline{hot}}=1) \lor \nonumber \\
		&\phantom{{}\leftrightarrow{}} \text{\dcplpinline{machine(1)}} \land (\text{\dcplpinline{temperature(not_hot)}}<25.0) \land  (\text{\dcplpinline{hot}}=0) \nonumber \\
		&\leftrightarrow (\text{\dcplpinline{cooling(1)}}=1) \lor \nonumber \\
		&\phantom{{}\leftrightarrow{}} (\text{\dcplpinline{temperature(hot)}}<25.0) \land (\text{\dcplpinline{hot}}=1) \lor \nonumber \\
		&\phantom{{}\leftrightarrow{}} (\text{\dcplpinline{temperature(not_hot)}}<25.0) \land  (\text{\dcplpinline{hot}}=0)  
	\end{align}
	The weight function $w_q$ is simply obtained by multiplying together the functions corresponding to the random variables declared in the \dcplpsty program.
\end{example}


























\subsection{Correctness of the Transformations}

In Algorithm~\ref{algo:inference_dc_problog} we outline the steps that are performed to map a \dcplpsty program to a weighted SMT formula. They closely follows the steps presented in~\citep[Section 5]{fierens2015inference}. 
\ak{the query should be an inout of the alg as well (note that the Boolean queries in the program are the comparison atoms, not the inference query)}

\begin{mdframed}
	\begin{algo}[\dcplpsty to Weighted SMT] \label{algo:inference_dc_problog}
		The algorithm takes as input a \dcplpsty program \dcpprogram, consisting of a countable set $P$ of ground distributional facts, a countable set of measurable Boolean queries $Q$, and a purely logic program $L$. The algorithm then maps $\dcpprogram$ through the following steps to a weighted SMT formula $(\support_q, \weight_q)$.
		\begin{enumerate}
			\item Ground out the purely logic program $L$ of $\dcpprogram$ with respect to a query $q$ and obtain the ground program $L_g$. This will also ground the Boolean queries in $Q$, leading to $Q_g$.
    		\item Break cycles in the ground logic program $L_g$.
			\item Convert the ground logic program consisting of $L_g$ and the set of measurable queries $Q_g$ to an equivalent SMT formula $\support_q$.
			\item Define a weight function $\weight_q$, which corresponds to the countable set of random variables in $P$.
		\end{enumerate}
	\end{algo}
\end{mdframed}


\begin{theorem}
The probability of a query $q$ to a valid \dcplpsty program $\dcpprogram$ can be expressed as a weighted model integral of a weighted SMT formula $(\support_q, \weight_q)$.\ak{too vague for a thm? why not make it concrete?}
\end{theorem}

\proof{The proof consists of showing that we can formulate the relevant ground program $L_g$ of the program $\dcpprogram$ with respect to the query $q$ as an SMT formula, that we can map the  }



\todo{work this in after Section 2 and 3 are written}

Let us consider the definition of weighted model integration given in \ref{app:wmi} and in particular the formulation given in Equation~\ref{eqn:wmi_sum_ive_weight}.
\begin{align}
	\wmi(\support, \weight) = \sum_{\langle\wsupport_i,\wweight_i\rangle \in \wtuples_f} \sum_{\bvars} \int \ive{\wsupport_i(\xvars, \bvars)} \wweight_i(\xvars) d\xvars 
\end{align}


Comparing the definition of the probability of a \dcplpsty program to the definition weighted model integration, and in particular the form of WMI given in Equation~\ref{eqn:wmi_sum_ive_weight}:
\begin{align}
	\sum_{\langle\wsupport_i,\wweight_i\rangle \in \wtuples_f} \sum_{\bvars} \int \ive{\wsupport_i(\xvars, \bvars)} \wweight_i(\xvars) d\xvars 
\end{align}
We cannot but appreciate the striking similarity between both Equations. The only substantial difference is that Equation~\ref{eq:definition_probability_dcplp} uses Lebesgue integration to marginalize out Boolean random variables, whereas Equation~\ref{eqn:wmi_sum_ive_weight} uses a summation. Other than that it is straight forward to map one equation to the other:

\begin{itemize}
	\item We associate the sum over the models $l \in MOD(L)$ to the sum over different SMT(\lra) formulas $\wsupport_i$ in weighted model
	\item We associate a specific product of Iverson brackets of Boolean queries $\prod_{q \in Q(l)} \ive{q}$ to the Iverson bracket of a specific SMT(\lra) formula $\ive{\wsupport_i}$, which is a conjunction of atomic SMT(\lra) formulas.
	\item We associate the distributions in $ D_l$ with the weight function $\wweight_i$.
\end{itemize}
\todo{end}

































==> files_old/inference.tex <==

\section{Computing Probabilities}\label{sec:inference}


In the previous section we saw how to implement \dcproblogsty using components of the existing \problogsys system. More specifically, we delineated how the first two program transformations in the \dcproblogsys implementation (grounding and cycle breaking) relate to analogous steps in \problogsys.
In order to calculate probabilities, we will now show how the compilation and evaluation steps from \problogsys can be adapted in such a way that they can accommodate continuous random variables as well.



\subsection{Conditional Queries}

\ak{this section is semantics; at least the conceptual parts discussing different types of observations etc should probably move to sec \ref{sec:inference-tasks}}



For \dcproblogsty programs that include evidence on logic atoms the probability is simply obtained by computing two weighted model integrals, one for the evidence $\support_e$ and one for the conjunction of the evidence with the query $\support_e \land \support_q$:
\begin{equation}
	p(\support_q|\support_e)=\frac{p(\support_q,\support_e)}{p(\support_e)}=\frac{\wmi(\support_q \land \support_e,w_{qe})}{\wmi(\support_e,w_e)}
\end{equation}


As the probability of a random variable with uncountably many outcomes taking a specific value is zero, conditioning with \probloginline{observation/2} is slightly more complicated. Consider the program in Example~\ref{example:dcproblog:observation}. The probability of the the conditioning set is zero:
\begin{equation}
	p(\text{\probloginline{observation(size,4/10))}}=p(\text{\probloginline{size}=4/10})=0
\end{equation}
Were we to apply the same approach as for conditional queries with \probloginline{evidence}, we would obtain a division by zero and consequently an undefined conditional probability. 
This problem is related to the Borel-Kolomogorov paradox~\citep{kolmogorov1950foundations,gyenis2017conditioning}, which is again caused by a zero-division.

We will, analogously to \citet{nitti2016probabilistic},   follow~\citet{kadane2011principles} to resolve the division by zero issue.
We make the explicit distinction between the probability $P$ and the probability density function $p:\frac{d}{dx}P(X \leq x)=p(x)$. The conditional probability is defined as:
\begin{align}
	P(\support_q| \support_e)
	&=P(\support_q|rv=v) & (\support_e \leftrightarrow rv=v )\\
	&=\lim_{\Delta v\rightarrow 0} \frac{P(\support_q,rv \in [v-\nicefrac{\Delta v}{2},v+\nicefrac{\Delta v}{2}])}{ P(rv \in [v-\nicefrac{\Delta v}{2},v+\nicefrac{\Delta v}{2}])} \label{equ:borel_limit} \\
	&=\lim_{\Delta v\rightarrow 0} \frac{\int \ive{ \support_q(x,rv=v)} p(x,rv=v)dx \cancel{\Delta v}}{p(rv=v)\cancel{\Delta v}} \\
	&=\frac{\int \ive{ \support_q(x, rv=v)} p(x,rv=v)dx}{p(rv=v)}
\end{align}
This means that we do not divide anymore by zero but by the number obtained when evaluating the probability distribution at the observed point. For example, when evaluating \probloginline{beta(2,3)} (cf. Example~\ref{example:dcproblog:observation}, Line~\ref{example:dcproblog:observation:beta23}) at $4/10$  we get $1.7280$ instead of zero.
% Note that this is not a probability between zero and one.

In order to guarantee that the limit in Equation~\ref{equ:borel_limit} exists, we need to restrict the type signature of the \probloginline{observation} predicate. The  first argument is a {\em named} random variable and the second argument a number, cf. Example~\ref{example:dcproblog:observation}.
Relaxing this restriction might lead to the non-existence of the limit. Exactly this situation gives rise to the Borel-Kolmogorov paradox emerges. 

Nevertheless, some languages lift this restriction, which results in possibly semantically ill-defined programs, such as in Distributional Clauses~\citep[Section 3.2]{nitti2016probabilistic}. A more sophisticated method to tackle the non-uniqueness of the conditional probability is {\em disintegration}~\citep{shan2017exact}, where, instead of returning a conditional probability, a family of conditional probabilities is returned (representing an uncountable number of limits). Other languages, such as BLOG, simply assume the existence of the limit~\citep{wu2018discrete}.

The type signature we impose on the \probloginline{observation/2} predicate might seem too restrictive for the purpose of probabilistic programming. Take for example the following conditional probability~\citep{nitti2016probabilistic}:
\begin{align}
	P(nationality| height {=} 160 \lor height {=} 180) \label{eqn:disj_conditioning}
\end{align}
This probability cannot be expressed using the \probloginline{observation/2} predicate. However, if we think about what a conditioning set represents in the context of probabilistic programming and machine learning, the example above appears quite odd. The conditioning set tells us which observations we have made about the world, \ie data that we collected using a physical device (\eg tape measure for the height of a person). The example in Equation~\ref{eqn:disj_conditioning} now tells us that our measuring device returned two numbers for a single measurement, which means that the measuring protocol is underspecified.

We just stated that a measurement consists of retrieving a number from a measuring device. This is not entirely correct. In the natural sciences a measurement consists always of a number and an upper and lower error bound, which effectively eliminates the problem of zero probability events. However, given the ubiquity of single point measurement, we feel that a probabilistic programming language that is not able to handle single point measurements is greatly hurt in its expressivity.

To conclude, in \dcproblogsty,  the \probloginline{observation/2} predicate allows a user to condition on zero probability events, while at the same time the imposed restrictions ensure that the encoded probability distribution is well defined.


\ak{conditional probabilities: just wondering: is it possible to condition on tests, \eg, observing that someone's height is at most 180? related to that, in (17), what if someone with bad handwriting measured the height and recorded it on a piece of paper, and I can't tell whether it is 160 or 180? :) }
\pedro{in this case the measuremnt is the pixels and you would have yes/no for each pixel}




%%%%%%%%%%%%%%%%%%%%


\subsection{Compiling SMT formulas}

State-of-the art methods that perform probabilistic inference with discrete random variables, divide inference into a computationally expensive step, which is followed by a computationally cheap one. The first step, which is also called knowledge compilation~\citep{darwiche2002knowledge}, takes a propositional logic formula and compiles it into a decision diagram (DD). The most prominent representatives of DDs are arguably {\em binary decisions diagrams}~\citep{bryant1986graph}. The advantage of compiling Boolean structures to decision diagrams is that probabilistic inference (the second step), \ie computing the weighted model count, becomes computationally tractable~\citep{chavira2008probabilistic}.

This idea of compiling logic formulas, in order to perform probabilistic inference, has also been mapped to (quantifier free) SMT formulas~\citep{kolb2018efficient,zuidbergdosmartires2019exact} and
has led to state-of-the art algorithms to perform inference in hybrid domains~\citep{derkinderen2020ordering}.

There are, however, two important differences between probabilistic inference via knowledge compilation using propositional logic formulas and SMT formulas. First, the possible target languages for the compilation step differ. We can use BDDs, d-DNNFs~\citep{darwiche2004ddnnf}, or SDD~\citep{darwiche2011sdd} for propositional logic but we need to resort to {\em  extended decision diagrams} (XDD) for SMT formulas~\citep{sanner2011symbolic,zuidbergdosmartires2019exact,kolb2019exploit}.

A second and more fundamental difference is the computational hardness of performing probabilistic inference in DDs vs. XDDs: computing the weighted model count on a DD can be done in polytime but computing the weighted model integral on an XDD is in general \#P-hard.


\subsection{Algebraic Likelihood Weighting}

Performing probabilistic inference with Boolean random variables boils down to performing computations in the so-called probability semiring. \citet{kimmig2017algebraic} formulated a generalization of probabilistic inference on Boolean formulas by using arbitrary semirings, which they dubbed algebraic model counting. 
\citet{zuidbergdosmartires2019exact} picked up this idea and also formulated probabilistic inference in the discrete-continuous domain (using SMT formulas) as a semiring computation by reformulating weighted model integration as an algebraic model counting problem. The advantage of this approach is that by simplifying an algberaic structure that adheres to the properties already proves the correctness of the inference algorithm. 






% Probabilistic programming languages that successfully handle mixtures of discrete and continuous random variables, including conditioning with zero probability events deploy either purely symbolic inference algorithms~\citep{gehr2016psi,shan2017exact} or extend the likelihood weighting~\citep{fung1989weighing} algorithm leading to a hybrid symbolic-approximate inference algorithm~\citep{nitti2016probabilistic,wu2018discrete}.

In this section we frame the {\em lexicographic likelihood weighting} (LLW) algorithm~\citep{wu2018discrete} in an algebraic model counting context, which we dub algebraic likelihood weighting (\ialw). LLW is based on ideas presented in~\citep{nitti2016probabilistic} and combines sampling based probabilistic inference with symbolic inference to correctly handle mixtures of discrete and continuous random variables. The advantage of framing LLW  as an algebraic model counting problem is that the resulting algorithm becomes agnostic of the underlying inference mechanism (\eg Monte Carlo sampling, or symbolic integration). Moreover, we can simply reuse algorithms already developed in the WMI literature in order to perform inference in \dcproblogsty.

Following \citet{kimmig2017algebraic}, we first define a labelling function, which maps atomic SMT formulas to elements of a semiring, and continue by defining the semiring operations.

\begin{definition}[\ialw labeling function]
	\label{def:label_alpha_alw}
	Let be an atomic SMT formula. Then the label of the atomic formula $l$ is given by:
	\begin{align*}
		\alpha_{\ialw}(l) \coloneqq 
		\begin{cases}
% 			(p(l), 0)& \text{if $l$ is a Boolean variable} \\
			(p(x{=}v),1) & \text{if $l$ encodes \probloginline{observation(x,v)}, \ie $l\leftrightarrow (x{=}v)$} \\
			(\ive{l},0) & \text{otherwise} 
		\end{cases}
	\end{align*}
    In the first case $p(x{=}v)$ denotes the value of the probability distribution of the random variable $x$ evaluated at $v$.
	The label of a negated atomic SMT formula $ \neg l$ is given by:
	\begin{align*}
		\alpha_{\ialw}(\neg l) \coloneqq 
		\begin{cases}
% 			(1-p(l),0)& \text{if $l$ is a Boolean variable} \\
			(1,0) & \text{if $l$ encodes \probloginline{observation(x,v)}}\\
			(\ive{\neg l},0) & \text{otherwise} 
		\end{cases}
	\end{align*}
\end{definition}

\begin{example}[ALW labeling function]

\end{example}


\begin{definition}[\ialw semiring]
	The elements of the semiring $\mathcal{S}_{\ialw}$ are given by the set
	\begin{equation}\label{eqn:set_aws}
		\mathcal{A}_{\ialw}\coloneqq \left \{ (a, d) \right \}
	\end{equation}
	where $a$ denotes a real-valued weight (produce by the labeling function) and $d$ the number of probability densities (continuous probability distribution) that have contributed to $a$. The neutral elements $e^\oplus$ and $e^\otimes$ are defined as:
	\begin{align}
		e_{\ialw}^\oplus  \coloneqq (0,0)  &&
		e_{\ialw}^\otimes  \coloneqq (1,0)
	\end{align}
	For the addition and multiplication we define:
	\begin{align}
		(a_1,d_1) \oplus
		(a_2,d_2)
		&\coloneqq
		\begin{cases}
			(a_1+a_2,d_1) &\quad  \text{if $d_1=d_2$} \\
			(a_1,d_1) &\quad  \text{if $d_1<d_2$} \\
			(a_2,d_2) &\quad  \text{if $d_1>d_2$}
		\end{cases} \\
		(a_1,d_1) \otimes
		(a_2,d_2)
		&\coloneqq (a_1 \times a_2 , d_1+d_2)  &
	\end{align}
\end{definition}

\citet{zuidbergdosmartires2019exact} have shown that the weighted model integral is correctly computed on compiled logic structures that respect determinism (e.g XSDD, XADD), if the properties of a commutative semiring are respected and if the labeling function and the addition of the semiring form a neutral pair.

\begin{lemma} The structure $\mathcal{S}_{\ialw}=({\cal A}_{\ialw}, \oplus, \otimes, e^\oplus,e^\otimes)$ is a commutative semiring.
\end{lemma}	

\begin{lemma} The pair  $(\oplus, \alpha_{\ialw})$ is neutral ($\alpha_{\ialw}(l)\oplus \alpha_{\ialw}(\neg l) = e_{\ialw}^{\otimes}$).
\end{lemma}

Performing a computation on a compiled SMT formula using the \ialw semiring gives a tuple of tuple of two elements, which we denote by 
$$\ialw(\support,\weight)=\Big( \ialw_1(\support, w), \ialw_2(\support, w) \Big)$$
We can now express probabilities of a conditional queries in terms of algebraic likelihood weights. 
\begin{align}
    p(\support_q|\support_e) &=
    \begin{dcases}
        \frac{\E[\ialw_1(\support_q \land \support_e, {\weight_{q,e}})]}{\E[\ialw_1(\support_e, \weight_e)]} & \text{if $\ialw_2(\support_q {\land} \support_e, \weight_{q,e})\geq \ialw_2(\support_e, \weight_e)$}\\
        0 & \text{else}
    \end{dcases} \\
     &=\begin{dcases}
        \frac{\wmi(\support_q \land \support_e, {\weight_{q,e}})]}{\wmi(\support_e, \weight_e)]} & \text{if $\ialw_2(\support_q {\land} \support_e, \weight_{q,e})\geq \ialw_2(\support_e, \weight_e)$}\\
        0 & \text{else}
    \end{dcases} 
\end{align}
$\E(\ialw_1(\cdot, \cdot))$ denotes the expected value of the first element of tuple obtained by the algebraic likelihood computation and is equal to the weighted model integral over the same SMT formula.

\begin{example}[ALW on a circuit]

\end{example}


\subsection{What about \problogsty's External Engine?}


Syntactically, the \dcplpsty assembler language does not make a difference between Boolean random variables (\probloginline{flip}\lstinline[columns=fixed]{/2}) and other random variables (\eg \probloginline{normal}\lstinline[columns=fixed]{/2}).
Furthermore, \dcplpsty is constituted of a logic program (deterministic system) and random variables (independent choices).
This indicates that implementations of probabilistic logic programming languages with and without continuous random variables should not be too different from each other.
After all, a probabilistic logic programming language with continuous random variables simply adds additional probability distributions besides the \probloginline{flip} distribution.  


% Assume now that the algebraic model count of $\support_q \land \support_e$ and $\support_e$ evaluate respectively to:
% \begin{align}
% 	\AMC(\support_{q}\land \support_e , \alpha_{\ialw})&= (\amc_{qe}, d_{qe}) \label{eqn:amc_alw_qe} \\
% 	\AMC(\support_e , \alpha_{\ialw})&= (\amc_{e}, d_{e}) \label{eqn:amc_alw_e}
% \end{align}

% The conditional probability is then given by:
% \begin{align}
% 	p(\support_{q} | \support_e) =
% 	\begin{cases}
% 		\frac{\wmi(\support_q \land \support_e, \weight_{qe})}{\wmi(\support_e, \weight_{e})} & \text{if $d_{qe}=d_e$} \\
% 		0  & \text{if $d_{qe}>d_e$} 
% 	\end{cases} \label{eqn:conditional_wmi}
% \end{align}

% Note, in Equations~\ref{eqn:amc_alw_qe} to~\ref{eqn:conditional_wmi} we have omitted the dependence of the algebraic model counts and the weighted model integration on the Boolean and/or real variables.



% \todo{talk about difference BLOG and DC to ALW, make difference on algorithmic level}
% DC~\citep{nitti2016probabilistic} and BLOG~\citep{wu2018discrete} do return the correct probabilities as well, however, the advantage of using Sampo in conjunction with ALW gives515the correct result without drawing any samples.

==> files_old/introduction.tex <==

\section{Introduction}
\ak{intro should get to the point more quickly; what is the exciting thing about this work? see Table \ref{tab:features} for a (partial) answer covering the language/semantics side, which would need to be extended to inference and implementation}

\begin{table}[ht]
    \centering
    \begin{tabular}{|p{0.3\textwidth}||c|c|c||c|c|}
    \hline
       Feature  & ProbLog & DC & DC & \dcproblogsty & \dcproblogsty  \\
       & & (Gutmann) & (Nitti) & (core) & (full)\\
       \hline\hline
       fully declarative semantics & y & y & n & y & y \\\hline
       negation & y & n & y & y & y \\\hline
       RVs with finite, countable and continuous domains & n & y & y & y & y\\\hline
       RVs with distributions parameterised by other RVs & n & y & y & y & y \\\hline
       RVs with distributions determined by logical context / (full) DCs & n & y & y & n & y \\\hline
       probabilistic facts / tuple-independent PDB  & y & n & n & n & y \\\hline
       annotated disjunctions / independent causation  & y & n & n & n & y \\\hline
    \end{tabular}
    \caption{Probabilistic logic programming languages and their features \todo{expand beyond our own languages / refine features further} \ak{adapting a comment from Luc in a different semantics discussion, the goal here is to show that we introduce the first PLP language that brings the range of modeling features / syntax elements together with the fully declarative semantics in a single language; then, the examples in sec 2 should illustrate how cool this is}}
    \label{tab:features}
\end{table}

\ak{I think these only motivate part of the whole, and should be adapted to illustrate the full power of the features in table \ref{tab:features} -- show what we can do and discuss that others can't rather than showing how others need to hack approximations }




Uncertainty is ubiquitous in real-world phenomena and successfully modelling such phenomena necessitates taking into account this uncertainty.
Expressing the knowledge we have about the world in a formal fashion constitutes a necessary first step in mechanizing the reasoning process for these probabilistic phenomena.
An emerging paradigm of doing so is probabilistic programming~\citep{meent2018introduction}.
Probabilistic programming languages (PPL) unify the expressive power of general purpose (Turing complete) programming languages and probabilistic modelling.

PPLs come in various different flavors, adhering for example to the declarative programming paradigm or the imperative programming paradigm.
All PPLs have in common that a user writes down a probabilistic program and the probabilistic inference engine, which is shipped along side the language, takes subsequently care of performing probabilistic inference.\footnote{One could argue that imperative probabilistic programming languages are to a degree declarative: the user only specifies/declares the probability distributions, and does not write any probabilistic inference algorithm.}

The particular PPL flavor that we investigate in this paper is probabilistic logic programming (PLP)~\citep{de2015probabilistic,riguzzi2018foundations}.
PLP can be seen as the continuation of a long line of research of unifying logic and probability theory~\citep{russell2015unifying}. With the introduction of {\em probabilistic Horn abduction} (PHA) by ~\citet{poole1993probabilistic}, a first important step had been made towards combining (non-probabilistic) logic programming and probability theory. PHA allowed~\citeauthor{poole1993probabilistic} to  construct the {\em Independent Choice Logic} (ICL) language~\citep{poole1997independent}, an expressive universal probabilistic logic programming language.
In a seminal paper, \citet{sato1995statistical} built on top of the ideas advanced by~\citet{poole1993probabilistic} and introduced the so-called {\em distribution semantics} (DS) for probabilistic logic programs.  
Since the inception of DS, a variety of  additional PLP languages have appeared, such as {\em PRISM}~\citep{sato1997prism}, {\em Logic Programs with Annotated Disjunctions}~\citep{vennekens2004logic}, and {\em \problogsty}~\citep{de2007problog,fierens2015inference}, to name a few.
\ak{careful with history claims (eg Dantsin)}

Probabilistic logic programming has first and foremost been concerned with random variables that have finite sample spaces -- mainly due to the fact that it is rather straightforward to turn deterministic logic atoms into probabilistic logic atoms.
As a consequence, PLP languages that allow for continuous random variables, such as \extendedprismsty~\citep{islam2012inference} and \dcsty\todo{cite on first mention}, have been proposed.
In the context of probabilistic logic programming such languages have been dubbed {\em hybrid}, as they allow for discrete and continuous random variables alike.
Unfortunately, the semantics that have been proposed so far for hybrid PLP languages have been imprecise, as pointed out by~\citet{azzolini2021semantics}, or exhibit some caveats. For example, the declarative semantics proposed in~\citep{islam2012inference} or~\citep{gutmann2011magic} do not allow for negation, and while the semantics proposed in~\citep{nitti2016probabilistic}  do allow negation, they are not declarative anymore but procedural. Our first contribution tackles these issues:
\begin{enumerate}
    \item We introduce the hybrid probabilistic logic programming language \dcproblogsty, for which we define {\bf declarative semantics} that cover negation and are based on \citeauthor{sato1995statistical}'s distribution semantics.
\end{enumerate}
The declarative semantics that we define for the hybrid PLP langugage \dcproblogsty extends the semantics given in~\citep{gutmann2011magic} such that negation is allowed. Furthermore, we simplify the definition of the semantics and eliminate some inconsistencies present in~\citep{gutmann2011magic}.

Eventually, a probabilistic programming language should be able to compute (conditional) probabilities of queries given by the user. This means that PLPs need to be equipped with inference mechanism. We show how inference for the hybrid PLP language \dcproblogsty can be mapped onto weighted model integration (WMI)~\citep{belle2015probabilistic}. 

\begin{enumerate}
\setcounter{enumi}{1}
	\item We {\bf reduce inference} in \dcproblogsty to {\bf weighted model integration}, analogous to reducing inference in \problogsty to weighted model counting~\citep{chavira2008probabilistic} when dealing with discrete random variables only.
	\item We present {\em algebraic likelihood weighting}, an inference algorithm for hybrid probabilistic logic programs that combines {\bf knowledge compilation}~\citep{darwiche2002knowledge}, {\bf algebraic model counting}~\citep{kimmig2017algebraic}, and {\bf likelihood weighting}~\citep{fung1989weighing}.
\end{enumerate}
Until now only probabilistic programming languages targeting discrete random variables exclusively have leveraged knowledge compilation. This has allowed them to exploit structure present in the program when performing inference.
Algebraic likelihood weighting is the first inference algorithm in the hybrid domain exhibiting this feature and is consequently the first inference algorithm to exploit discrete structures in hybrid probabilistic programs. 



Furthermore, we provide an implementation of \dcproblogsty that we dub \dcproblogsys and which is an extension of the ProbLog2 system~\citep{dries2015problog2}.
\begin{enumerate}
\setcounter{enumi}{3}
% 	\item We introduce a {\bf type system} for \dcproblogsty. The type system allows us to overload the existing \problogsty syntax and use it for hybrid probabilistic logic programming.
% 	While type systems are omnipresent in non-logic probabilistic programming languages, they have not received any attention in the PLP community.
    % To the best of our knowledge, we present the first type system for a probabilistic logic programming language.
	\item We present an {\bf implementation of \dcproblogsty} that uses algebraic likelihood weighting and reduces naturally  to \problogsty in the absence of continuous random variables.
% 	\item We give two implementations of AWL. An exact implementation that performs exact  probabilistic inference using PSI~\citep{gehr2016psi} in its back end and an approximate implementation using Pyro~\citep{bingham2019pyro}.
\end{enumerate}




% \begin{itemize}
%     \item fully unify discrete and continuous semantics
%     \item disentangle random variables from program
%     \item perform inference by mapping to WMI -> generalizes WMC
%     \item what is different to other approaches, non-logical? separation of combinatorial \#P-hardness and integration \#-hardness
% \end{itemize}












\subsection*{Paper Organization}
In Section~\ref{sec:motivation}, we motivate our work by giving introductory examples. We continue in Section~\ref{sec:semantics} by presenting \dcplpsty, a bare bones probabilistic logic programming language with minimal syntax.
\dcplpsty with its minimal syntax has the advantage of facilitating the definition of a declarative semantics. In Section~\ref{sec:dcproblog} we formally introduce \dcproblogsty.
The semantics of \dcproblogsty programs are obtained via deterministically transforming \dcproblogsty programs to \dcplpsty programs, for which we will have defined the semantics in Section~\ref{sec:semantics}.
In Section~\ref{sec:implementation} we describe \dcproblogsys, an implementation of \dcproblogsty built on top of the \problogsys system~\citep{fierens2015inference,dries2015problog2}.
Subsequently, we map inference in \dcproblogsty to weighted model integration ~\citep{belle2015probabilistic} and describe the implementation of the inference algorithm in \dcproblogsys. 
In Section~\ref{sec:related} we discuss \dcproblogsty in a broader probabilistic programming context and relate the language to other probabilistic programming languages such as BLOG~\citep{milch2005blog}.
We end with concluding remarks in Section~\ref{sec:conclusions}.




\subsection*{Prerequisites}

We expect the reader to be familiar with rudimentary language concepts and terms of (non-probabilistic) logic programming and more specifically of Prolog~\citep{lloyd2012foundations,flach1994simply}. We provide a brief summary of these concepts in~\ref{app:lp}. Furthermore, a working knowledge of probabilistic inference with discrete random variables using weighted model counting and integration would be beneficial. A refresher on probabilistic inference using WMC and WMI can be found in~\ref{app:amc}, ~\ref{app:compilation}, and \ref{app:wmi}.

\ak{decide on LP/Prolog citation(s), here vs start of next sec (and elsewhere?)}


\subsection{stuff from elsewhere}
\ak{these are bits and pieces that disturbed the flow of the semantics section but may still be relevant somewhere...}

\ak{the following message seems better placed in the intro/motivation: }
\citet{poole2010probabilistic} has characterised probabilistic programs as deterministic systems with  independent choices. \dcproblogsty relaxes \citeauthor{poole2010probabilistic}'s independent choices by allowing for connections between the independent choices by means of random variables appearing as parameters of distributions, thus introducing a kind of hierarchical system of independent choices, as illustrated in  Example~\ref{ex:random_choice_dependency}.
\dcproblogsty is the first probabilistic programming language to make the distinction between:
\begin{enumerate}
    \item structure expressed by the the deterministic system
    \item structure expressed by hierarchically parameterized distributions of random variables
\end{enumerate}
\ak{any better term to refer to the structure between RVs than "hierarchical"? }

\ak{We need to decide what to do with this; can we claim it's syntactic sugar and deal with it in that section? }
Note that while we implicitly assume   univariate (or {\em `atomic'}) random variables here, the principles do also apply to multivariate (or {\em `compound'}) random variables, such as multivariate Gaussians, provided that the usual laws of probability are respected and suitable syntax for such variables is introduced.


%Distributional facts are not limited to describe continuous random variables but can, for example, also model discrete probability distributions such as the Poisson distribution.
%\begin{example}\label{example:dcproblog_poisson_population}
%The following DC-ProbLog program models the size of a group of people as a Poisson distribution and
%defines predicates related to that size using the comparison predicates  \probloginline{>}\lstinline[columns=fixed]{/2} and \probloginline{=:=}\lstinline[{columns=fixed}]{/2}, where the latter is standard Prolog syntax for equality comparisons on numbers.
%\luc{=:= non-standard}\ak{it is standard Prolog}
%	\begin{problog*}{linenos}
%n_people ~ poisson(6).

%more_than_five:- n_people>5@.@
%exactly_five:- n_people=:=5@.@
%	\end{problog*}
%\end{example}

%We will provide further examples throughout the text, including showcase examples in Section~\ref{sec:showcase}. \ak{any good reason why we delay the showcases til then?}

% \section{Introduction}

% The mathematical discipline of logic constitutes the bedrock of a large body of work in artificial intelligence (AI) research, including sub-disciplines such as expert systems~\citep{jackson1998introduction}, inductive logic programming~\citep{muggleton1994inductive}, or more broadly knowledge representation and reasoning~\citep{levesque1986knowledge}. One of the main shortcomings of logic based AI systems is that they fail to capture the inherent uncertainty present in the world -- aleatoric and epistemic uncertainty alike~\citep{hullermeier2019aleatoric}. To express such uncertainties, AI researchers have set out to enhance pure logic with probabilities.

% As a matter of fact, the marriage of logic and probability is an enduring endeavor of AI research that predates AI itself~\citep{russell2015unifying}. Grandees of mathematics, philosophy, and economics such as Leibniz, Peirce, and Keynes, undertook early efforts to this end \citep{hailperin1984probability,howson2003probability}. In the field of AI, \citet{nilsson1986probabilistic} and~\citet{pearl1988probabilistic} presented seminal works investigating the combination of logic and probability, which heralded the era of {\em modern AI}: systems were now able to capture the inherent uncertainty present in the world as well as reason about it.

% \luc{Dantsin 89, PDBs, general PP ?}

% \citet{poole1993probabilistic} improved upon these ideas and introduced {\em probabilistic Horn abduction}, which allowed him to later on construct the {\em Independent Choice Logic} (ICL) language~\citep{poole1997independent}. ICL is an expressive universal probabilistic logic programming language (PLP) \citep{de2015probabilistic,riguzzi2018foundations} rooted in logic programming.
% Subsequently, \citet{sato1995statistical} built on top of the ideas advanced by~\citet{poole1993probabilistic} and introduced the so-called {\em distribution semantics} (DS) for probabilistic logic programs.  
% After the introduction of DS, a variety of  further PLP languages appeared, such as {\em PRISM}~\citep{sato1997prism}, {\em Logic Programs with Annotated Disjunctions}~\citep{vennekens2004logic}, and {\em \problogsty}~\citep{de2007problog,fierens2015inference}, to name a few.


% In this paper we focus on \problogsty, a probabilistic programming language inheriting its syntax from the (non-probabilistic) logic programming language \prologsty~\citep{sterling1994art}. \problogsty  allows one to express, in addition to logic rules and facts, so-called \textit{probabilistic facts}, which are logic facts labeled with the probability of them being satisfied.
% \begin{example}\label{example:problog_machine}
% 	We model two machines (Line \ref{program:problog_machines_dec} in the program below).
% 	We want to know the probability of the first machine working (Line \ref{program:problog_machines_query}), given that the second machine works (Line \ref{program:problog_machines_evidence}) and given a model that describes under which conditions the machines work (Lines \ref{program:problog_machines_work_cool} and \ref{program:problog_machines_work_temp}).
% 	Additionally the program models the outside temperature (Line \ref{program:problog_machines_temp})  and whether the cooling of each machine works (Lines \ref{program:problog_machines_cool1} and \ref{program:problog_machines_cool2}) as (Boolean) random variables (expressed as probabilistic facts).
% 	\begin{problog*}{linenos}
% machine(1). machine(2). @\label{program:problog_machines_dec}@

% 0.8::temperature(low). @\label{program:problog_machines_temp}@
% 0.99::cooling(1). @\label{program:problog_machines_cool1}@
% 0.95::cooling(2). @\label{program:problog_machines_cool2}@

% works(N):- machine(N), cooling(N). @\label{program:problog_machines_work_cool}@
% works(N):- machine(N), temperature(low). @\label{program:problog_machines_work_temp}@

% evidence(works(2)).  @\label{program:problog_machines_evidence}@
% query(works(1)). @\label{program:problog_machines_query}@
% 	\end{problog*}
% Running the program yields $P(\text{\probloginline{works(1)}}|\text{\probloginline{works(2)}})\approx 0.998$.
% \end{example}

% A major limitation of \problogsty becomes immediately apparent in Example~\ref{example:problog_machine}: we need to model the {\em temperature} as a discrete (Boolean) random variable rather than a continuous probability density.


% To repair this deficiency we present \dcproblogsty, a probabilistic logic programming language derived from \problogsty and Distributional Clauses (DC) -- two related but separate probabilistic logic programming languages.
% \dcproblogsty inherits its syntax and the concept of probabilistic facts from \problogsty. Moreover, \dcproblogsty adapts the idea of defining and querying continuous random variables using so-called {\em distributional facts}.
% Distributional facts allow a user to express random variables that are distributed according to a certain probability distribution specified by a random function symbol.

% In the following example, the distributional fact in Line~\ref{program:dcproblog_machines_work_temp} introduces the random variable \probloginline{temperature} and associates it with the distribution term \probloginline{normal(20,5)}. This is done using the \probloginline{~}\lstinline[columns=fixed]|/2| predicate in infix notation.
% In Line~\ref{program:dcproblog_machines_work_temp} the random variable is then queried using the comparison predicate \probloginline{<}\lstinline[columns=fixed]|/2|, again written in infix notation. 


% \begin{example}\label{example:dcproblog_machine}
% 	We model the temperature as a continuous random variable distributed according to a normal distribution with mean $20$ and standard deviation $5$ (Line \ref{program:dcproblog_machines_temp}).
% 	\begin{problog*}{linenos}
% machine(1). machine(2).

% temperature ~ normal(20,5). @\label{program:dcproblog_machines_temp}@
% 0.99::cooling(1).
% 0.95::cooling(2).

% works(N):- machine(N), cooling(N).
% works(N):- machine(N), temperature<25.0. @\label{program:dcproblog_machines_work_temp}@

% evidence(works(2)).  @\label{program:dcproblog_machines_evidence}@
% query(works(1)).
% 	\end{problog*}
% \end{example}
% \luc{query(works(1)|works(2))}

% Distributional facts are not limited to describe continuous random variables but can, for example, also model discrete probability distributions, of which an example would be the Poisson distribution.
% \begin{example}\label{example:dcproblog_poisson_population}
% 	In this example we show how to model the size of a group of people as a Poisson distribution and answer queries about the size of the group using the comparison predicates  \probloginline{>}\lstinline[columns=fixed]{/2} and \probloginline{=:=}\lstinline[{columns=fixed}]{/2}.\luc{=:= non-standard}\ak{it is standard Prolog}
% 	\begin{problog*}{linenos}
% n_people ~ poisson(6).

% more_than_five:- n_people>5@.@
% exactly_five:- n_people=:=5@.@

% query(more_than_five).
% query(exactly_five).
% 	\end{problog*}
	
% \end{example}


% \citet{poole2010probabilistic} has characterized probabilistic programming as {\em independent choices plus deterministic systems}.
% In the case of probabilistic logic programming with discrete random variables the deterministic system is given by a logic program.
% \dcproblogsty builds on this idea but relaxes the independence assumption by explicitly distinguishing two types of dependencies 1) those expressed by the logic program (the deterministic system) and 2) those expressed by using random variables as parameters of distributions for other random variables (the independent random choices \ak{sounds like  independent random choices are a form of dependencies, which they aren't; in general, this is a line of thought that we repeat in too many places -- we have to pick one and explain it well there}). This explicit distinction is not made by any other probabilistic (logic) programming language including discrete and continuous random variables. Such a programming language is also called {\em hybrid}. \luc{what about BLOG?}

% When writing (hybrid) probabilistic programs, users have a range of options, from encoding entire probability distributions defined by the probabilistic program into a single choice random variable (no deterministic system), all the way to 
% a set of individual independent choice random variables with minimal use of random variables as parameters tied together by a deterministic system.
% As already discussed by~\citet{poole2010probabilistic}, not all options work equally well with all inference algorithms. \dcproblogsty provides these options within the same semantic framework, leaving it to system developers to focus the syntax towards a subset of options and/or to exploit the different options when integrating different inference approaches into their system.

% Developing the \dcproblogsty language, leads to the following specific contributions:
% \todo{update needed}

% \begin{enumerate}
% 	\item We introduce a {\bf type system} for \dcproblogsty, which allows us to introduce a {\bf neat and clean syntax} to extend \problogsty with function symbols for continuous random variables.
% 	\item We introduce a purely {\bf declarative semantics for \dcproblogsty} based on \citeauthor{sato1995statistical}'s distribution semantics that allows us to disentangle independent choices and the discrete system underlying a probabilistic program.
% 	\item We {\bf reduce inference} in \dcproblogsty to {\bf weighted model integration} in the algebraic model counting setting~\citep{kimmig2011algebraic,kimmig2017algebraic}, analogous to reducing inference in \problogsty to weighted model counting~\citep{chavira2008probabilistic}.
% 	\item We present an {\bf implementation of \dcproblogsty}, which reduces naturally to \problogsty in the absence of continuous random variables.
% \end{enumerate}
% \dcproblogsty is heavily influenced by two predecessor languages: 1) \problogsty and 2) Distributional Clauses~\citep{gutmann2011magic,nitti2016probabilistic}. The latter is a probabilistic logic programming languages that allows for continuous random variables. However, its semantics differ from the semantics of \problogsty such that it does not reduce to \problogsty in case of the absence of continuous random variables.


% \subsection*{Prerequisites}

% To fully appreciate the paper, we expect the reader to be familiar with rudimentary language concepts and terms of (non-probabilistic) logic programming and more specifically of Prolog~\citep{lloyd2012foundations,flach1994simply}. We provide a brief summary of these concepts in~\ref{app:lp}.

% Furthermore, a working knowledge of probabilistic inference with discrete random variables using weighted model counting would be beneficial (WMC)~\citep{chavira2008probabilistic,darwiche2009modeling}, as we present an inference algorithm for \dcproblogsty that extends WMC. A refresher on probabilistic inference in the discrete domain can be found in~\ref{app:amc} and ~\ref{app:compilation}.


% \subsection*{Paper Organization}
% \todo{}




==> files_old/preliminaries.tex <==
\section{Preliminaries}

We expect the reader to be familiar with basic language concepts and terms of Prolog \todo{cite (Lloyd, 1989; Flach, 1994)}; a quick summary can be found in~\ref{app:lp}. \ak{this sentence and appendix copied from plp concepts paper; should go earlier given we already have examples there?}



\subsection{Probabilistic Logic Programming}
\ak{how much do we need here, given that we later introduce ProbLog constructs through their mappings to the new language? how much detail on the distribution semantics is needed for completeness? (the semantics sec is heavily linked to the Sato paper, but we can't repeat all of that)}


\subsection{Weighted Model Integration}

\todo{introduce all the wmc, amc, wmi gadgets}

==> files_old/syntax_types.tex <==
\section{\dcproblogsty Syntax and Type System} \label{sec:syntax}
\ak{I propose to move the type system and multiple dispatch stuff to a separate implementation section as much as possible;\ie, from here onwards: 1) introduce DC-ProbLog programs as normal logic program + probabilistic facts + distributional facts + comparison predicates instead of wrapped query terms, 2) show that these map to DC-PLP, 3) add further syntactic sugar (is/2, distributional clauses, anything else? are annotated disjunctions part of DC-ProbLog?) and show how that maps back onto the basic version, 4) talk about multiple dispatch and all that }


\todo{this is just moved from earlier sec 3, needs linking to DC-PLP and merging with semantics in next section; the goal is to introduce DC-ProbLog as a higher level modeling language that makes concrete choices for the reserved functors in DC and introduces nicer syntax / syntactic sugar, but for its semantics maps back to (an instance of) DC-PLP}

\subsection{Type System}
Before we formally specify the syntax of \dcproblogsty, we specify a hierarchical type system. To this end we will modify the type system given in~\citep{sterling1994art}, one of the main references on \prologsty. The base type in the type system of~\citep{sterling1994art} is the \type{Term} type, from which other types are subtyped. In other words: everything is a \type{Term}.
\begin{enumerate}
	\item[]   \type{Term}
	\begin{itemize}		
		\item \type{Atomic}
		\begin{itemize}
			\item \type{Atom}
			\item \type{Number}
		\end{itemize}
		\item \type{Compound}
	\end{itemize}
\end{enumerate}

{\em Logical variables} (technically referred to as {\em meta-logical variables}~\citep[Chapter 10]{sterling1994art}) are omitted from the type system hierarchy, as they can ground to any type, depending on the context. In Figure~\ref{fig:type_system_prolog} we give a diagrammatic representation of the \prologsty type system.
Note that \problogsty uses a different nomenclature: atom terms in \problogsty correspond to the union of atom terms and compound terms in the \prologsty nomenclature of~\citep{sterling1994art}. In a first step we are going to change the \prologsty type system to match the nomenclature of \problogsty.
\begin{enumerate}
	\item[]   \type{Term}
	\begin{itemize}		
		\item \type{Number}
	\end{itemize}
	\begin{itemize}
		\item \type{Atom}
	\end{itemize}
\end{enumerate}

In Table~\ref{table:comp_type_system} we give a side by side comparison of the two type systems and in Figure~\ref{fig:type_system_prolog} and~\ref{fig:type_system_problog} we give diagrammatic representations of both type systems.

\begin{table}[h]
	\caption{Comparison of the \prologsty type system and the \problogsty type system.}
	\label{table:comp_type_system}
	\begin{center}
		\begin{tabular}{c||c|c|c}
			example \type{Term} & \multicolumn{2}{c|}{\prologsty} & \problogsty \\ 
			\hline
			\probloginline{3} & \type{Number} & \multirow{2}{*}{\type{Atomic}}  &  \type{Number}  \\
			\cline{1-1} \cline{4-4}
			\probloginline{foo} & \type{Atom} &   & \multirow{2}{*}{\type{Atom}}  \\
			\cline{1-3}
			\probloginline{bar(foo)} &  \multicolumn{2}{c|}{\type{Compound}}  &   \\
			%	\probloginline{foo} & \begin{tabular}{@{}c|c@{}}
			%		\type{Atom} &\multirow{0}{c}{\phantom{\type{Atomic}}} 
			%	\end{tabular}  &  \type{Atom} \\
		\end{tabular}
	\end{center}
\end{table}



\begin{figure}[h!]
	\centering
	\begin{minipage}{.45\textwidth}
		\centering
		\includegraphics[width=0.85\linewidth]{../figures/type_hierarchy_prolog.pdf}
	\end{minipage}%
	\hfill
	\begin{minipage}{.45\textwidth}
		\centering
		\includegraphics[width=0.85\linewidth]{../figures/type_hierarchy_problog.pdf}
	\end{minipage}
	\par
	\medskip
	\noindent
	\begin{minipage}[t]{.45\textwidth}
		\captionof{figure}[Diagrammatic representation of the hierarchical \prologsty type system.]{Diagrammatic representation of the hierarchical \prologsty type system~\citep{sterling1994art}. The \type{Number} type is further subtyped into \type{Integer} and \type{Float}.}
		\label{fig:type_system_prolog}
	\end{minipage}%
	\hfill
	\begin{minipage}[t]{.45\textwidth}
		\captionof{figure}[Diagrammatic representation of the hierarchical \problogsty type system.]{Diagrammatic representation of the hierarchical \problogsty type system. The \type{Number} type is further subtyped into \type{Integer} and \type{Float}.}
		\label{fig:type_system_problog}
	\end{minipage}
\end{figure}



Analogously to the just introduced type system of \problogsty, the base type for \dcproblogsty is again the \type{Term} type. At this point we modify the \problogsty type system by subtyping terms with a \type{Distrbution} type and a \type{Symbol} type. 
Dividing \dcproblogsty terms into \type{Distribution} terms and \type{Symbol} terms reflects the characterization of~\citet{poole2010probabilistic} of probabilistic programs as being constituted of independent choices (\type{Distribution}) and a deterministic system (\type{Symbol}).

\begin{definition}\label{def:type_system}
	The \dcproblogsty type system is a hierarchical type system with each type being a disjoint union of its subtypes.
	\begin{enumerate}
		\item[] \type{Term} 
		\begin{enumerate}
			\item[1.] \type{Distribution}
			\begin{itemize}
				\item \type{DiscreteD}
				\item \type{ContinuousD}
				\item \type{MixtureD}
			\end{itemize}
			\item[2.] \type{Symbol}
			\begin{itemize}		
				\item \type{Arithmetic}
				\begin{itemize}
					\item  \type{RandomVariable}
					%			\begin{itemize}
					%				\item \type{DiscreteRV}
					%				\item \type{ContinuousRV}
					%				\item \type{MixtureRV}
					%			\end{itemize}
					\item \type{Number}
				\end{itemize}
				\item \type{Atom}
			\end{itemize}
		\end{enumerate}
	\end{enumerate}
\end{definition}

A diagrammatic overview of the \dcproblogsty type system is given in Figure~\ref{fig:type_system}.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\linewidth]{../figures/type_hierarchy.pdf}
	\end{center}
	\caption[Diagrammatic representation of the hierarchical \dcproblogsty type system.]{Diagrammatic representation of the hierarchical \dcproblogsty type system. Compared to Definition~\ref{def:type_system},  the \type{Number} type is further subtyped into \type{Integer} and \type{Float} types and the \type{RandomVariable} type is subtyped into \type{DiscreteRV}, \type{ContinuousRV}, and \type{MixtureRV}. These subtypes of \type{RandomVariable} mimic the subtypes of the \type{Distribution} type.}
	\label{fig:type_system}
\end{figure}



%A type is a disjoint union of its subtytpes, for example:
%$$\type{Term}=\type{Distribution} \cup \type{Symbol}$$







\subsubsection{Distribution Terms}
As already seen in Examples~\ref{example:dcproblog_machine} and~\ref{example:dcproblog_poisson_population}, \type{Distribution} terms determine the probability distribution according to which a random variable is distributed.

\begin{definition}[\type{Distribution}]
	Terms of type \type{Distribution} are constructed by using a reserved random function symbol and applying it to a (possible empty) tuple of input arguments, which maps the input tuple to a distribution term.
	Distribution terms are only allowed to be invoked as a second argument to the reserved distribution predicate \probloginline{is}\lstinline[columns=fixed]|/2|.
	This also means that random function symbols are only used there as well. \dcproblogsty subtypes the \type{Distribution} type into the \type{DiscreteD}, \type{ContinuousD}, and \type{MixtureD} types.
\end{definition}

\probloginline{poisson(6)} and \probloginline{normal(20,5)} are for instance of types \type{DiscreteD} and  \type{ContinuousD}, respectively.
Note that distributions of type \type{ContinuousD} denote {\em absolutely continuous} probability distributions\footnote{\dcproblogsty does not support {\em singular continuous} probability distributions such as the Cantor distribution.}. \ak{would be nice to have a hint on why this restriction is there} We give an example of a distribution of type \type{MixtureD} in Example~\ref{ex:indian_gpa_function}.
%\begin{example} \probloginline{mixed} is a random variables that is a mixture of a continuous part (the truncated normal between $0$ and $4$ with mean $3$ and standard deviation $1$) and a discrete part. 
%\begin{problog}
%mixted~Mix((0.998,TruncNormal(3,1,0,4)),(0.001,4),(0.001,4))
%\end{problog}
%\end{example}

%For and example, see Example~\ref{example:dcproblog_poisson_population}: we have the random function symbol \probloginline{poisson}\lstinline[columns=fixed]{/1}, apply it to the input tuple \probloginline{(6)}, and obtain a term of type \type{Distribution}.


\subsubsection{Symbol Terms}
\type{Symbol} terms are the building blocks of the discrete structure that makes up a logic program and as such determine also the deterministic system of a probabilistic logic program. Beyond the reserved syntax, which is used to define the distribution terms, the user is free to use any identifier (following \prologsty conventions) to declare \type{Symbol} terms -- this includes standard \prologsty terms such as lists.
%The subtyping of the \type{Symbol} type (shown in Figure~\ref{fig:type_system}) follows the convention given in~\citep[Chapter 9]{sterling1994art}.

\begin{definition}[\type{Arithmetic}]
	Terms of type \type{Symbol} for which arithmetic operations are defined are of type \type{Arithmetic}. \type{Arithmetic} terms can be used as second argument to the builtin \probloginline{is}\lstinline[columns=fixed]|/2| functor. \type{Arithmetic} terms are subtyped with \type{RandomVariable} terms and \type{Number} terms.
%	\ak{Def 6.3 Arithmetic terms: if (as stated in def 6.1) each type is the disjoint union of its subtypes, that means that "arithmetic" is made up exclusively of numbers and RVs, \ie, terms like 3-2 or min(x,5) for a RV x are not allowed, whereas the first two sentences of def 6.3 suggests they might be allowed (only having numbers and RVs directly on the rhs of is/2 seems quite boring...). Which is it?
%		Related to this, defs 6.8 and 6.10 talk about RVs and Numbers, why not simply "arithmetic"?}
\end{definition}
We talk in more detail about \type{Arithmetic} terms and their evaluation in Subsection~\ref{sec:arithmetic}.

\begin{definition}[\type{RandomVariable}] \label{def:random_variable}
	\type{RandomVariable} terms are named by the programmer using distributional facts with the binary infix predicate \probloginline{is}\lstinline[columns=fixed]|/2| and inherit their subtype from the distribution term. All random variables present in a \dcproblogsty program are named. \type{RandomVariable} terms are a subtype of the \type{Arithmetic} type. \ak{Def 6.4: why do you restrict random variables to be arithmetic? What about color(Ball)~uniform([red,green,blue])? Of course, such finite discrete domains could be encoded using integers and then translated back in the LP, so theoretically speaking it's probably not a restriction to only have numbers, but from a modeling perspective, it is surprising to me.}
\end{definition}

Examples of terms of type \type{RandomVariable} would be \probloginline{temperature} and \probloginline{n_people} in Examples~\ref{example:dcproblog_machine} and~\ref{example:dcproblog_poisson_population}, where we declared the random variables through so-called {\em distributional facts}: 
\begin{problog}
temperature ~ normal(20,5).
n_people ~ poisson(6).
\end{problog}
As mentioned in Defintion~\ref{def:random_variable}, \type{RandomVariable} terms inherit their type from the associated \type{Distribution} term, \eg a \type{ContinuousD} term induces a random variable term of type \type{ContinuousRV}.

Note that not all probabilistic programming languages enforce the naming of random variables. In the functional probabilistic programming language \anglicansty~\citep{wood2014approach}, for instance, the user can declare anonymous random variables, much like anonymous functions, \ie \textlambda-functions.
\ak{Discussion of named/unnamed between Defs 6.4 and 6.5: would be nice to have a brief hint on why you made that choice}

\begin{definition}[\type{Number}] Terms of type \type{Number} are used to express numerical data types such as integers and floating point numbers.	
\end{definition}


\ak{terminology mix-up; predicates never form terms}
\begin{definition}[\type{Atom}]
	An atom is of the form \probloginline{p(t@$_1$@,@\dots @, t@$_n$@ )} where \probloginline{p} is a predicate of arity $n$ and the \probloginline{t@$_i$@} are \type{Symbol} terms~\citep{fierens2015inference}. Predicates used to construct \type{Atom} terms must not clash with the builtin predicates and reserved random function symbols used to declare \type{Distribution} terms. Terms of type \type{Atoms} constitute the building blocks of the discrete structure of a probabilistic logic program.
\end{definition}

Examples of atoms terms would be \probloginline{foo} or \probloginline{bar(foo,42)}. The latter is constructed using the predicate \lstinline{bar/2} and the tuple of \type{Symbol} terms \probloginline{(foo,42)}. \probloginline{foo} is of type \type{Atom} and \probloginline{42} is a \type{Number} term.
























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Syntax}
%Based on the type system, we now define the syntactic components of DC-ProbLog and its syntax.
\begin{definition}[Deterministic Rules and Facts]
	A (normal) logic program is a set of rules. A rule is a universally quantified expression of the form
	\begin{problog}
h:- b@$_1$@, @\dots@, b@$_n$@.
	\end{problog}
	where \probloginline{h} is an \type{Atom} term and $\{ \text{\probloginline{b@$_1$@}}, \text{\dots},\text{\probloginline{b@$_n$@}} \}$ is a set of $n$ literals.
	Literals are either \type{Atom} terms, or their negation.
	The \type{Atom} term \probloginline{h} is called the head of the rule and \probloginline{b@$_1$@, @\dots@, b@$_n$@} the body. The latter represents the
	conjunction $\text{\probloginline{b@$_1$@}} \land \cdots \land  \text{\probloginline{b@$_n$@}}$. A fact is a rule that has \probloginline{true} as its body and is simply written as
	\begin{problog}
h.
	\end{problog}
\end{definition}




\begin{definition}[Probabilistic Facts]
	Probabilistic facts are of the form \probloginline{p::fact}. \probloginline{p} is a term of type \type{Number} or \type{RandomVariable}, with $0{\leq} \text{\probloginline{p}} {\leq} 1$  and \probloginline{fact} is a ground atom. 
	%\begin{definition} A {\bf probabilistic fact} is a ground definite fact labeled with a probability.
\end{definition}


\begin{definition}[Distributional Facts]
	Distributional facts introduce random variable terms and associate them with a distribution using the reserved binary predicate \probloginline{~}\lstinline[columns=fixed]|/2| in infix notation. A distributional fact is a ground fact of the form \probloginline{rand ~ distribution}, where \probloginline{distribution} is a well-typed distribution term with output type \type{DistributionX} and \probloginline{rand} is a ground term whose functor is not reserved. The distributional fact introduces \probloginline{rand} as a random variable of type \type{RandomVariableX}, \ie the type of the random variable term mimics the type of the distribution term.
\end{definition}
Distributional facts can be thought of as the link between the independent choices (in form of distributions) and the discrete structure (in form of rules and facts).

\begin{definition}[Comparison predicates] \label{def:comparison}
	\dcproblogsty (similar to \prologsty and \problogsty) uses a fixed set of builtin binary predicates whose truth values depend on the \emph{evaluation} of its arguments. For terms that can be evaluated (\type{RandomVariable} terms and \type{Number} terms) we use the set
	$\bowtie=\{ \text{\probloginline{=:=}}, \text{\probloginline{=\=}}, \text{\probloginline{<}}, \text{\probloginline{>}},  \text{\probloginline{=<}}, \text{\probloginline{>=}} \}$
	of binary predicates written in infix notation.
	Each of these has the usual \prologsty arithmetic interpretation of evaluating each side and comparing the results.
	Just as for \prologsty arithmetic, truth values of atoms using these predicates are determined through an evaluation process that is external to the (probabilistic) logic program. Such atoms can be used in clause bodies, but never in clause heads (or as facts).
\end{definition}

%We will further discuss arithmetic evaluations in Subsection~\ref{sec:arithmetic}.

\begin{example} Comparison predicates allow for the comparison of random variables to numbers. 
	\begin{problog*}{linenos}
x ~ normal(0,3).
q:- x>0.
query(q).
	\end{problog*}
\end{example}



%\begin{definition}\label{def:distributional_fact}
%	A {\bf distributional fact} is a ground definite fact with the reserved binary predicate \probloginline{is}\lstinline[columns=fixed]|/2| used in infix notation.
%\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multiple Dispatch} \label{ref:multiple_dispatch}
The attentive reader might have noticed that in Definition~\ref{def:comparison} we used the same comparison predicates, for \type{RandomVariable} terms as well as \type{Number} terms. In \dcproblogsty we resolve this clash through {\em multiple dispatching}\citep{castagna1995calculus}.
{ Multiple dispatching} is the process of dynamically selecting at run time\footnote{In the context of logic programming we understand as run time the time it takes to ground the logic program part of a \dcproblogsty program.} a specific implementation of a function based on the types of the arguments that are fed as input to the corresponding function symbol.
Such functions are referred to as {\em multimethods}. 
An early example of multiple dispatch is the {\em Common Lisp Object System}~\citep{keene1989object}. Multiple dispatch is also the programming paradigm on which the \juliasty programming language is built~\citep{bezanson2017julia}. We reuse this idea in the context of probabilistic logic programming with random function symbols to retain a simple and neat syntax.
Consider, for instance, the declaration of the normal distribution in Example~\ref{example:dcproblog_machine}.
The definition of the function is the following:
$$ \text{\probloginline{normal}}: \type{Number} \times \type{Number} \rightarrow \type{ContinuousD}$$
However, the arguments of a normal distribution (its mean and standard deviation) might as well be random variables themselves.
Multiple dispatching then allows us to {\em overload} the \probloginline{normal} function symbol by using arguments of a different type\footnote{For simplicity we omit that the standard deviation has to be a strictly positive (real) number, which can be enforced by extending the type system.}:
\begin{align*}
	\text{\probloginline{normal}}&: \type{RandomVariable} \times \type{Number} \rightarrow \type{ContinuousD} \\
	\text{\probloginline{normal}}&: \type{Number} \times \type{RandomVariable} \rightarrow \type{ContinuousD} \\
	\text{\probloginline{normal}}&: \type{RandomVariable} \times \type{RandomVariable} \rightarrow \type{ContinuousD}
\end{align*}
The exact implementation of these random function symbols is left to the designer of the implementation of the language.
%In the next Subsection~\ref{sec:arithmetic} we will encounter further usages of multiple dispatching in \dcproblogsty.




\subsection{Arithmetic Evaluation}\label{sec:arithmetic}

\ak{Sec 6.1.4: you say the correct functor is determined during grounding, but doesn't grounding (at least to some extend) depend on the type of inference? \eg, if we ground during sampling, I'd expect the second line of ex 6.4 to ground the X to different numbers in different samples / runs, whereas exact inference techniques (including techniques to find the relevant ground program of a query) would probably ground to something symbolic? Theoretically speaking, grounding usually refers to grounding wrt the Herbrand universe, \ie, all the symbols in the program (plus in the case of arithmetic the countably many outcomes of arithmetic evaluations), but continuous distributions are extending that potential universe into the uncountable, so we need to be careful (and I need to think about this again for the journal version...)}

\prologsty implementations reserve a set of predicate names for system-related procedures. These system predicates are usually deployed when the goal is to perform efficient arithmetic operations on numbers, either by using specialized algortihms or specialized hardware. For example, when a user wants to add up the integers \probloginline{3} and \probloginline{5} they simply write \probloginline{Sum is 3+5}. The predicate \probloginline{is}\lstinline[columns=fixed]|/2| takes the second argument, passes it to an external evaluation engine, which performs integer addition, and unifies the result with the logical variable \probloginline{Sum}. It is rather obvious that the concept of multiple dispatch comes in handy here: the same functors can be used to perform the same operations on terms of different types. The correct functor is only dertermined during the grounding of the logic program, \ie during runtime.

The key difference between the external arithmetic engine of \prologsty (or \problogsty) and the external arithmetic engine of \dcproblogsty is that the external engine of the latter is capable of performing arithmetic operations (perform evaluations) with random variables. Combining this innovation with multiple dispatch allows us to retain the same syntax (same functor) to perform arithmetic operations on \type{RandomVariable} terms and/or \type{Number} terms.


\begin{example} A \dcproblogsty code snippet showing how random variable terms can be used in an arithmetic expression. 
	\begin{problog*}{linenos}
x ~ normal(0,3).
q:- X is x+3, X>3.
query(q).
	\end{problog*}
\end{example}

Multiple dispatch allows \dcproblogsty to call specific implementations of the comparison predicates in the external arithmetic engine.
In other words, multiple dispatch allows for using the same predicate for semantically different terms.
Comparing two terms of type \type{Number}, for example, materializes as a deterministic fact, whereas a comparison between terms of types \type{Number} and \type{RandomVariable} materializes as a probabilistic query. We will see how this extremely useful mechanism works in the next Section~\ref{sec:semantics}, where we also introduce the semantics of \dcproblogsty.




\subsection{Relationship of Multiple Dispatch to Typing in \prologsty}

Traditionally \prologsty is {\em weakly typed}. This means that only at run time (grounding time) it is checked whether a relation with certain arguments is present in the logic database, which is a set of ground relations. If the relation is not present, \prologsty implementations do usually not throw an error but the proof of the goal that is currently proven fails. For builtin predicates such as \probloginline{is}\lstinline[columns=fixed]|/2| or any comparison predicates, the run time type system is more strict and the \prologsty implementation might actually throw an error. For instance, the presence of the relation \probloginline{three=:=3} in a proof would throw an error.
Such typed arithmetic relations can be thought of as {\em multirelations}, which have a different interpretations based on their type at run time. In other words, they are the logic programming equivalent to multimethods: their interpretation depends on their predicate and the types of their arguments. 

In \dcproblogsty we extend this idea of multirelations using the framework of multiple dispatch. The major difference being that the typed relations in \dcproblogsty are not only used to select the right computation in the external arithmetic engine (\eg floating point addition vs. integer addition) but the multirelations in \dcproblogsty can also affect the structure of the probabilistic program. We will encounter examples thereof in Section~\ref{sec:dcproblog}, where we rewrite a \dcproblogsty program as a DC-PLP program and where we have rewrite rules that do not only depend on the predicate of a relation but also on the types of the relation's arguments.

Note that in \dcproblogsty not only the builtin comparison predicates and the \probloginline{is}\lstinline[columns=fixed]|/2| have a typed signature but also the random function symbols, \eg \probloginline{normal/2}. We can say that interpreted predicated and functors, that is predicates and functors that have a system internal meaning, possess a type signature. This results in a type dependent calculus.




\subsubsection*{Strongly Typed \prologsty}

While \prologsty is traditionally not strongly/statically typed, there have been efforts to extend \prologsty with such a type system. The most interesting effort is probably the one presented in~\citet{Schrijvers2008TowardsTP}, where the authors develop the idea of partially typing a \prologsty program, \ie typing is optional and untyped code is interpreted instead of compiled.  Our efforts to utilize multiple dispatch within a (probabilistic) logic programming language can be understood as an effort orthogonal to the efforts towards statically typed \prologsty. Introducing predicates with strongly typed signatures can also be regarded as adding interpreted predicates to the internal \prologsty engine. 

==> files_old/types.tex <==
\section{System Predicates and Arithmetic Evaluations}



Every Prolog implementation reserves some predicate names for
system-related procedures. Queries to these predicates, called system
predicates, are handled by special code in the implementation in contrast
to calls to predicates denned by pure Prolog programs. 


builtin predicates



The role of the system predicates for arithmetic introduced in Prolog is
to provide an interface to the underlying arithmetic capabilities of the
computer in a straightforward way. The price paid for this efficiency is
that some of the machine-oriented arithmetic operations are not as gen-
general as their logical counterparts. The interface provided is an arithmetic
evaluator, which uses the underlying arithmetic facilities of the com-
computer. 


\subsubsection{Arithmetic Evaluation}
\todo{write a paragraph introducing the use of is/2 and define its semantics}

\ak{for the cases where the lhs of is/2 ends up in a comparison atom (such as Example \ref{ex:is}), it should be enough to replace is/2 by unification and thereby delay evaluation until the comparison is externally evaluated, but if we also have "regular" uses of is/2, where the (deterministic?) result is \eg returned as an answer, then things get a bit more complex; as I don't know what uses are intended (and valid), this is for someone else to draft... (or it might be that this is really an engine rather than a language thing, in which case it should only be discussed later with the general multiple dispatch stuff)}



\ak{this sec is for Pedro to fix / integrate -- I think a lot of the Prolog type system discussion is not needed for the purpose of this paper; note that the old tex file is still there if needed again}

\dcproblogsty's type system refines the one of DC-PLP to instantiate a conrete version of the abstract language.  Specifically, we have the following refinements:
\begin{enumerate}
    \item distribution functors are further partitioned into \emph{discrete distribution functors}. \emph{continuous distribution functors} and \emph{mixture distribution functors}
    \item arithmetic functors are further partitioned into \emph{operation functors} and \emph{number functors}, with the latter in turn partitioned into \emph{integers} and \emph{floats} \todo{do we have / want a complete list of operations? should we at least give some examples?}
    \item we use Boolean query functors 	$\bowtie=\{ \text{\probloginline{=:=}}, \text{\probloginline{=\=}}, \text{\probloginline{<}}, \text{\probloginline{>}},  \text{\probloginline{=<}}, \text{\probloginline{>=}} \}$
	in infix notation (and lift them to predicate level as discussed before)
\end{enumerate}

\ak{I don't think we need to sub-type random variable functors here, as rv terms inherit the \emph{output} type of the distribution only, which should be integer, float etc, not "discrete distribution"}

\probloginline{poisson(6)} and \probloginline{normal(20,5)} are for instance of types \type{DiscreteD} and  \type{ContinuousD}, respectively.
Note that distributions of type \type{ContinuousD} denote {\em absolutely continuous} probability distributions\footnote{\dcproblogsty does not support {\em singular continuous} probability distributions such as the Cantor distribution.}. \ak{would be nice to have a hint on why this restriction is there} We give an example of a distribution of type \type{MixtureD} in Example~\ref{ex:indian_gpa_function}.

\subsection{Multiple Dispatch} \label{ref:multiple_dispatch}
The attentive reader might have noticed that in Definition~\ref{def:comparison} we used the same comparison predicates, for \type{RandomVariable} terms as well as \type{Number} terms. In \dcproblogsty we resolve this clash through {\em multiple dispatching}\citep{castagna1995calculus}.
{ Multiple dispatching} is the process of dynamically selecting at run time\footnote{In the context of logic programming we understand as run time the time it takes to ground the logic program part of a \dcproblogsty program.} a specific implementation of a function based on the types of the arguments that are fed as input to the corresponding function symbol.
Such functions are referred to as {\em multimethods}. 
An early example of multiple dispatch is the {\em Common Lisp Object System}~\citep{keene1989object}. Multiple dispatch is also the programming paradigm on which the \juliasty programming language is built~\citep{bezanson2017julia}. We reuse this idea in the context of probabilistic logic programming with random function symbols to retain a simple and neat syntax.
Consider, for instance, the declaration of the normal distribution in Example~\ref{example:dcproblog_machine}.
The definition of the function is the following:
$$ \text{\probloginline{normal}}: \type{Number} \times \type{Number} \rightarrow \type{ContinuousD}$$
However, the arguments of a normal distribution (its mean and standard deviation) might as well be random variables themselves.
Multiple dispatching then allows us to {\em overload} the \probloginline{normal} function symbol by using arguments of a different type\footnote{For simplicity we omit that the standard deviation has to be a strictly positive (real) number, which can be enforced by extending the type system.}:
\begin{align*}
	\text{\probloginline{normal}}&: \type{RandomVariable} \times \type{Number} \rightarrow \type{ContinuousD} \\
	\text{\probloginline{normal}}&: \type{Number} \times \type{RandomVariable} \rightarrow \type{ContinuousD} \\
	\text{\probloginline{normal}}&: \type{RandomVariable} \times \type{RandomVariable} \rightarrow \type{ContinuousD}
\end{align*}
The exact implementation of these random function symbols is left to the designer of the implementation of the language.
%In the next Subsection~\ref{sec:arithmetic} we will encounter further usages of multiple dispatching in \dcproblogsty.




\subsection{Arithmetic Evaluation}\label{sec:arithmetic}

\ak{Sec 6.1.4: you say the correct functor is determined during grounding, but doesn't grounding (at least to some extend) depend on the type of inference? \eg, if we ground during sampling, I'd expect the second line of ex 6.4 to ground the X to different numbers in different samples / runs, whereas exact inference techniques (including techniques to find the relevant ground program of a query) would probably ground to something symbolic? Theoretically speaking, grounding usually refers to grounding wrt the Herbrand universe, \ie, all the symbols in the program (plus in the case of arithmetic the countably many outcomes of arithmetic evaluations), but continuous distributions are extending that potential universe into the uncountable, so we need to be careful (and I need to think about this again for the journal version...)}

\prologsty implementations reserve a set of predicate names for system-related procedures. These system predicates are usually deployed when the goal is to perform efficient arithmetic operations on numbers, either by using specialized algortihms or specialized hardware. For example, when a user wants to add up the integers \probloginline{3} and \probloginline{5} they simply write \probloginline{Sum is 3+5}. The predicate \probloginline{is}\lstinline[columns=fixed]|/2| takes the second argument, passes it to an external evaluation engine, which performs integer addition, and unifies the result with the logical variable \probloginline{Sum}. It is rather obvious that the concept of multiple dispatch comes in handy here: the same functors can be used to perform the same operations on terms of different types. The correct functor is only dertermined during the grounding of the logic program, \ie during runtime.

The key difference between the external arithmetic engine of \prologsty (or \problogsty) and the external arithmetic engine of \dcproblogsty is that the external engine of the latter is capable of performing arithmetic operations (perform evaluations) with random variables. Combining this innovation with multiple dispatch allows us to retain the same syntax (same functor) to perform arithmetic operations on \type{RandomVariable} terms and/or \type{Number} terms.


\begin{example}\label{ex:is} A \dcproblogsty code snippet showing how random variable terms can be used in an arithmetic expression. 
	\begin{problog*}{linenos}
x ~ normal(0,3).
q:- X is x+3, X>3.
query(q).
	\end{problog*}
\end{example}

Multiple dispatch allows \dcproblogsty to call specific implementations of the comparison predicates in the external arithmetic engine.
In other words, multiple dispatch allows for using the same predicate for semantically different terms.
Comparing two terms of type \type{Number}, for example, materializes as a deterministic fact, whereas a comparison between terms of types \type{Number} and \type{RandomVariable} materializes as a probabilistic query. We will see how this extremely useful mechanism works in the next Section~\ref{sec:semantics}, where we also introduce the semantics of \dcproblogsty.




\subsection{Relationship of Multiple Dispatch to Typing in \prologsty}

Traditionally \prologsty is {\em weakly typed}. This means that only at run time (grounding time) it is checked whether a relation with certain arguments is present in the logic database, which is a set of ground relations. If the relation is not present, \prologsty implementations do usually not throw an error but the proof of the goal that is currently proven fails. For builtin predicates such as \probloginline{is}\lstinline[columns=fixed]|/2| or any comparison predicates, the run time type system is more strict and the \prologsty implementation might actually throw an error. For instance, the presence of the relation \probloginline{three=:=3} in a proof would throw an error.
Such typed arithmetic relations can be thought of as {\em multirelations}, which have a different interpretations based on their type at run time. In other words, they are the logic programming equivalent to multimethods: their interpretation depends on their predicate and the types of their arguments. 

In \dcproblogsty we extend this idea of multirelations using the framework of multiple dispatch. The major difference being that the typed relations in \dcproblogsty are not only used to select the right computation in the external arithmetic engine (\eg floating point addition vs. integer addition) but the multirelations in \dcproblogsty can also affect the structure of the probabilistic program. We will encounter examples thereof in Section~\ref{sec:dcproblog}, where we rewrite a \dcproblogsty program as a DC-PLP program and where we have rewrite rules that do not only depend on the predicate of a relation but also on the types of the relation's arguments.

Note that in \dcproblogsty not only the builtin comparison predicates and the \probloginline{is}\lstinline[columns=fixed]|/2| have a typed signature but also the random function symbols, \eg \probloginline{normal/2}. We can say that interpreted predicated and functors, that is predicates and functors that have a system internal meaning, possess a type signature. This results in a type dependent calculus.




\subsubsection*{Strongly Typed \prologsty}
\ak{move to related work?}

While \prologsty is traditionally not strongly/statically typed, there have been efforts to extend \prologsty with such a type system. The most interesting effort is probably the one presented in~\citet{Schrijvers2008TowardsTP}, where the authors develop the idea of partially typing a \prologsty program, \ie typing is optional and untyped code is interpreted instead of compiled.  Our efforts to utilize multiple dispatch within a (probabilistic) logic programming language can be understood as an effort orthogonal to the efforts towards statically typed \prologsty. Introducing predicates with strongly typed signatures can also be regarded as adding interpreted predicates to the internal \prologsty engine. 
